Measurements of top-quark pair to $Z$-boson cross-section ratios at $\sqrt s = 13, 8, 7$TeV with the ATLAS detector

Ratios of top-quark pair to $Z$-boson cross sections measured from proton--proton collisions at the LHC centre-of-mass energies of $\sqrt s=13$TeV, 8TeV, and 7TeV are presented by the ATLAS Collaboration. Single ratios, at a given $\sqrt s$ for the two processes and at different $\sqrt s$ for each process, as well as double ratios of the two processes at different $\sqrt s$, are evaluated. The ratios are constructed using previously published ATLAS measurements of the $t\overline{t}$ and $Z$-boson production cross sections, corrected to a common phase space where required, and a new analysis of $Z \rightarrow \ell^+ \ell^-$ where $\ell=e,\mu$ at $\sqrt s=13$TeV performed with data collected in 2015 with an integrated luminosity of $3.2$fb$^{-1}$. Correlations of systematic uncertainties are taken into account when evaluating the uncertainties in the ratios. The correlation model is also used to evaluate the combined cross section of the $Z\rightarrow e^+e^-$ and the $Z\rightarrow \mu^+ \mu^-$ channels for each $\sqrt s$ value. The results are compared to calculations performed at next-to-next-to-leading-order accuracy using recent sets of parton distribution functions. The data demonstrate significant power to constrain the gluon distribution function for the Bjorken-$x$ values near 0.1 and the light-quark sea for $x<0.02$.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 2-Aug-2016

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, the Canada Council, CANARIE, CRC, Compute Canada, FQRNT, and the Ontario Innovation Trust, Canada; EPLANET, ERC, FP7, Horizon 2020 and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d'Avenir Labex and Idex, ANR, R{\'e}gion Auvergne and Fondation Partager le Savoir, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF; BSF, GIF and Minerva, Israel; BRF, Norway; Generalitat de Catalunya, Generalitat Valenciana, Spain; the Royal Society and Leverhulme Trust, United Kingdom.

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------



==> atlas_authlist.tex <==
% ATLAS Collaboration author list
% Data extracted on 17-Nov-2016 for paper reference STDM-2016-02
%\documentclass[11pt]{article}
%\usepackage{a4wide}
%\begin{document}
\begin{flushleft}
{\Large The ATLAS Collaboration}

\bigskip

M.~Aaboud$^\textrm{\scriptsize 137d}$,
G.~Aad$^\textrm{\scriptsize 88}$,
B.~Abbott$^\textrm{\scriptsize 115}$,
J.~Abdallah$^\textrm{\scriptsize 8}$,
O.~Abdinov$^\textrm{\scriptsize 12}$,
B.~Abeloos$^\textrm{\scriptsize 119}$,
S.H.~Abidi$^\textrm{\scriptsize 161}$,
O.S.~AbouZeid$^\textrm{\scriptsize 139}$,
N.L.~Abraham$^\textrm{\scriptsize 151}$,
H.~Abramowicz$^\textrm{\scriptsize 155}$,
H.~Abreu$^\textrm{\scriptsize 154}$,
R.~Abreu$^\textrm{\scriptsize 118}$,
Y.~Abulaiti$^\textrm{\scriptsize 148a,148b}$,
B.S.~Acharya$^\textrm{\scriptsize 167a,167b}$$^{,a}$,
S.~Adachi$^\textrm{\scriptsize 157}$,
L.~Adamczyk$^\textrm{\scriptsize 41a}$,
D.L.~Adams$^\textrm{\scriptsize 27}$,
J.~Adelman$^\textrm{\scriptsize 110}$,
T.~Adye$^\textrm{\scriptsize 133}$,
A.A.~Affolder$^\textrm{\scriptsize 139}$,
T.~Agatonovic-Jovin$^\textrm{\scriptsize 14}$,
C.~Agheorghiesei$^\textrm{\scriptsize 28b}$,
J.A.~Aguilar-Saavedra$^\textrm{\scriptsize 128a,128f}$,
S.P.~Ahlen$^\textrm{\scriptsize 24}$,
F.~Ahmadov$^\textrm{\scriptsize 68}$$^{,b}$,
G.~Aielli$^\textrm{\scriptsize 135a,135b}$,
S.~Akatsuka$^\textrm{\scriptsize 71}$,
H.~Akerstedt$^\textrm{\scriptsize 148a,148b}$,
T.P.A.~{\AA}kesson$^\textrm{\scriptsize 84}$,
A.V.~Akimov$^\textrm{\scriptsize 98}$,
G.L.~Alberghi$^\textrm{\scriptsize 22a,22b}$,
J.~Albert$^\textrm{\scriptsize 172}$,
M.J.~Alconada~Verzini$^\textrm{\scriptsize 74}$,
M.~Aleksa$^\textrm{\scriptsize 32}$,
I.N.~Aleksandrov$^\textrm{\scriptsize 68}$,
C.~Alexa$^\textrm{\scriptsize 28b}$,
G.~Alexander$^\textrm{\scriptsize 155}$,
T.~Alexopoulos$^\textrm{\scriptsize 10}$,
M.~Alhroob$^\textrm{\scriptsize 115}$,
B.~Ali$^\textrm{\scriptsize 130}$,
M.~Aliev$^\textrm{\scriptsize 76a,76b}$,
G.~Alimonti$^\textrm{\scriptsize 94a}$,
J.~Alison$^\textrm{\scriptsize 33}$,
S.P.~Alkire$^\textrm{\scriptsize 38}$,
B.M.M.~Allbrooke$^\textrm{\scriptsize 151}$,
B.W.~Allen$^\textrm{\scriptsize 118}$,
P.P.~Allport$^\textrm{\scriptsize 19}$,
A.~Aloisio$^\textrm{\scriptsize 106a,106b}$,
A.~Alonso$^\textrm{\scriptsize 39}$,
F.~Alonso$^\textrm{\scriptsize 74}$,
C.~Alpigiani$^\textrm{\scriptsize 140}$,
A.A.~Alshehri$^\textrm{\scriptsize 56}$,
M.~Alstaty$^\textrm{\scriptsize 88}$,
B.~Alvarez~Gonzalez$^\textrm{\scriptsize 32}$,
D.~\'{A}lvarez~Piqueras$^\textrm{\scriptsize 170}$,
M.G.~Alviggi$^\textrm{\scriptsize 106a,106b}$,
B.T.~Amadio$^\textrm{\scriptsize 16}$,
Y.~Amaral~Coutinho$^\textrm{\scriptsize 26a}$,
C.~Amelung$^\textrm{\scriptsize 25}$,
D.~Amidei$^\textrm{\scriptsize 92}$,
S.P.~Amor~Dos~Santos$^\textrm{\scriptsize 128a,128c}$,
A.~Amorim$^\textrm{\scriptsize 128a,128b}$,
S.~Amoroso$^\textrm{\scriptsize 32}$,
G.~Amundsen$^\textrm{\scriptsize 25}$,
C.~Anastopoulos$^\textrm{\scriptsize 141}$,
L.S.~Ancu$^\textrm{\scriptsize 52}$,
N.~Andari$^\textrm{\scriptsize 19}$,
T.~Andeen$^\textrm{\scriptsize 11}$,
C.F.~Anders$^\textrm{\scriptsize 60b}$,
J.K.~Anders$^\textrm{\scriptsize 77}$,
K.J.~Anderson$^\textrm{\scriptsize 33}$,
A.~Andreazza$^\textrm{\scriptsize 94a,94b}$,
V.~Andrei$^\textrm{\scriptsize 60a}$,
S.~Angelidakis$^\textrm{\scriptsize 9}$,
I.~Angelozzi$^\textrm{\scriptsize 109}$,
A.~Angerami$^\textrm{\scriptsize 38}$,
F.~Anghinolfi$^\textrm{\scriptsize 32}$,
A.V.~Anisenkov$^\textrm{\scriptsize 111}$$^{,c}$,
N.~Anjos$^\textrm{\scriptsize 13}$,
A.~Annovi$^\textrm{\scriptsize 126a,126b}$,
C.~Antel$^\textrm{\scriptsize 60a}$,
M.~Antonelli$^\textrm{\scriptsize 50}$,
A.~Antonov$^\textrm{\scriptsize 100}$$^{,*}$,
D.J.~Antrim$^\textrm{\scriptsize 166}$,
F.~Anulli$^\textrm{\scriptsize 134a}$,
M.~Aoki$^\textrm{\scriptsize 69}$,
L.~Aperio~Bella$^\textrm{\scriptsize 19}$,
G.~Arabidze$^\textrm{\scriptsize 93}$,
Y.~Arai$^\textrm{\scriptsize 69}$,
J.P.~Araque$^\textrm{\scriptsize 128a}$,
V.~Araujo~Ferraz$^\textrm{\scriptsize 26a}$,
A.T.H.~Arce$^\textrm{\scriptsize 48}$,
F.A.~Arduh$^\textrm{\scriptsize 74}$,
J-F.~Arguin$^\textrm{\scriptsize 97}$,
S.~Argyropoulos$^\textrm{\scriptsize 66}$,
M.~Arik$^\textrm{\scriptsize 20a}$,
A.J.~Armbruster$^\textrm{\scriptsize 145}$,
L.J.~Armitage$^\textrm{\scriptsize 79}$,
O.~Arnaez$^\textrm{\scriptsize 32}$,
H.~Arnold$^\textrm{\scriptsize 51}$,
M.~Arratia$^\textrm{\scriptsize 30}$,
O.~Arslan$^\textrm{\scriptsize 23}$,
A.~Artamonov$^\textrm{\scriptsize 99}$,
G.~Artoni$^\textrm{\scriptsize 122}$,
S.~Artz$^\textrm{\scriptsize 86}$,
S.~Asai$^\textrm{\scriptsize 157}$,
N.~Asbah$^\textrm{\scriptsize 45}$,
A.~Ashkenazi$^\textrm{\scriptsize 155}$,
B.~{\AA}sman$^\textrm{\scriptsize 148a,148b}$,
L.~Asquith$^\textrm{\scriptsize 151}$,
K.~Assamagan$^\textrm{\scriptsize 27}$,
R.~Astalos$^\textrm{\scriptsize 146a}$,
M.~Atkinson$^\textrm{\scriptsize 169}$,
N.B.~Atlay$^\textrm{\scriptsize 143}$,
K.~Augsten$^\textrm{\scriptsize 130}$,
G.~Avolio$^\textrm{\scriptsize 32}$,
B.~Axen$^\textrm{\scriptsize 16}$,
M.K.~Ayoub$^\textrm{\scriptsize 119}$,
G.~Azuelos$^\textrm{\scriptsize 97}$$^{,d}$,
A.E.~Baas$^\textrm{\scriptsize 60a}$,
M.J.~Baca$^\textrm{\scriptsize 19}$,
H.~Bachacou$^\textrm{\scriptsize 138}$,
K.~Bachas$^\textrm{\scriptsize 76a,76b}$,
M.~Backes$^\textrm{\scriptsize 122}$,
M.~Backhaus$^\textrm{\scriptsize 32}$,
P.~Bagiacchi$^\textrm{\scriptsize 134a,134b}$,
P.~Bagnaia$^\textrm{\scriptsize 134a,134b}$,
J.T.~Baines$^\textrm{\scriptsize 133}$,
M.~Bajic$^\textrm{\scriptsize 39}$,
O.K.~Baker$^\textrm{\scriptsize 179}$,
E.M.~Baldin$^\textrm{\scriptsize 111}$$^{,c}$,
P.~Balek$^\textrm{\scriptsize 175}$,
T.~Balestri$^\textrm{\scriptsize 150}$,
F.~Balli$^\textrm{\scriptsize 138}$,
W.K.~Balunas$^\textrm{\scriptsize 124}$,
E.~Banas$^\textrm{\scriptsize 42}$,
Sw.~Banerjee$^\textrm{\scriptsize 176}$$^{,e}$,
A.A.E.~Bannoura$^\textrm{\scriptsize 178}$,
L.~Barak$^\textrm{\scriptsize 32}$,
E.L.~Barberio$^\textrm{\scriptsize 91}$,
D.~Barberis$^\textrm{\scriptsize 53a,53b}$,
M.~Barbero$^\textrm{\scriptsize 88}$,
T.~Barillari$^\textrm{\scriptsize 103}$,
M-S~Barisits$^\textrm{\scriptsize 32}$,
T.~Barklow$^\textrm{\scriptsize 145}$,
N.~Barlow$^\textrm{\scriptsize 30}$,
S.L.~Barnes$^\textrm{\scriptsize 87}$,
B.M.~Barnett$^\textrm{\scriptsize 133}$,
R.M.~Barnett$^\textrm{\scriptsize 16}$,
Z.~Barnovska-Blenessy$^\textrm{\scriptsize 36a}$,
A.~Baroncelli$^\textrm{\scriptsize 136a}$,
G.~Barone$^\textrm{\scriptsize 25}$,
A.J.~Barr$^\textrm{\scriptsize 122}$,
L.~Barranco~Navarro$^\textrm{\scriptsize 170}$,
F.~Barreiro$^\textrm{\scriptsize 85}$,
J.~Barreiro~Guimar\~{a}es~da~Costa$^\textrm{\scriptsize 35a}$,
R.~Bartoldus$^\textrm{\scriptsize 145}$,
A.E.~Barton$^\textrm{\scriptsize 75}$,
P.~Bartos$^\textrm{\scriptsize 146a}$,
A.~Basalaev$^\textrm{\scriptsize 125}$,
A.~Bassalat$^\textrm{\scriptsize 119}$$^{,f}$,
R.L.~Bates$^\textrm{\scriptsize 56}$,
S.J.~Batista$^\textrm{\scriptsize 161}$,
J.R.~Batley$^\textrm{\scriptsize 30}$,
M.~Battaglia$^\textrm{\scriptsize 139}$,
M.~Bauce$^\textrm{\scriptsize 134a,134b}$,
F.~Bauer$^\textrm{\scriptsize 138}$,
H.S.~Bawa$^\textrm{\scriptsize 145}$$^{,g}$,
J.B.~Beacham$^\textrm{\scriptsize 113}$,
M.D.~Beattie$^\textrm{\scriptsize 75}$,
T.~Beau$^\textrm{\scriptsize 83}$,
P.H.~Beauchemin$^\textrm{\scriptsize 165}$,
P.~Bechtle$^\textrm{\scriptsize 23}$,
H.P.~Beck$^\textrm{\scriptsize 18}$$^{,h}$,
K.~Becker$^\textrm{\scriptsize 122}$,
M.~Becker$^\textrm{\scriptsize 86}$,
M.~Beckingham$^\textrm{\scriptsize 173}$,
C.~Becot$^\textrm{\scriptsize 112}$,
A.J.~Beddall$^\textrm{\scriptsize 20e}$,
A.~Beddall$^\textrm{\scriptsize 20b}$,
V.A.~Bednyakov$^\textrm{\scriptsize 68}$,
M.~Bedognetti$^\textrm{\scriptsize 109}$,
C.P.~Bee$^\textrm{\scriptsize 150}$,
L.J.~Beemster$^\textrm{\scriptsize 109}$,
T.A.~Beermann$^\textrm{\scriptsize 32}$,
M.~Begel$^\textrm{\scriptsize 27}$,
J.K.~Behr$^\textrm{\scriptsize 45}$,
A.S.~Bell$^\textrm{\scriptsize 81}$,
G.~Bella$^\textrm{\scriptsize 155}$,
L.~Bellagamba$^\textrm{\scriptsize 22a}$,
A.~Bellerive$^\textrm{\scriptsize 31}$,
M.~Bellomo$^\textrm{\scriptsize 89}$,
K.~Belotskiy$^\textrm{\scriptsize 100}$,
O.~Beltramello$^\textrm{\scriptsize 32}$,
N.L.~Belyaev$^\textrm{\scriptsize 100}$,
O.~Benary$^\textrm{\scriptsize 155}$$^{,*}$,
D.~Benchekroun$^\textrm{\scriptsize 137a}$,
M.~Bender$^\textrm{\scriptsize 102}$,
K.~Bendtz$^\textrm{\scriptsize 148a,148b}$,
N.~Benekos$^\textrm{\scriptsize 10}$,
Y.~Benhammou$^\textrm{\scriptsize 155}$,
E.~Benhar~Noccioli$^\textrm{\scriptsize 179}$,
J.~Benitez$^\textrm{\scriptsize 66}$,
D.P.~Benjamin$^\textrm{\scriptsize 48}$,
M.~Benoit$^\textrm{\scriptsize 52}$,
J.R.~Bensinger$^\textrm{\scriptsize 25}$,
S.~Bentvelsen$^\textrm{\scriptsize 109}$,
L.~Beresford$^\textrm{\scriptsize 122}$,
M.~Beretta$^\textrm{\scriptsize 50}$,
D.~Berge$^\textrm{\scriptsize 109}$,
E.~Bergeaas~Kuutmann$^\textrm{\scriptsize 168}$,
N.~Berger$^\textrm{\scriptsize 5}$,
J.~Beringer$^\textrm{\scriptsize 16}$,
S.~Berlendis$^\textrm{\scriptsize 58}$,
N.R.~Bernard$^\textrm{\scriptsize 89}$,
G.~Bernardi$^\textrm{\scriptsize 83}$,
C.~Bernius$^\textrm{\scriptsize 112}$,
F.U.~Bernlochner$^\textrm{\scriptsize 23}$,
T.~Berry$^\textrm{\scriptsize 80}$,
P.~Berta$^\textrm{\scriptsize 131}$,
C.~Bertella$^\textrm{\scriptsize 86}$,
G.~Bertoli$^\textrm{\scriptsize 148a,148b}$,
F.~Bertolucci$^\textrm{\scriptsize 126a,126b}$,
I.A.~Bertram$^\textrm{\scriptsize 75}$,
C.~Bertsche$^\textrm{\scriptsize 45}$,
D.~Bertsche$^\textrm{\scriptsize 115}$,
G.J.~Besjes$^\textrm{\scriptsize 39}$,
O.~Bessidskaia~Bylund$^\textrm{\scriptsize 148a,148b}$,
M.~Bessner$^\textrm{\scriptsize 45}$,
N.~Besson$^\textrm{\scriptsize 138}$,
C.~Betancourt$^\textrm{\scriptsize 51}$,
A.~Bethani$^\textrm{\scriptsize 58}$,
S.~Bethke$^\textrm{\scriptsize 103}$,
A.J.~Bevan$^\textrm{\scriptsize 79}$,
R.M.~Bianchi$^\textrm{\scriptsize 127}$,
M.~Bianco$^\textrm{\scriptsize 32}$,
O.~Biebel$^\textrm{\scriptsize 102}$,
D.~Biedermann$^\textrm{\scriptsize 17}$,
R.~Bielski$^\textrm{\scriptsize 87}$,
N.V.~Biesuz$^\textrm{\scriptsize 126a,126b}$,
M.~Biglietti$^\textrm{\scriptsize 136a}$,
J.~Bilbao~De~Mendizabal$^\textrm{\scriptsize 52}$,
T.R.V.~Billoud$^\textrm{\scriptsize 97}$,
H.~Bilokon$^\textrm{\scriptsize 50}$,
M.~Bindi$^\textrm{\scriptsize 57}$,
A.~Bingul$^\textrm{\scriptsize 20b}$,
C.~Bini$^\textrm{\scriptsize 134a,134b}$,
S.~Biondi$^\textrm{\scriptsize 22a,22b}$,
T.~Bisanz$^\textrm{\scriptsize 57}$,
C.~Bittrich$^\textrm{\scriptsize 47}$,
D.M.~Bjergaard$^\textrm{\scriptsize 48}$,
C.W.~Black$^\textrm{\scriptsize 152}$,
J.E.~Black$^\textrm{\scriptsize 145}$,
K.M.~Black$^\textrm{\scriptsize 24}$,
D.~Blackburn$^\textrm{\scriptsize 140}$,
R.E.~Blair$^\textrm{\scriptsize 6}$,
T.~Blazek$^\textrm{\scriptsize 146a}$,
I.~Bloch$^\textrm{\scriptsize 45}$,
C.~Blocker$^\textrm{\scriptsize 25}$,
A.~Blue$^\textrm{\scriptsize 56}$,
W.~Blum$^\textrm{\scriptsize 86}$$^{,*}$,
U.~Blumenschein$^\textrm{\scriptsize 57}$,
S.~Blunier$^\textrm{\scriptsize 34a}$,
G.J.~Bobbink$^\textrm{\scriptsize 109}$,
V.S.~Bobrovnikov$^\textrm{\scriptsize 111}$$^{,c}$,
S.S.~Bocchetta$^\textrm{\scriptsize 84}$,
A.~Bocci$^\textrm{\scriptsize 48}$,
C.~Bock$^\textrm{\scriptsize 102}$,
M.~Boehler$^\textrm{\scriptsize 51}$,
D.~Boerner$^\textrm{\scriptsize 178}$,
D.~Bogavac$^\textrm{\scriptsize 102}$,
A.G.~Bogdanchikov$^\textrm{\scriptsize 111}$,
C.~Bohm$^\textrm{\scriptsize 148a}$,
V.~Boisvert$^\textrm{\scriptsize 80}$,
P.~Bokan$^\textrm{\scriptsize 168}$,
T.~Bold$^\textrm{\scriptsize 41a}$,
A.S.~Boldyrev$^\textrm{\scriptsize 101}$,
M.~Bomben$^\textrm{\scriptsize 83}$,
M.~Bona$^\textrm{\scriptsize 79}$,
M.~Boonekamp$^\textrm{\scriptsize 138}$,
A.~Borisov$^\textrm{\scriptsize 132}$,
G.~Borissov$^\textrm{\scriptsize 75}$,
J.~Bortfeldt$^\textrm{\scriptsize 32}$,
D.~Bortoletto$^\textrm{\scriptsize 122}$,
V.~Bortolotto$^\textrm{\scriptsize 62a,62b,62c}$,
K.~Bos$^\textrm{\scriptsize 109}$,
D.~Boscherini$^\textrm{\scriptsize 22a}$,
M.~Bosman$^\textrm{\scriptsize 13}$,
J.D.~Bossio~Sola$^\textrm{\scriptsize 29}$,
J.~Boudreau$^\textrm{\scriptsize 127}$,
J.~Bouffard$^\textrm{\scriptsize 2}$,
E.V.~Bouhova-Thacker$^\textrm{\scriptsize 75}$,
D.~Boumediene$^\textrm{\scriptsize 37}$,
C.~Bourdarios$^\textrm{\scriptsize 119}$,
S.K.~Boutle$^\textrm{\scriptsize 56}$,
A.~Boveia$^\textrm{\scriptsize 113}$,
J.~Boyd$^\textrm{\scriptsize 32}$,
I.R.~Boyko$^\textrm{\scriptsize 68}$,
J.~Bracinik$^\textrm{\scriptsize 19}$,
A.~Brandt$^\textrm{\scriptsize 8}$,
G.~Brandt$^\textrm{\scriptsize 57}$,
O.~Brandt$^\textrm{\scriptsize 60a}$,
U.~Bratzler$^\textrm{\scriptsize 158}$,
B.~Brau$^\textrm{\scriptsize 89}$,
J.E.~Brau$^\textrm{\scriptsize 118}$,
W.D.~Breaden~Madden$^\textrm{\scriptsize 56}$,
K.~Brendlinger$^\textrm{\scriptsize 45}$,
A.J.~Brennan$^\textrm{\scriptsize 91}$,
L.~Brenner$^\textrm{\scriptsize 109}$,
R.~Brenner$^\textrm{\scriptsize 168}$,
S.~Bressler$^\textrm{\scriptsize 175}$,
T.M.~Bristow$^\textrm{\scriptsize 49}$,
D.~Britton$^\textrm{\scriptsize 56}$,
D.~Britzger$^\textrm{\scriptsize 45}$,
F.M.~Brochu$^\textrm{\scriptsize 30}$,
I.~Brock$^\textrm{\scriptsize 23}$,
R.~Brock$^\textrm{\scriptsize 93}$,
G.~Brooijmans$^\textrm{\scriptsize 38}$,
T.~Brooks$^\textrm{\scriptsize 80}$,
W.K.~Brooks$^\textrm{\scriptsize 34b}$,
J.~Brosamer$^\textrm{\scriptsize 16}$,
E.~Brost$^\textrm{\scriptsize 110}$,
J.H~Broughton$^\textrm{\scriptsize 19}$,
P.A.~Bruckman~de~Renstrom$^\textrm{\scriptsize 42}$,
D.~Bruncko$^\textrm{\scriptsize 146b}$,
A.~Bruni$^\textrm{\scriptsize 22a}$,
G.~Bruni$^\textrm{\scriptsize 22a}$,
L.S.~Bruni$^\textrm{\scriptsize 109}$,
BH~Brunt$^\textrm{\scriptsize 30}$,
M.~Bruschi$^\textrm{\scriptsize 22a}$,
N.~Bruscino$^\textrm{\scriptsize 23}$,
P.~Bryant$^\textrm{\scriptsize 33}$,
L.~Bryngemark$^\textrm{\scriptsize 84}$,
T.~Buanes$^\textrm{\scriptsize 15}$,
Q.~Buat$^\textrm{\scriptsize 144}$,
P.~Buchholz$^\textrm{\scriptsize 143}$,
A.G.~Buckley$^\textrm{\scriptsize 56}$,
I.A.~Budagov$^\textrm{\scriptsize 68}$,
F.~Buehrer$^\textrm{\scriptsize 51}$,
M.K.~Bugge$^\textrm{\scriptsize 121}$,
O.~Bulekov$^\textrm{\scriptsize 100}$,
D.~Bullock$^\textrm{\scriptsize 8}$,
H.~Burckhart$^\textrm{\scriptsize 32}$,
S.~Burdin$^\textrm{\scriptsize 77}$,
C.D.~Burgard$^\textrm{\scriptsize 51}$,
A.M.~Burger$^\textrm{\scriptsize 5}$,
B.~Burghgrave$^\textrm{\scriptsize 110}$,
K.~Burka$^\textrm{\scriptsize 42}$,
S.~Burke$^\textrm{\scriptsize 133}$,
I.~Burmeister$^\textrm{\scriptsize 46}$,
J.T.P.~Burr$^\textrm{\scriptsize 122}$,
E.~Busato$^\textrm{\scriptsize 37}$,
D.~B\"uscher$^\textrm{\scriptsize 51}$,
V.~B\"uscher$^\textrm{\scriptsize 86}$,
P.~Bussey$^\textrm{\scriptsize 56}$,
J.M.~Butler$^\textrm{\scriptsize 24}$,
C.M.~Buttar$^\textrm{\scriptsize 56}$,
J.M.~Butterworth$^\textrm{\scriptsize 81}$,
P.~Butti$^\textrm{\scriptsize 109}$,
W.~Buttinger$^\textrm{\scriptsize 27}$,
A.~Buzatu$^\textrm{\scriptsize 35c}$,
A.R.~Buzykaev$^\textrm{\scriptsize 111}$$^{,c}$,
S.~Cabrera~Urb\'an$^\textrm{\scriptsize 170}$,
D.~Caforio$^\textrm{\scriptsize 130}$,
V.M.~Cairo$^\textrm{\scriptsize 40a,40b}$,
O.~Cakir$^\textrm{\scriptsize 4a}$,
N.~Calace$^\textrm{\scriptsize 52}$,
P.~Calafiura$^\textrm{\scriptsize 16}$,
A.~Calandri$^\textrm{\scriptsize 88}$,
G.~Calderini$^\textrm{\scriptsize 83}$,
P.~Calfayan$^\textrm{\scriptsize 64}$,
G.~Callea$^\textrm{\scriptsize 40a,40b}$,
L.P.~Caloba$^\textrm{\scriptsize 26a}$,
S.~Calvente~Lopez$^\textrm{\scriptsize 85}$,
D.~Calvet$^\textrm{\scriptsize 37}$,
S.~Calvet$^\textrm{\scriptsize 37}$,
T.P.~Calvet$^\textrm{\scriptsize 88}$,
R.~Camacho~Toro$^\textrm{\scriptsize 33}$,
S.~Camarda$^\textrm{\scriptsize 32}$,
P.~Camarri$^\textrm{\scriptsize 135a,135b}$,
D.~Cameron$^\textrm{\scriptsize 121}$,
R.~Caminal~Armadans$^\textrm{\scriptsize 169}$,
C.~Camincher$^\textrm{\scriptsize 58}$,
S.~Campana$^\textrm{\scriptsize 32}$,
M.~Campanelli$^\textrm{\scriptsize 81}$,
A.~Camplani$^\textrm{\scriptsize 94a,94b}$,
A.~Campoverde$^\textrm{\scriptsize 143}$,
V.~Canale$^\textrm{\scriptsize 106a,106b}$,
M.~Cano~Bret$^\textrm{\scriptsize 36c}$,
J.~Cantero$^\textrm{\scriptsize 116}$,
T.~Cao$^\textrm{\scriptsize 155}$,
M.D.M.~Capeans~Garrido$^\textrm{\scriptsize 32}$,
I.~Caprini$^\textrm{\scriptsize 28b}$,
M.~Caprini$^\textrm{\scriptsize 28b}$,
M.~Capua$^\textrm{\scriptsize 40a,40b}$,
R.M.~Carbone$^\textrm{\scriptsize 38}$,
R.~Cardarelli$^\textrm{\scriptsize 135a}$,
F.~Cardillo$^\textrm{\scriptsize 51}$,
I.~Carli$^\textrm{\scriptsize 131}$,
T.~Carli$^\textrm{\scriptsize 32}$,
G.~Carlino$^\textrm{\scriptsize 106a}$,
B.T.~Carlson$^\textrm{\scriptsize 127}$,
L.~Carminati$^\textrm{\scriptsize 94a,94b}$,
R.M.D.~Carney$^\textrm{\scriptsize 148a,148b}$,
S.~Caron$^\textrm{\scriptsize 108}$,
E.~Carquin$^\textrm{\scriptsize 34b}$,
G.D.~Carrillo-Montoya$^\textrm{\scriptsize 32}$,
J.R.~Carter$^\textrm{\scriptsize 30}$,
J.~Carvalho$^\textrm{\scriptsize 128a,128c}$,
D.~Casadei$^\textrm{\scriptsize 19}$,
M.P.~Casado$^\textrm{\scriptsize 13}$$^{,i}$,
M.~Casolino$^\textrm{\scriptsize 13}$,
D.W.~Casper$^\textrm{\scriptsize 166}$,
R.~Castelijn$^\textrm{\scriptsize 109}$,
A.~Castelli$^\textrm{\scriptsize 109}$,
V.~Castillo~Gimenez$^\textrm{\scriptsize 170}$,
N.F.~Castro$^\textrm{\scriptsize 128a}$$^{,j}$,
A.~Catinaccio$^\textrm{\scriptsize 32}$,
J.R.~Catmore$^\textrm{\scriptsize 121}$,
A.~Cattai$^\textrm{\scriptsize 32}$,
J.~Caudron$^\textrm{\scriptsize 23}$,
V.~Cavaliere$^\textrm{\scriptsize 169}$,
E.~Cavallaro$^\textrm{\scriptsize 13}$,
D.~Cavalli$^\textrm{\scriptsize 94a}$,
M.~Cavalli-Sforza$^\textrm{\scriptsize 13}$,
V.~Cavasinni$^\textrm{\scriptsize 126a,126b}$,
F.~Ceradini$^\textrm{\scriptsize 136a,136b}$,
L.~Cerda~Alberich$^\textrm{\scriptsize 170}$,
A.S.~Cerqueira$^\textrm{\scriptsize 26b}$,
A.~Cerri$^\textrm{\scriptsize 151}$,
L.~Cerrito$^\textrm{\scriptsize 135a,135b}$,
F.~Cerutti$^\textrm{\scriptsize 16}$,
A.~Cervelli$^\textrm{\scriptsize 18}$,
S.A.~Cetin$^\textrm{\scriptsize 20d}$,
A.~Chafaq$^\textrm{\scriptsize 137a}$,
D.~Chakraborty$^\textrm{\scriptsize 110}$,
S.K.~Chan$^\textrm{\scriptsize 59}$,
W.S.~Chan$^\textrm{\scriptsize 62a}$,
Y.L.~Chan$^\textrm{\scriptsize 62a}$,
P.~Chang$^\textrm{\scriptsize 169}$,
J.D.~Chapman$^\textrm{\scriptsize 30}$,
D.G.~Charlton$^\textrm{\scriptsize 19}$,
A.~Chatterjee$^\textrm{\scriptsize 52}$,
C.C.~Chau$^\textrm{\scriptsize 161}$,
C.A.~Chavez~Barajas$^\textrm{\scriptsize 151}$,
S.~Che$^\textrm{\scriptsize 113}$,
S.~Cheatham$^\textrm{\scriptsize 167a,167c}$,
A.~Chegwidden$^\textrm{\scriptsize 93}$,
S.~Chekanov$^\textrm{\scriptsize 6}$,
S.V.~Chekulaev$^\textrm{\scriptsize 163a}$,
G.A.~Chelkov$^\textrm{\scriptsize 68}$$^{,k}$,
M.A.~Chelstowska$^\textrm{\scriptsize 32}$,
C.~Chen$^\textrm{\scriptsize 67}$,
H.~Chen$^\textrm{\scriptsize 27}$,
S.~Chen$^\textrm{\scriptsize 35b}$,
S.~Chen$^\textrm{\scriptsize 157}$,
X.~Chen$^\textrm{\scriptsize 35c}$$^{,l}$,
Y.~Chen$^\textrm{\scriptsize 70}$,
H.C.~Cheng$^\textrm{\scriptsize 92}$,
H.J.~Cheng$^\textrm{\scriptsize 35a}$,
Y.~Cheng$^\textrm{\scriptsize 33}$,
A.~Cheplakov$^\textrm{\scriptsize 68}$,
E.~Cheremushkina$^\textrm{\scriptsize 132}$,
R.~Cherkaoui~El~Moursli$^\textrm{\scriptsize 137e}$,
V.~Chernyatin$^\textrm{\scriptsize 27}$$^{,*}$,
E.~Cheu$^\textrm{\scriptsize 7}$,
L.~Chevalier$^\textrm{\scriptsize 138}$,
V.~Chiarella$^\textrm{\scriptsize 50}$,
G.~Chiarelli$^\textrm{\scriptsize 126a,126b}$,
G.~Chiodini$^\textrm{\scriptsize 76a}$,
A.S.~Chisholm$^\textrm{\scriptsize 32}$,
A.~Chitan$^\textrm{\scriptsize 28b}$,
Y.H.~Chiu$^\textrm{\scriptsize 172}$,
M.V.~Chizhov$^\textrm{\scriptsize 68}$,
K.~Choi$^\textrm{\scriptsize 64}$,
A.R.~Chomont$^\textrm{\scriptsize 37}$,
S.~Chouridou$^\textrm{\scriptsize 9}$,
B.K.B.~Chow$^\textrm{\scriptsize 102}$,
V.~Christodoulou$^\textrm{\scriptsize 81}$,
D.~Chromek-Burckhart$^\textrm{\scriptsize 32}$,
J.~Chudoba$^\textrm{\scriptsize 129}$,
A.J.~Chuinard$^\textrm{\scriptsize 90}$,
J.J.~Chwastowski$^\textrm{\scriptsize 42}$,
L.~Chytka$^\textrm{\scriptsize 117}$,
A.K.~Ciftci$^\textrm{\scriptsize 4a}$,
D.~Cinca$^\textrm{\scriptsize 46}$,
V.~Cindro$^\textrm{\scriptsize 78}$,
I.A.~Cioara$^\textrm{\scriptsize 23}$,
C.~Ciocca$^\textrm{\scriptsize 22a,22b}$,
A.~Ciocio$^\textrm{\scriptsize 16}$,
F.~Cirotto$^\textrm{\scriptsize 106a,106b}$,
Z.H.~Citron$^\textrm{\scriptsize 175}$,
M.~Citterio$^\textrm{\scriptsize 94a}$,
M.~Ciubancan$^\textrm{\scriptsize 28b}$,
A.~Clark$^\textrm{\scriptsize 52}$,
B.L.~Clark$^\textrm{\scriptsize 59}$,
M.R.~Clark$^\textrm{\scriptsize 38}$,
P.J.~Clark$^\textrm{\scriptsize 49}$,
R.N.~Clarke$^\textrm{\scriptsize 16}$,
C.~Clement$^\textrm{\scriptsize 148a,148b}$,
Y.~Coadou$^\textrm{\scriptsize 88}$,
M.~Cobal$^\textrm{\scriptsize 167a,167c}$,
A.~Coccaro$^\textrm{\scriptsize 52}$,
J.~Cochran$^\textrm{\scriptsize 67}$,
L.~Colasurdo$^\textrm{\scriptsize 108}$,
B.~Cole$^\textrm{\scriptsize 38}$,
A.P.~Colijn$^\textrm{\scriptsize 109}$,
J.~Collot$^\textrm{\scriptsize 58}$,
T.~Colombo$^\textrm{\scriptsize 166}$,
P.~Conde~Mui\~no$^\textrm{\scriptsize 128a,128b}$,
E.~Coniavitis$^\textrm{\scriptsize 51}$,
S.H.~Connell$^\textrm{\scriptsize 147b}$,
I.A.~Connelly$^\textrm{\scriptsize 80}$,
V.~Consorti$^\textrm{\scriptsize 51}$,
S.~Constantinescu$^\textrm{\scriptsize 28b}$,
G.~Conti$^\textrm{\scriptsize 32}$,
F.~Conventi$^\textrm{\scriptsize 106a}$$^{,m}$,
M.~Cooke$^\textrm{\scriptsize 16}$,
B.D.~Cooper$^\textrm{\scriptsize 81}$,
A.M.~Cooper-Sarkar$^\textrm{\scriptsize 122}$,
F.~Cormier$^\textrm{\scriptsize 171}$,
K.J.R.~Cormier$^\textrm{\scriptsize 161}$,
T.~Cornelissen$^\textrm{\scriptsize 178}$,
M.~Corradi$^\textrm{\scriptsize 134a,134b}$,
F.~Corriveau$^\textrm{\scriptsize 90}$$^{,n}$,
A.~Cortes-Gonzalez$^\textrm{\scriptsize 32}$,
G.~Cortiana$^\textrm{\scriptsize 103}$,
G.~Costa$^\textrm{\scriptsize 94a}$,
M.J.~Costa$^\textrm{\scriptsize 170}$,
D.~Costanzo$^\textrm{\scriptsize 141}$,
G.~Cottin$^\textrm{\scriptsize 30}$,
G.~Cowan$^\textrm{\scriptsize 80}$,
B.E.~Cox$^\textrm{\scriptsize 87}$,
K.~Cranmer$^\textrm{\scriptsize 112}$,
S.J.~Crawley$^\textrm{\scriptsize 56}$,
R.A.~Creager$^\textrm{\scriptsize 124}$,
G.~Cree$^\textrm{\scriptsize 31}$,
S.~Cr\'ep\'e-Renaudin$^\textrm{\scriptsize 58}$,
F.~Crescioli$^\textrm{\scriptsize 83}$,
W.A.~Cribbs$^\textrm{\scriptsize 148a,148b}$,
M.~Crispin~Ortuzar$^\textrm{\scriptsize 122}$,
M.~Cristinziani$^\textrm{\scriptsize 23}$,
V.~Croft$^\textrm{\scriptsize 108}$,
G.~Crosetti$^\textrm{\scriptsize 40a,40b}$,
A.~Cueto$^\textrm{\scriptsize 85}$,
T.~Cuhadar~Donszelmann$^\textrm{\scriptsize 141}$,
J.~Cummings$^\textrm{\scriptsize 179}$,
M.~Curatolo$^\textrm{\scriptsize 50}$,
J.~C\'uth$^\textrm{\scriptsize 86}$,
H.~Czirr$^\textrm{\scriptsize 143}$,
P.~Czodrowski$^\textrm{\scriptsize 3}$,
G.~D'amen$^\textrm{\scriptsize 22a,22b}$,
S.~D'Auria$^\textrm{\scriptsize 56}$,
M.~D'Onofrio$^\textrm{\scriptsize 77}$,
M.J.~Da~Cunha~Sargedas~De~Sousa$^\textrm{\scriptsize 128a,128b}$,
C.~Da~Via$^\textrm{\scriptsize 87}$,
W.~Dabrowski$^\textrm{\scriptsize 41a}$,
T.~Dado$^\textrm{\scriptsize 146a}$,
T.~Dai$^\textrm{\scriptsize 92}$,
O.~Dale$^\textrm{\scriptsize 15}$,
F.~Dallaire$^\textrm{\scriptsize 97}$,
C.~Dallapiccola$^\textrm{\scriptsize 89}$,
M.~Dam$^\textrm{\scriptsize 39}$,
J.R.~Dandoy$^\textrm{\scriptsize 124}$,
N.P.~Dang$^\textrm{\scriptsize 51}$,
A.C.~Daniells$^\textrm{\scriptsize 19}$,
N.S.~Dann$^\textrm{\scriptsize 87}$,
M.~Danninger$^\textrm{\scriptsize 171}$,
M.~Dano~Hoffmann$^\textrm{\scriptsize 138}$,
V.~Dao$^\textrm{\scriptsize 51}$,
G.~Darbo$^\textrm{\scriptsize 53a}$,
S.~Darmora$^\textrm{\scriptsize 8}$,
J.~Dassoulas$^\textrm{\scriptsize 3}$,
A.~Dattagupta$^\textrm{\scriptsize 118}$,
T.~Daubney$^\textrm{\scriptsize 45}$,
W.~Davey$^\textrm{\scriptsize 23}$,
C.~David$^\textrm{\scriptsize 45}$,
T.~Davidek$^\textrm{\scriptsize 131}$,
M.~Davies$^\textrm{\scriptsize 155}$,
P.~Davison$^\textrm{\scriptsize 81}$,
E.~Dawe$^\textrm{\scriptsize 91}$,
I.~Dawson$^\textrm{\scriptsize 141}$,
K.~De$^\textrm{\scriptsize 8}$,
R.~de~Asmundis$^\textrm{\scriptsize 106a}$,
A.~De~Benedetti$^\textrm{\scriptsize 115}$,
S.~De~Castro$^\textrm{\scriptsize 22a,22b}$,
S.~De~Cecco$^\textrm{\scriptsize 83}$,
N.~De~Groot$^\textrm{\scriptsize 108}$,
P.~de~Jong$^\textrm{\scriptsize 109}$,
H.~De~la~Torre$^\textrm{\scriptsize 93}$,
F.~De~Lorenzi$^\textrm{\scriptsize 67}$,
A.~De~Maria$^\textrm{\scriptsize 57}$,
D.~De~Pedis$^\textrm{\scriptsize 134a}$,
A.~De~Salvo$^\textrm{\scriptsize 134a}$,
U.~De~Sanctis$^\textrm{\scriptsize 151}$,
A.~De~Santo$^\textrm{\scriptsize 151}$,
J.B.~De~Vivie~De~Regie$^\textrm{\scriptsize 119}$,
W.J.~Dearnaley$^\textrm{\scriptsize 75}$,
R.~Debbe$^\textrm{\scriptsize 27}$,
C.~Debenedetti$^\textrm{\scriptsize 139}$,
D.V.~Dedovich$^\textrm{\scriptsize 68}$,
N.~Dehghanian$^\textrm{\scriptsize 3}$,
I.~Deigaard$^\textrm{\scriptsize 109}$,
M.~Del~Gaudio$^\textrm{\scriptsize 40a,40b}$,
J.~Del~Peso$^\textrm{\scriptsize 85}$,
T.~Del~Prete$^\textrm{\scriptsize 126a,126b}$,
D.~Delgove$^\textrm{\scriptsize 119}$,
F.~Deliot$^\textrm{\scriptsize 138}$,
C.M.~Delitzsch$^\textrm{\scriptsize 52}$,
A.~Dell'Acqua$^\textrm{\scriptsize 32}$,
L.~Dell'Asta$^\textrm{\scriptsize 24}$,
M.~Dell'Orso$^\textrm{\scriptsize 126a,126b}$,
M.~Della~Pietra$^\textrm{\scriptsize 106a}$$^{,m}$,
D.~della~Volpe$^\textrm{\scriptsize 52}$,
M.~Delmastro$^\textrm{\scriptsize 5}$,
P.A.~Delsart$^\textrm{\scriptsize 58}$,
D.A.~DeMarco$^\textrm{\scriptsize 161}$,
S.~Demers$^\textrm{\scriptsize 179}$,
M.~Demichev$^\textrm{\scriptsize 68}$,
A.~Demilly$^\textrm{\scriptsize 83}$,
S.P.~Denisov$^\textrm{\scriptsize 132}$,
D.~Denysiuk$^\textrm{\scriptsize 138}$,
D.~Derendarz$^\textrm{\scriptsize 42}$,
J.E.~Derkaoui$^\textrm{\scriptsize 137d}$,
F.~Derue$^\textrm{\scriptsize 83}$,
P.~Dervan$^\textrm{\scriptsize 77}$,
K.~Desch$^\textrm{\scriptsize 23}$,
C.~Deterre$^\textrm{\scriptsize 45}$,
K.~Dette$^\textrm{\scriptsize 46}$,
P.O.~Deviveiros$^\textrm{\scriptsize 32}$,
A.~Dewhurst$^\textrm{\scriptsize 133}$,
S.~Dhaliwal$^\textrm{\scriptsize 25}$,
A.~Di~Ciaccio$^\textrm{\scriptsize 135a,135b}$,
L.~Di~Ciaccio$^\textrm{\scriptsize 5}$,
W.K.~Di~Clemente$^\textrm{\scriptsize 124}$,
C.~Di~Donato$^\textrm{\scriptsize 106a,106b}$,
A.~Di~Girolamo$^\textrm{\scriptsize 32}$,
B.~Di~Girolamo$^\textrm{\scriptsize 32}$,
B.~Di~Micco$^\textrm{\scriptsize 136a,136b}$,
R.~Di~Nardo$^\textrm{\scriptsize 32}$,
K.F.~Di~Petrillo$^\textrm{\scriptsize 59}$,
A.~Di~Simone$^\textrm{\scriptsize 51}$,
R.~Di~Sipio$^\textrm{\scriptsize 161}$,
D.~Di~Valentino$^\textrm{\scriptsize 31}$,
C.~Diaconu$^\textrm{\scriptsize 88}$,
M.~Diamond$^\textrm{\scriptsize 161}$,
F.A.~Dias$^\textrm{\scriptsize 49}$,
M.A.~Diaz$^\textrm{\scriptsize 34a}$,
E.B.~Diehl$^\textrm{\scriptsize 92}$,
J.~Dietrich$^\textrm{\scriptsize 17}$,
S.~D\'iez~Cornell$^\textrm{\scriptsize 45}$,
A.~Dimitrievska$^\textrm{\scriptsize 14}$,
J.~Dingfelder$^\textrm{\scriptsize 23}$,
P.~Dita$^\textrm{\scriptsize 28b}$,
S.~Dita$^\textrm{\scriptsize 28b}$,
F.~Dittus$^\textrm{\scriptsize 32}$,
F.~Djama$^\textrm{\scriptsize 88}$,
T.~Djobava$^\textrm{\scriptsize 54b}$,
J.I.~Djuvsland$^\textrm{\scriptsize 60a}$,
M.A.B.~do~Vale$^\textrm{\scriptsize 26c}$,
D.~Dobos$^\textrm{\scriptsize 32}$,
M.~Dobre$^\textrm{\scriptsize 28b}$,
C.~Doglioni$^\textrm{\scriptsize 84}$,
J.~Dolejsi$^\textrm{\scriptsize 131}$,
Z.~Dolezal$^\textrm{\scriptsize 131}$,
M.~Donadelli$^\textrm{\scriptsize 26d}$,
S.~Donati$^\textrm{\scriptsize 126a,126b}$,
P.~Dondero$^\textrm{\scriptsize 123a,123b}$,
J.~Donini$^\textrm{\scriptsize 37}$,
J.~Dopke$^\textrm{\scriptsize 133}$,
A.~Doria$^\textrm{\scriptsize 106a}$,
M.T.~Dova$^\textrm{\scriptsize 74}$,
A.T.~Doyle$^\textrm{\scriptsize 56}$,
E.~Drechsler$^\textrm{\scriptsize 57}$,
M.~Dris$^\textrm{\scriptsize 10}$,
Y.~Du$^\textrm{\scriptsize 36b}$,
J.~Duarte-Campderros$^\textrm{\scriptsize 155}$,
E.~Duchovni$^\textrm{\scriptsize 175}$,
G.~Duckeck$^\textrm{\scriptsize 102}$,
O.A.~Ducu$^\textrm{\scriptsize 97}$$^{,o}$,
D.~Duda$^\textrm{\scriptsize 109}$,
A.~Dudarev$^\textrm{\scriptsize 32}$,
A.Chr.~Dudder$^\textrm{\scriptsize 86}$,
E.M.~Duffield$^\textrm{\scriptsize 16}$,
L.~Duflot$^\textrm{\scriptsize 119}$,
M.~D\"uhrssen$^\textrm{\scriptsize 32}$,
M.~Dumancic$^\textrm{\scriptsize 175}$,
A.K.~Duncan$^\textrm{\scriptsize 56}$,
M.~Dunford$^\textrm{\scriptsize 60a}$,
H.~Duran~Yildiz$^\textrm{\scriptsize 4a}$,
M.~D\"uren$^\textrm{\scriptsize 55}$,
A.~Durglishvili$^\textrm{\scriptsize 54b}$,
D.~Duschinger$^\textrm{\scriptsize 47}$,
B.~Dutta$^\textrm{\scriptsize 45}$,
M.~Dyndal$^\textrm{\scriptsize 45}$,
C.~Eckardt$^\textrm{\scriptsize 45}$,
K.M.~Ecker$^\textrm{\scriptsize 103}$,
R.C.~Edgar$^\textrm{\scriptsize 92}$,
T.~Eifert$^\textrm{\scriptsize 32}$,
G.~Eigen$^\textrm{\scriptsize 15}$,
K.~Einsweiler$^\textrm{\scriptsize 16}$,
T.~Ekelof$^\textrm{\scriptsize 168}$,
M.~El~Kacimi$^\textrm{\scriptsize 137c}$,
V.~Ellajosyula$^\textrm{\scriptsize 88}$,
M.~Ellert$^\textrm{\scriptsize 168}$,
S.~Elles$^\textrm{\scriptsize 5}$,
F.~Ellinghaus$^\textrm{\scriptsize 178}$,
A.A.~Elliot$^\textrm{\scriptsize 172}$,
N.~Ellis$^\textrm{\scriptsize 32}$,
J.~Elmsheuser$^\textrm{\scriptsize 27}$,
M.~Elsing$^\textrm{\scriptsize 32}$,
D.~Emeliyanov$^\textrm{\scriptsize 133}$,
Y.~Enari$^\textrm{\scriptsize 157}$,
O.C.~Endner$^\textrm{\scriptsize 86}$,
J.S.~Ennis$^\textrm{\scriptsize 173}$,
J.~Erdmann$^\textrm{\scriptsize 46}$,
A.~Ereditato$^\textrm{\scriptsize 18}$,
G.~Ernis$^\textrm{\scriptsize 178}$,
J.~Ernst$^\textrm{\scriptsize 2}$,
M.~Ernst$^\textrm{\scriptsize 27}$,
S.~Errede$^\textrm{\scriptsize 169}$,
E.~Ertel$^\textrm{\scriptsize 86}$,
M.~Escalier$^\textrm{\scriptsize 119}$,
H.~Esch$^\textrm{\scriptsize 46}$,
C.~Escobar$^\textrm{\scriptsize 127}$,
B.~Esposito$^\textrm{\scriptsize 50}$,
A.I.~Etienvre$^\textrm{\scriptsize 138}$,
E.~Etzion$^\textrm{\scriptsize 155}$,
H.~Evans$^\textrm{\scriptsize 64}$,
A.~Ezhilov$^\textrm{\scriptsize 125}$,
M.~Ezzi$^\textrm{\scriptsize 137e}$,
F.~Fabbri$^\textrm{\scriptsize 22a,22b}$,
L.~Fabbri$^\textrm{\scriptsize 22a,22b}$,
G.~Facini$^\textrm{\scriptsize 33}$,
R.M.~Fakhrutdinov$^\textrm{\scriptsize 132}$,
S.~Falciano$^\textrm{\scriptsize 134a}$,
R.J.~Falla$^\textrm{\scriptsize 81}$,
J.~Faltova$^\textrm{\scriptsize 32}$,
Y.~Fang$^\textrm{\scriptsize 35a}$,
M.~Fanti$^\textrm{\scriptsize 94a,94b}$,
A.~Farbin$^\textrm{\scriptsize 8}$,
A.~Farilla$^\textrm{\scriptsize 136a}$,
C.~Farina$^\textrm{\scriptsize 127}$,
E.M.~Farina$^\textrm{\scriptsize 123a,123b}$,
T.~Farooque$^\textrm{\scriptsize 93}$,
S.~Farrell$^\textrm{\scriptsize 16}$,
S.M.~Farrington$^\textrm{\scriptsize 173}$,
P.~Farthouat$^\textrm{\scriptsize 32}$,
F.~Fassi$^\textrm{\scriptsize 137e}$,
P.~Fassnacht$^\textrm{\scriptsize 32}$,
D.~Fassouliotis$^\textrm{\scriptsize 9}$,
M.~Faucci~Giannelli$^\textrm{\scriptsize 80}$,
A.~Favareto$^\textrm{\scriptsize 53a,53b}$,
W.J.~Fawcett$^\textrm{\scriptsize 122}$,
L.~Fayard$^\textrm{\scriptsize 119}$,
O.L.~Fedin$^\textrm{\scriptsize 125}$$^{,p}$,
W.~Fedorko$^\textrm{\scriptsize 171}$,
S.~Feigl$^\textrm{\scriptsize 121}$,
L.~Feligioni$^\textrm{\scriptsize 88}$,
C.~Feng$^\textrm{\scriptsize 36b}$,
E.J.~Feng$^\textrm{\scriptsize 32}$,
H.~Feng$^\textrm{\scriptsize 92}$,
A.B.~Fenyuk$^\textrm{\scriptsize 132}$,
L.~Feremenga$^\textrm{\scriptsize 8}$,
P.~Fernandez~Martinez$^\textrm{\scriptsize 170}$,
S.~Fernandez~Perez$^\textrm{\scriptsize 13}$,
J.~Ferrando$^\textrm{\scriptsize 45}$,
A.~Ferrari$^\textrm{\scriptsize 168}$,
P.~Ferrari$^\textrm{\scriptsize 109}$,
R.~Ferrari$^\textrm{\scriptsize 123a}$,
D.E.~Ferreira~de~Lima$^\textrm{\scriptsize 60b}$,
A.~Ferrer$^\textrm{\scriptsize 170}$,
D.~Ferrere$^\textrm{\scriptsize 52}$,
C.~Ferretti$^\textrm{\scriptsize 92}$,
F.~Fiedler$^\textrm{\scriptsize 86}$,
A.~Filip\v{c}i\v{c}$^\textrm{\scriptsize 78}$,
M.~Filipuzzi$^\textrm{\scriptsize 45}$,
F.~Filthaut$^\textrm{\scriptsize 108}$,
M.~Fincke-Keeler$^\textrm{\scriptsize 172}$,
K.D.~Finelli$^\textrm{\scriptsize 152}$,
M.C.N.~Fiolhais$^\textrm{\scriptsize 128a,128c}$,
L.~Fiorini$^\textrm{\scriptsize 170}$,
A.~Fischer$^\textrm{\scriptsize 2}$,
C.~Fischer$^\textrm{\scriptsize 13}$,
J.~Fischer$^\textrm{\scriptsize 178}$,
W.C.~Fisher$^\textrm{\scriptsize 93}$,
N.~Flaschel$^\textrm{\scriptsize 45}$,
I.~Fleck$^\textrm{\scriptsize 143}$,
P.~Fleischmann$^\textrm{\scriptsize 92}$,
G.T.~Fletcher$^\textrm{\scriptsize 141}$,
R.R.M.~Fletcher$^\textrm{\scriptsize 124}$,
T.~Flick$^\textrm{\scriptsize 178}$,
B.M.~Flierl$^\textrm{\scriptsize 102}$,
L.R.~Flores~Castillo$^\textrm{\scriptsize 62a}$,
M.J.~Flowerdew$^\textrm{\scriptsize 103}$,
G.T.~Forcolin$^\textrm{\scriptsize 87}$,
A.~Formica$^\textrm{\scriptsize 138}$,
A.~Forti$^\textrm{\scriptsize 87}$,
A.G.~Foster$^\textrm{\scriptsize 19}$,
D.~Fournier$^\textrm{\scriptsize 119}$,
H.~Fox$^\textrm{\scriptsize 75}$,
S.~Fracchia$^\textrm{\scriptsize 13}$,
P.~Francavilla$^\textrm{\scriptsize 83}$,
M.~Franchini$^\textrm{\scriptsize 22a,22b}$,
D.~Francis$^\textrm{\scriptsize 32}$,
L.~Franconi$^\textrm{\scriptsize 121}$,
M.~Franklin$^\textrm{\scriptsize 59}$,
M.~Frate$^\textrm{\scriptsize 166}$,
M.~Fraternali$^\textrm{\scriptsize 123a,123b}$,
D.~Freeborn$^\textrm{\scriptsize 81}$,
S.M.~Fressard-Batraneanu$^\textrm{\scriptsize 32}$,
D.~Froidevaux$^\textrm{\scriptsize 32}$,
J.A.~Frost$^\textrm{\scriptsize 122}$,
C.~Fukunaga$^\textrm{\scriptsize 158}$,
E.~Fullana~Torregrosa$^\textrm{\scriptsize 86}$,
T.~Fusayasu$^\textrm{\scriptsize 104}$,
J.~Fuster$^\textrm{\scriptsize 170}$,
C.~Gabaldon$^\textrm{\scriptsize 58}$,
O.~Gabizon$^\textrm{\scriptsize 154}$,
A.~Gabrielli$^\textrm{\scriptsize 22a,22b}$,
A.~Gabrielli$^\textrm{\scriptsize 16}$,
G.P.~Gach$^\textrm{\scriptsize 41a}$,
S.~Gadatsch$^\textrm{\scriptsize 32}$,
G.~Gagliardi$^\textrm{\scriptsize 53a,53b}$,
L.G.~Gagnon$^\textrm{\scriptsize 97}$,
P.~Gagnon$^\textrm{\scriptsize 64}$,
C.~Galea$^\textrm{\scriptsize 108}$,
B.~Galhardo$^\textrm{\scriptsize 128a,128c}$,
E.J.~Gallas$^\textrm{\scriptsize 122}$,
B.J.~Gallop$^\textrm{\scriptsize 133}$,
P.~Gallus$^\textrm{\scriptsize 130}$,
G.~Galster$^\textrm{\scriptsize 39}$,
K.K.~Gan$^\textrm{\scriptsize 113}$,
S.~Ganguly$^\textrm{\scriptsize 37}$,
J.~Gao$^\textrm{\scriptsize 36a}$,
Y.~Gao$^\textrm{\scriptsize 77}$,
Y.S.~Gao$^\textrm{\scriptsize 145}$$^{,g}$,
F.M.~Garay~Walls$^\textrm{\scriptsize 49}$,
C.~Garc\'ia$^\textrm{\scriptsize 170}$,
J.E.~Garc\'ia~Navarro$^\textrm{\scriptsize 170}$,
M.~Garcia-Sciveres$^\textrm{\scriptsize 16}$,
R.W.~Gardner$^\textrm{\scriptsize 33}$,
N.~Garelli$^\textrm{\scriptsize 145}$,
V.~Garonne$^\textrm{\scriptsize 121}$,
A.~Gascon~Bravo$^\textrm{\scriptsize 45}$,
K.~Gasnikova$^\textrm{\scriptsize 45}$,
C.~Gatti$^\textrm{\scriptsize 50}$,
A.~Gaudiello$^\textrm{\scriptsize 53a,53b}$,
G.~Gaudio$^\textrm{\scriptsize 123a}$,
L.~Gauthier$^\textrm{\scriptsize 97}$,
I.L.~Gavrilenko$^\textrm{\scriptsize 98}$,
C.~Gay$^\textrm{\scriptsize 171}$,
G.~Gaycken$^\textrm{\scriptsize 23}$,
E.N.~Gazis$^\textrm{\scriptsize 10}$,
C.N.P.~Gee$^\textrm{\scriptsize 133}$,
Ch.~Geich-Gimbel$^\textrm{\scriptsize 23}$,
M.~Geisen$^\textrm{\scriptsize 86}$,
M.P.~Geisler$^\textrm{\scriptsize 60a}$,
K.~Gellerstedt$^\textrm{\scriptsize 148a,148b}$,
C.~Gemme$^\textrm{\scriptsize 53a}$,
M.H.~Genest$^\textrm{\scriptsize 58}$,
C.~Geng$^\textrm{\scriptsize 36a}$$^{,q}$,
S.~Gentile$^\textrm{\scriptsize 134a,134b}$,
C.~Gentsos$^\textrm{\scriptsize 156}$,
S.~George$^\textrm{\scriptsize 80}$,
D.~Gerbaudo$^\textrm{\scriptsize 13}$,
A.~Gershon$^\textrm{\scriptsize 155}$,
S.~Ghasemi$^\textrm{\scriptsize 143}$,
M.~Ghneimat$^\textrm{\scriptsize 23}$,
B.~Giacobbe$^\textrm{\scriptsize 22a}$,
S.~Giagu$^\textrm{\scriptsize 134a,134b}$,
P.~Giannetti$^\textrm{\scriptsize 126a,126b}$,
S.M.~Gibson$^\textrm{\scriptsize 80}$,
M.~Gignac$^\textrm{\scriptsize 171}$,
M.~Gilchriese$^\textrm{\scriptsize 16}$,
T.P.S.~Gillam$^\textrm{\scriptsize 30}$,
D.~Gillberg$^\textrm{\scriptsize 31}$,
G.~Gilles$^\textrm{\scriptsize 178}$,
D.M.~Gingrich$^\textrm{\scriptsize 3}$$^{,d}$,
N.~Giokaris$^\textrm{\scriptsize 9}$$^{,*}$,
M.P.~Giordani$^\textrm{\scriptsize 167a,167c}$,
F.M.~Giorgi$^\textrm{\scriptsize 22a}$,
P.F.~Giraud$^\textrm{\scriptsize 138}$,
P.~Giromini$^\textrm{\scriptsize 59}$,
D.~Giugni$^\textrm{\scriptsize 94a}$,
F.~Giuli$^\textrm{\scriptsize 122}$,
C.~Giuliani$^\textrm{\scriptsize 103}$,
M.~Giulini$^\textrm{\scriptsize 60b}$,
B.K.~Gjelsten$^\textrm{\scriptsize 121}$,
S.~Gkaitatzis$^\textrm{\scriptsize 156}$,
I.~Gkialas$^\textrm{\scriptsize 9}$,
E.L.~Gkougkousis$^\textrm{\scriptsize 139}$,
L.K.~Gladilin$^\textrm{\scriptsize 101}$,
C.~Glasman$^\textrm{\scriptsize 85}$,
J.~Glatzer$^\textrm{\scriptsize 13}$,
P.C.F.~Glaysher$^\textrm{\scriptsize 49}$,
A.~Glazov$^\textrm{\scriptsize 45}$,
M.~Goblirsch-Kolb$^\textrm{\scriptsize 25}$,
J.~Godlewski$^\textrm{\scriptsize 42}$,
S.~Goldfarb$^\textrm{\scriptsize 91}$,
T.~Golling$^\textrm{\scriptsize 52}$,
D.~Golubkov$^\textrm{\scriptsize 132}$,
A.~Gomes$^\textrm{\scriptsize 128a,128b,128d}$,
R.~Gon\c{c}alo$^\textrm{\scriptsize 128a}$,
R.~Goncalves~Gama$^\textrm{\scriptsize 26a}$,
J.~Goncalves~Pinto~Firmino~Da~Costa$^\textrm{\scriptsize 138}$,
G.~Gonella$^\textrm{\scriptsize 51}$,
L.~Gonella$^\textrm{\scriptsize 19}$,
A.~Gongadze$^\textrm{\scriptsize 68}$,
S.~Gonz\'alez~de~la~Hoz$^\textrm{\scriptsize 170}$,
S.~Gonzalez-Sevilla$^\textrm{\scriptsize 52}$,
L.~Goossens$^\textrm{\scriptsize 32}$,
P.A.~Gorbounov$^\textrm{\scriptsize 99}$,
H.A.~Gordon$^\textrm{\scriptsize 27}$,
I.~Gorelov$^\textrm{\scriptsize 107}$,
B.~Gorini$^\textrm{\scriptsize 32}$,
E.~Gorini$^\textrm{\scriptsize 76a,76b}$,
A.~Gori\v{s}ek$^\textrm{\scriptsize 78}$,
A.T.~Goshaw$^\textrm{\scriptsize 48}$,
C.~G\"ossling$^\textrm{\scriptsize 46}$,
M.I.~Gostkin$^\textrm{\scriptsize 68}$,
C.R.~Goudet$^\textrm{\scriptsize 119}$,
D.~Goujdami$^\textrm{\scriptsize 137c}$,
A.G.~Goussiou$^\textrm{\scriptsize 140}$,
N.~Govender$^\textrm{\scriptsize 147b}$$^{,r}$,
E.~Gozani$^\textrm{\scriptsize 154}$,
L.~Graber$^\textrm{\scriptsize 57}$,
I.~Grabowska-Bold$^\textrm{\scriptsize 41a}$,
P.O.J.~Gradin$^\textrm{\scriptsize 58}$,
P.~Grafstr\"om$^\textrm{\scriptsize 22a,22b}$,
J.~Gramling$^\textrm{\scriptsize 52}$,
E.~Gramstad$^\textrm{\scriptsize 121}$,
S.~Grancagnolo$^\textrm{\scriptsize 17}$,
V.~Gratchev$^\textrm{\scriptsize 125}$,
P.M.~Gravila$^\textrm{\scriptsize 28e}$,
H.M.~Gray$^\textrm{\scriptsize 32}$,
E.~Graziani$^\textrm{\scriptsize 136a}$,
Z.D.~Greenwood$^\textrm{\scriptsize 82}$$^{,s}$,
C.~Grefe$^\textrm{\scriptsize 23}$,
K.~Gregersen$^\textrm{\scriptsize 81}$,
I.M.~Gregor$^\textrm{\scriptsize 45}$,
P.~Grenier$^\textrm{\scriptsize 145}$,
K.~Grevtsov$^\textrm{\scriptsize 5}$,
J.~Griffiths$^\textrm{\scriptsize 8}$,
A.A.~Grillo$^\textrm{\scriptsize 139}$,
K.~Grimm$^\textrm{\scriptsize 75}$,
S.~Grinstein$^\textrm{\scriptsize 13}$$^{,t}$,
Ph.~Gris$^\textrm{\scriptsize 37}$,
J.-F.~Grivaz$^\textrm{\scriptsize 119}$,
S.~Groh$^\textrm{\scriptsize 86}$,
E.~Gross$^\textrm{\scriptsize 175}$,
J.~Grosse-Knetter$^\textrm{\scriptsize 57}$,
G.C.~Grossi$^\textrm{\scriptsize 82}$,
Z.J.~Grout$^\textrm{\scriptsize 81}$,
L.~Guan$^\textrm{\scriptsize 92}$,
W.~Guan$^\textrm{\scriptsize 176}$,
J.~Guenther$^\textrm{\scriptsize 65}$,
F.~Guescini$^\textrm{\scriptsize 163a}$,
D.~Guest$^\textrm{\scriptsize 166}$,
O.~Gueta$^\textrm{\scriptsize 155}$,
B.~Gui$^\textrm{\scriptsize 113}$,
E.~Guido$^\textrm{\scriptsize 53a,53b}$,
T.~Guillemin$^\textrm{\scriptsize 5}$,
S.~Guindon$^\textrm{\scriptsize 2}$,
U.~Gul$^\textrm{\scriptsize 56}$,
C.~Gumpert$^\textrm{\scriptsize 32}$,
J.~Guo$^\textrm{\scriptsize 36c}$,
W.~Guo$^\textrm{\scriptsize 92}$,
Y.~Guo$^\textrm{\scriptsize 36a}$,
R.~Gupta$^\textrm{\scriptsize 43}$,
S.~Gupta$^\textrm{\scriptsize 122}$,
G.~Gustavino$^\textrm{\scriptsize 134a,134b}$,
P.~Gutierrez$^\textrm{\scriptsize 115}$,
N.G.~Gutierrez~Ortiz$^\textrm{\scriptsize 81}$,
C.~Gutschow$^\textrm{\scriptsize 81}$,
C.~Guyot$^\textrm{\scriptsize 138}$,
C.~Gwenlan$^\textrm{\scriptsize 122}$,
C.B.~Gwilliam$^\textrm{\scriptsize 77}$,
A.~Haas$^\textrm{\scriptsize 112}$,
C.~Haber$^\textrm{\scriptsize 16}$,
H.K.~Hadavand$^\textrm{\scriptsize 8}$,
N.~Haddad$^\textrm{\scriptsize 137e}$,
A.~Hadef$^\textrm{\scriptsize 88}$,
S.~Hageb\"ock$^\textrm{\scriptsize 23}$,
M.~Hagihara$^\textrm{\scriptsize 164}$,
H.~Hakobyan$^\textrm{\scriptsize 180}$$^{,*}$,
M.~Haleem$^\textrm{\scriptsize 45}$,
J.~Haley$^\textrm{\scriptsize 116}$,
G.~Halladjian$^\textrm{\scriptsize 93}$,
G.D.~Hallewell$^\textrm{\scriptsize 88}$,
K.~Hamacher$^\textrm{\scriptsize 178}$,
P.~Hamal$^\textrm{\scriptsize 117}$,
K.~Hamano$^\textrm{\scriptsize 172}$,
A.~Hamilton$^\textrm{\scriptsize 147a}$,
G.N.~Hamity$^\textrm{\scriptsize 141}$,
P.G.~Hamnett$^\textrm{\scriptsize 45}$,
L.~Han$^\textrm{\scriptsize 36a}$,
S.~Han$^\textrm{\scriptsize 35a}$,
K.~Hanagaki$^\textrm{\scriptsize 69}$$^{,u}$,
K.~Hanawa$^\textrm{\scriptsize 157}$,
M.~Hance$^\textrm{\scriptsize 139}$,
B.~Haney$^\textrm{\scriptsize 124}$,
P.~Hanke$^\textrm{\scriptsize 60a}$,
R.~Hanna$^\textrm{\scriptsize 138}$,
J.B.~Hansen$^\textrm{\scriptsize 39}$,
J.D.~Hansen$^\textrm{\scriptsize 39}$,
M.C.~Hansen$^\textrm{\scriptsize 23}$,
P.H.~Hansen$^\textrm{\scriptsize 39}$,
K.~Hara$^\textrm{\scriptsize 164}$,
A.S.~Hard$^\textrm{\scriptsize 176}$,
T.~Harenberg$^\textrm{\scriptsize 178}$,
F.~Hariri$^\textrm{\scriptsize 119}$,
S.~Harkusha$^\textrm{\scriptsize 95}$,
R.D.~Harrington$^\textrm{\scriptsize 49}$,
P.F.~Harrison$^\textrm{\scriptsize 173}$,
F.~Hartjes$^\textrm{\scriptsize 109}$,
N.M.~Hartmann$^\textrm{\scriptsize 102}$,
M.~Hasegawa$^\textrm{\scriptsize 70}$,
Y.~Hasegawa$^\textrm{\scriptsize 142}$,
A.~Hasib$^\textrm{\scriptsize 49}$,
S.~Hassani$^\textrm{\scriptsize 138}$,
S.~Haug$^\textrm{\scriptsize 18}$,
R.~Hauser$^\textrm{\scriptsize 93}$,
L.~Hauswald$^\textrm{\scriptsize 47}$,
L.B.~Havener$^\textrm{\scriptsize 38}$,
M.~Havranek$^\textrm{\scriptsize 130}$,
C.M.~Hawkes$^\textrm{\scriptsize 19}$,
R.J.~Hawkings$^\textrm{\scriptsize 32}$,
D.~Hayakawa$^\textrm{\scriptsize 159}$,
D.~Hayden$^\textrm{\scriptsize 93}$,
C.P.~Hays$^\textrm{\scriptsize 122}$,
J.M.~Hays$^\textrm{\scriptsize 79}$,
H.S.~Hayward$^\textrm{\scriptsize 77}$,
S.J.~Haywood$^\textrm{\scriptsize 133}$,
S.J.~Head$^\textrm{\scriptsize 19}$,
T.~Heck$^\textrm{\scriptsize 86}$,
V.~Hedberg$^\textrm{\scriptsize 84}$,
L.~Heelan$^\textrm{\scriptsize 8}$,
S.~Heim$^\textrm{\scriptsize 45}$,
T.~Heim$^\textrm{\scriptsize 16}$,
B.~Heinemann$^\textrm{\scriptsize 45}$$^{,v}$,
J.J.~Heinrich$^\textrm{\scriptsize 102}$,
L.~Heinrich$^\textrm{\scriptsize 112}$,
C.~Heinz$^\textrm{\scriptsize 55}$,
J.~Hejbal$^\textrm{\scriptsize 129}$,
L.~Helary$^\textrm{\scriptsize 32}$,
S.~Hellman$^\textrm{\scriptsize 148a,148b}$,
C.~Helsens$^\textrm{\scriptsize 32}$,
J.~Henderson$^\textrm{\scriptsize 122}$,
R.C.W.~Henderson$^\textrm{\scriptsize 75}$,
Y.~Heng$^\textrm{\scriptsize 176}$,
S.~Henkelmann$^\textrm{\scriptsize 171}$,
A.M.~Henriques~Correia$^\textrm{\scriptsize 32}$,
S.~Henrot-Versille$^\textrm{\scriptsize 119}$,
G.H.~Herbert$^\textrm{\scriptsize 17}$,
H.~Herde$^\textrm{\scriptsize 25}$,
V.~Herget$^\textrm{\scriptsize 177}$,
Y.~Hern\'andez~Jim\'enez$^\textrm{\scriptsize 147c}$,
G.~Herten$^\textrm{\scriptsize 51}$,
R.~Hertenberger$^\textrm{\scriptsize 102}$,
L.~Hervas$^\textrm{\scriptsize 32}$,
T.C.~Herwig$^\textrm{\scriptsize 124}$,
G.G.~Hesketh$^\textrm{\scriptsize 81}$,
N.P.~Hessey$^\textrm{\scriptsize 109}$,
J.W.~Hetherly$^\textrm{\scriptsize 43}$,
E.~Hig\'on-Rodriguez$^\textrm{\scriptsize 170}$,
E.~Hill$^\textrm{\scriptsize 172}$,
J.C.~Hill$^\textrm{\scriptsize 30}$,
K.H.~Hiller$^\textrm{\scriptsize 45}$,
S.J.~Hillier$^\textrm{\scriptsize 19}$,
I.~Hinchliffe$^\textrm{\scriptsize 16}$,
E.~Hines$^\textrm{\scriptsize 124}$,
M.~Hirose$^\textrm{\scriptsize 51}$,
D.~Hirschbuehl$^\textrm{\scriptsize 178}$,
O.~Hladik$^\textrm{\scriptsize 129}$,
X.~Hoad$^\textrm{\scriptsize 49}$,
J.~Hobbs$^\textrm{\scriptsize 150}$,
N.~Hod$^\textrm{\scriptsize 163a}$,
M.C.~Hodgkinson$^\textrm{\scriptsize 141}$,
P.~Hodgson$^\textrm{\scriptsize 141}$,
A.~Hoecker$^\textrm{\scriptsize 32}$,
M.R.~Hoeferkamp$^\textrm{\scriptsize 107}$,
F.~Hoenig$^\textrm{\scriptsize 102}$,
D.~Hohn$^\textrm{\scriptsize 23}$,
T.R.~Holmes$^\textrm{\scriptsize 16}$,
M.~Homann$^\textrm{\scriptsize 46}$,
S.~Honda$^\textrm{\scriptsize 164}$,
T.~Honda$^\textrm{\scriptsize 69}$,
T.M.~Hong$^\textrm{\scriptsize 127}$,
B.H.~Hooberman$^\textrm{\scriptsize 169}$,
W.H.~Hopkins$^\textrm{\scriptsize 118}$,
Y.~Horii$^\textrm{\scriptsize 105}$,
A.J.~Horton$^\textrm{\scriptsize 144}$,
J-Y.~Hostachy$^\textrm{\scriptsize 58}$,
S.~Hou$^\textrm{\scriptsize 153}$,
A.~Hoummada$^\textrm{\scriptsize 137a}$,
J.~Howarth$^\textrm{\scriptsize 45}$,
J.~Hoya$^\textrm{\scriptsize 74}$,
M.~Hrabovsky$^\textrm{\scriptsize 117}$,
I.~Hristova$^\textrm{\scriptsize 17}$,
J.~Hrivnac$^\textrm{\scriptsize 119}$,
T.~Hryn'ova$^\textrm{\scriptsize 5}$,
A.~Hrynevich$^\textrm{\scriptsize 96}$,
P.J.~Hsu$^\textrm{\scriptsize 63}$,
S.-C.~Hsu$^\textrm{\scriptsize 140}$,
Q.~Hu$^\textrm{\scriptsize 36a}$,
S.~Hu$^\textrm{\scriptsize 36c}$,
Y.~Huang$^\textrm{\scriptsize 35a}$,
Z.~Hubacek$^\textrm{\scriptsize 130}$,
F.~Hubaut$^\textrm{\scriptsize 88}$,
F.~Huegging$^\textrm{\scriptsize 23}$,
T.B.~Huffman$^\textrm{\scriptsize 122}$,
E.W.~Hughes$^\textrm{\scriptsize 38}$,
G.~Hughes$^\textrm{\scriptsize 75}$,
M.~Huhtinen$^\textrm{\scriptsize 32}$,
P.~Huo$^\textrm{\scriptsize 150}$,
N.~Huseynov$^\textrm{\scriptsize 68}$$^{,b}$,
J.~Huston$^\textrm{\scriptsize 93}$,
J.~Huth$^\textrm{\scriptsize 59}$,
G.~Iacobucci$^\textrm{\scriptsize 52}$,
G.~Iakovidis$^\textrm{\scriptsize 27}$,
I.~Ibragimov$^\textrm{\scriptsize 143}$,
L.~Iconomidou-Fayard$^\textrm{\scriptsize 119}$,
Z.~Idrissi$^\textrm{\scriptsize 137e}$,
P.~Iengo$^\textrm{\scriptsize 32}$,
O.~Igonkina$^\textrm{\scriptsize 109}$$^{,w}$,
T.~Iizawa$^\textrm{\scriptsize 174}$,
Y.~Ikegami$^\textrm{\scriptsize 69}$,
M.~Ikeno$^\textrm{\scriptsize 69}$,
Y.~Ilchenko$^\textrm{\scriptsize 11}$$^{,x}$,
D.~Iliadis$^\textrm{\scriptsize 156}$,
N.~Ilic$^\textrm{\scriptsize 145}$,
G.~Introzzi$^\textrm{\scriptsize 123a,123b}$,
P.~Ioannou$^\textrm{\scriptsize 9}$$^{,*}$,
M.~Iodice$^\textrm{\scriptsize 136a}$,
K.~Iordanidou$^\textrm{\scriptsize 38}$,
V.~Ippolito$^\textrm{\scriptsize 59}$,
N.~Ishijima$^\textrm{\scriptsize 120}$,
M.~Ishino$^\textrm{\scriptsize 157}$,
M.~Ishitsuka$^\textrm{\scriptsize 159}$,
C.~Issever$^\textrm{\scriptsize 122}$,
S.~Istin$^\textrm{\scriptsize 20a}$,
F.~Ito$^\textrm{\scriptsize 164}$,
J.M.~Iturbe~Ponce$^\textrm{\scriptsize 87}$,
R.~Iuppa$^\textrm{\scriptsize 162a,162b}$,
H.~Iwasaki$^\textrm{\scriptsize 69}$,
J.M.~Izen$^\textrm{\scriptsize 44}$,
V.~Izzo$^\textrm{\scriptsize 106a}$,
S.~Jabbar$^\textrm{\scriptsize 3}$,
P.~Jackson$^\textrm{\scriptsize 1}$,
V.~Jain$^\textrm{\scriptsize 2}$,
K.B.~Jakobi$^\textrm{\scriptsize 86}$,
K.~Jakobs$^\textrm{\scriptsize 51}$,
S.~Jakobsen$^\textrm{\scriptsize 32}$,
T.~Jakoubek$^\textrm{\scriptsize 129}$,
D.O.~Jamin$^\textrm{\scriptsize 116}$,
D.K.~Jana$^\textrm{\scriptsize 82}$,
R.~Jansky$^\textrm{\scriptsize 65}$,
J.~Janssen$^\textrm{\scriptsize 23}$,
M.~Janus$^\textrm{\scriptsize 57}$,
P.A.~Janus$^\textrm{\scriptsize 41a}$,
G.~Jarlskog$^\textrm{\scriptsize 84}$,
N.~Javadov$^\textrm{\scriptsize 68}$$^{,b}$,
T.~Jav\r{u}rek$^\textrm{\scriptsize 51}$,
M.~Javurkova$^\textrm{\scriptsize 51}$,
F.~Jeanneau$^\textrm{\scriptsize 138}$,
L.~Jeanty$^\textrm{\scriptsize 16}$,
J.~Jejelava$^\textrm{\scriptsize 54a}$$^{,y}$,
P.~Jenni$^\textrm{\scriptsize 51}$$^{,z}$,
C.~Jeske$^\textrm{\scriptsize 173}$,
S.~J\'ez\'equel$^\textrm{\scriptsize 5}$,
H.~Ji$^\textrm{\scriptsize 176}$,
J.~Jia$^\textrm{\scriptsize 150}$,
H.~Jiang$^\textrm{\scriptsize 67}$,
Y.~Jiang$^\textrm{\scriptsize 36a}$,
Z.~Jiang$^\textrm{\scriptsize 145}$,
S.~Jiggins$^\textrm{\scriptsize 81}$,
J.~Jimenez~Pena$^\textrm{\scriptsize 170}$,
S.~Jin$^\textrm{\scriptsize 35a}$,
A.~Jinaru$^\textrm{\scriptsize 28b}$,
O.~Jinnouchi$^\textrm{\scriptsize 159}$,
H.~Jivan$^\textrm{\scriptsize 147c}$,
P.~Johansson$^\textrm{\scriptsize 141}$,
K.A.~Johns$^\textrm{\scriptsize 7}$,
C.A.~Johnson$^\textrm{\scriptsize 64}$,
W.J.~Johnson$^\textrm{\scriptsize 140}$,
K.~Jon-And$^\textrm{\scriptsize 148a,148b}$,
G.~Jones$^\textrm{\scriptsize 173}$,
R.W.L.~Jones$^\textrm{\scriptsize 75}$,
S.~Jones$^\textrm{\scriptsize 7}$,
T.J.~Jones$^\textrm{\scriptsize 77}$,
J.~Jongmanns$^\textrm{\scriptsize 60a}$,
P.M.~Jorge$^\textrm{\scriptsize 128a,128b}$,
J.~Jovicevic$^\textrm{\scriptsize 163a}$,
X.~Ju$^\textrm{\scriptsize 176}$,
A.~Juste~Rozas$^\textrm{\scriptsize 13}$$^{,t}$,
M.K.~K\"{o}hler$^\textrm{\scriptsize 175}$,
A.~Kaczmarska$^\textrm{\scriptsize 42}$,
M.~Kado$^\textrm{\scriptsize 119}$,
H.~Kagan$^\textrm{\scriptsize 113}$,
M.~Kagan$^\textrm{\scriptsize 145}$,
S.J.~Kahn$^\textrm{\scriptsize 88}$,
T.~Kaji$^\textrm{\scriptsize 174}$,
E.~Kajomovitz$^\textrm{\scriptsize 48}$,
C.W.~Kalderon$^\textrm{\scriptsize 84}$,
A.~Kaluza$^\textrm{\scriptsize 86}$,
S.~Kama$^\textrm{\scriptsize 43}$,
A.~Kamenshchikov$^\textrm{\scriptsize 132}$,
N.~Kanaya$^\textrm{\scriptsize 157}$,
S.~Kaneti$^\textrm{\scriptsize 30}$,
L.~Kanjir$^\textrm{\scriptsize 78}$,
V.A.~Kantserov$^\textrm{\scriptsize 100}$,
J.~Kanzaki$^\textrm{\scriptsize 69}$,
B.~Kaplan$^\textrm{\scriptsize 112}$,
L.S.~Kaplan$^\textrm{\scriptsize 176}$,
A.~Kapliy$^\textrm{\scriptsize 33}$,
D.~Kar$^\textrm{\scriptsize 147c}$,
K.~Karakostas$^\textrm{\scriptsize 10}$,
A.~Karamaoun$^\textrm{\scriptsize 3}$,
N.~Karastathis$^\textrm{\scriptsize 10}$,
M.J.~Kareem$^\textrm{\scriptsize 57}$,
E.~Karentzos$^\textrm{\scriptsize 10}$,
S.N.~Karpov$^\textrm{\scriptsize 68}$,
Z.M.~Karpova$^\textrm{\scriptsize 68}$,
K.~Karthik$^\textrm{\scriptsize 112}$,
V.~Kartvelishvili$^\textrm{\scriptsize 75}$,
A.N.~Karyukhin$^\textrm{\scriptsize 132}$,
K.~Kasahara$^\textrm{\scriptsize 164}$,
L.~Kashif$^\textrm{\scriptsize 176}$,
R.D.~Kass$^\textrm{\scriptsize 113}$,
A.~Kastanas$^\textrm{\scriptsize 149}$,
Y.~Kataoka$^\textrm{\scriptsize 157}$,
C.~Kato$^\textrm{\scriptsize 157}$,
A.~Katre$^\textrm{\scriptsize 52}$,
J.~Katzy$^\textrm{\scriptsize 45}$,
K.~Kawade$^\textrm{\scriptsize 105}$,
K.~Kawagoe$^\textrm{\scriptsize 73}$,
T.~Kawamoto$^\textrm{\scriptsize 157}$,
G.~Kawamura$^\textrm{\scriptsize 57}$,
V.F.~Kazanin$^\textrm{\scriptsize 111}$$^{,c}$,
R.~Keeler$^\textrm{\scriptsize 172}$,
R.~Kehoe$^\textrm{\scriptsize 43}$,
J.S.~Keller$^\textrm{\scriptsize 45}$,
J.J.~Kempster$^\textrm{\scriptsize 80}$,
H.~Keoshkerian$^\textrm{\scriptsize 161}$,
O.~Kepka$^\textrm{\scriptsize 129}$,
B.P.~Ker\v{s}evan$^\textrm{\scriptsize 78}$,
S.~Kersten$^\textrm{\scriptsize 178}$,
R.A.~Keyes$^\textrm{\scriptsize 90}$,
M.~Khader$^\textrm{\scriptsize 169}$,
F.~Khalil-zada$^\textrm{\scriptsize 12}$,
A.~Khanov$^\textrm{\scriptsize 116}$,
A.G.~Kharlamov$^\textrm{\scriptsize 111}$$^{,c}$,
T.~Kharlamova$^\textrm{\scriptsize 111}$$^{,c}$,
T.J.~Khoo$^\textrm{\scriptsize 52}$,
V.~Khovanskiy$^\textrm{\scriptsize 99}$,
E.~Khramov$^\textrm{\scriptsize 68}$,
J.~Khubua$^\textrm{\scriptsize 54b}$$^{,aa}$,
S.~Kido$^\textrm{\scriptsize 70}$,
C.R.~Kilby$^\textrm{\scriptsize 80}$,
H.Y.~Kim$^\textrm{\scriptsize 8}$,
S.H.~Kim$^\textrm{\scriptsize 164}$,
Y.K.~Kim$^\textrm{\scriptsize 33}$,
N.~Kimura$^\textrm{\scriptsize 156}$,
O.M.~Kind$^\textrm{\scriptsize 17}$,
B.T.~King$^\textrm{\scriptsize 77}$,
D.~Kirchmeier$^\textrm{\scriptsize 47}$,
J.~Kirk$^\textrm{\scriptsize 133}$,
A.E.~Kiryunin$^\textrm{\scriptsize 103}$,
T.~Kishimoto$^\textrm{\scriptsize 157}$,
D.~Kisielewska$^\textrm{\scriptsize 41a}$,
K.~Kiuchi$^\textrm{\scriptsize 164}$,
O.~Kivernyk$^\textrm{\scriptsize 138}$,
E.~Kladiva$^\textrm{\scriptsize 146b}$,
T.~Klapdor-kleingrothaus$^\textrm{\scriptsize 51}$,
M.H.~Klein$^\textrm{\scriptsize 38}$,
M.~Klein$^\textrm{\scriptsize 77}$,
U.~Klein$^\textrm{\scriptsize 77}$,
K.~Kleinknecht$^\textrm{\scriptsize 86}$,
P.~Klimek$^\textrm{\scriptsize 110}$,
A.~Klimentov$^\textrm{\scriptsize 27}$,
R.~Klingenberg$^\textrm{\scriptsize 46}$,
T.~Klioutchnikova$^\textrm{\scriptsize 32}$,
E.-E.~Kluge$^\textrm{\scriptsize 60a}$,
P.~Kluit$^\textrm{\scriptsize 109}$,
S.~Kluth$^\textrm{\scriptsize 103}$,
J.~Knapik$^\textrm{\scriptsize 42}$,
E.~Kneringer$^\textrm{\scriptsize 65}$,
E.B.F.G.~Knoops$^\textrm{\scriptsize 88}$,
A.~Knue$^\textrm{\scriptsize 103}$,
A.~Kobayashi$^\textrm{\scriptsize 157}$,
D.~Kobayashi$^\textrm{\scriptsize 159}$,
T.~Kobayashi$^\textrm{\scriptsize 157}$,
M.~Kobel$^\textrm{\scriptsize 47}$,
M.~Kocian$^\textrm{\scriptsize 145}$,
P.~Kodys$^\textrm{\scriptsize 131}$,
T.~Koffas$^\textrm{\scriptsize 31}$,
E.~Koffeman$^\textrm{\scriptsize 109}$,
N.M.~K\"ohler$^\textrm{\scriptsize 103}$,
T.~Koi$^\textrm{\scriptsize 145}$,
H.~Kolanoski$^\textrm{\scriptsize 17}$,
M.~Kolb$^\textrm{\scriptsize 60b}$,
I.~Koletsou$^\textrm{\scriptsize 5}$,
A.A.~Komar$^\textrm{\scriptsize 98}$$^{,*}$,
Y.~Komori$^\textrm{\scriptsize 157}$,
T.~Kondo$^\textrm{\scriptsize 69}$,
N.~Kondrashova$^\textrm{\scriptsize 36c}$,
K.~K\"oneke$^\textrm{\scriptsize 51}$,
A.C.~K\"onig$^\textrm{\scriptsize 108}$,
T.~Kono$^\textrm{\scriptsize 69}$$^{,ab}$,
R.~Konoplich$^\textrm{\scriptsize 112}$$^{,ac}$,
N.~Konstantinidis$^\textrm{\scriptsize 81}$,
R.~Kopeliansky$^\textrm{\scriptsize 64}$,
S.~Koperny$^\textrm{\scriptsize 41a}$,
A.K.~Kopp$^\textrm{\scriptsize 51}$,
K.~Korcyl$^\textrm{\scriptsize 42}$,
K.~Kordas$^\textrm{\scriptsize 156}$,
A.~Korn$^\textrm{\scriptsize 81}$,
A.A.~Korol$^\textrm{\scriptsize 111}$$^{,c}$,
I.~Korolkov$^\textrm{\scriptsize 13}$,
E.V.~Korolkova$^\textrm{\scriptsize 141}$,
O.~Kortner$^\textrm{\scriptsize 103}$,
S.~Kortner$^\textrm{\scriptsize 103}$,
T.~Kosek$^\textrm{\scriptsize 131}$,
V.V.~Kostyukhin$^\textrm{\scriptsize 23}$,
A.~Kotwal$^\textrm{\scriptsize 48}$,
A.~Koulouris$^\textrm{\scriptsize 10}$,
A.~Kourkoumeli-Charalampidi$^\textrm{\scriptsize 123a,123b}$,
C.~Kourkoumelis$^\textrm{\scriptsize 9}$,
V.~Kouskoura$^\textrm{\scriptsize 27}$,
A.B.~Kowalewska$^\textrm{\scriptsize 42}$,
R.~Kowalewski$^\textrm{\scriptsize 172}$,
T.Z.~Kowalski$^\textrm{\scriptsize 41a}$,
C.~Kozakai$^\textrm{\scriptsize 157}$,
W.~Kozanecki$^\textrm{\scriptsize 138}$,
A.S.~Kozhin$^\textrm{\scriptsize 132}$,
V.A.~Kramarenko$^\textrm{\scriptsize 101}$,
G.~Kramberger$^\textrm{\scriptsize 78}$,
D.~Krasnopevtsev$^\textrm{\scriptsize 100}$,
M.W.~Krasny$^\textrm{\scriptsize 83}$,
A.~Krasznahorkay$^\textrm{\scriptsize 32}$,
A.~Kravchenko$^\textrm{\scriptsize 27}$,
J.A.~Kremer$^\textrm{\scriptsize 41a}$,
M.~Kretz$^\textrm{\scriptsize 60c}$,
J.~Kretzschmar$^\textrm{\scriptsize 77}$,
K.~Kreutzfeldt$^\textrm{\scriptsize 55}$,
P.~Krieger$^\textrm{\scriptsize 161}$,
K.~Krizka$^\textrm{\scriptsize 33}$,
K.~Kroeninger$^\textrm{\scriptsize 46}$,
H.~Kroha$^\textrm{\scriptsize 103}$,
J.~Kroll$^\textrm{\scriptsize 124}$,
J.~Kroseberg$^\textrm{\scriptsize 23}$,
J.~Krstic$^\textrm{\scriptsize 14}$,
U.~Kruchonak$^\textrm{\scriptsize 68}$,
H.~Kr\"uger$^\textrm{\scriptsize 23}$,
N.~Krumnack$^\textrm{\scriptsize 67}$,
M.C.~Kruse$^\textrm{\scriptsize 48}$,
M.~Kruskal$^\textrm{\scriptsize 24}$,
T.~Kubota$^\textrm{\scriptsize 91}$,
H.~Kucuk$^\textrm{\scriptsize 81}$,
S.~Kuday$^\textrm{\scriptsize 4b}$,
J.T.~Kuechler$^\textrm{\scriptsize 178}$,
S.~Kuehn$^\textrm{\scriptsize 51}$,
A.~Kugel$^\textrm{\scriptsize 60c}$,
F.~Kuger$^\textrm{\scriptsize 177}$,
T.~Kuhl$^\textrm{\scriptsize 45}$,
V.~Kukhtin$^\textrm{\scriptsize 68}$,
R.~Kukla$^\textrm{\scriptsize 138}$,
Y.~Kulchitsky$^\textrm{\scriptsize 95}$,
S.~Kuleshov$^\textrm{\scriptsize 34b}$,
M.~Kuna$^\textrm{\scriptsize 134a,134b}$,
T.~Kunigo$^\textrm{\scriptsize 71}$,
A.~Kupco$^\textrm{\scriptsize 129}$,
O.~Kuprash$^\textrm{\scriptsize 155}$,
H.~Kurashige$^\textrm{\scriptsize 70}$,
L.L.~Kurchaninov$^\textrm{\scriptsize 163a}$,
Y.A.~Kurochkin$^\textrm{\scriptsize 95}$,
M.G.~Kurth$^\textrm{\scriptsize 35a}$,
V.~Kus$^\textrm{\scriptsize 129}$,
E.S.~Kuwertz$^\textrm{\scriptsize 172}$,
M.~Kuze$^\textrm{\scriptsize 159}$,
J.~Kvita$^\textrm{\scriptsize 117}$,
T.~Kwan$^\textrm{\scriptsize 172}$,
D.~Kyriazopoulos$^\textrm{\scriptsize 141}$,
A.~La~Rosa$^\textrm{\scriptsize 103}$,
J.L.~La~Rosa~Navarro$^\textrm{\scriptsize 26d}$,
L.~La~Rotonda$^\textrm{\scriptsize 40a,40b}$,
C.~Lacasta$^\textrm{\scriptsize 170}$,
F.~Lacava$^\textrm{\scriptsize 134a,134b}$,
J.~Lacey$^\textrm{\scriptsize 31}$,
H.~Lacker$^\textrm{\scriptsize 17}$,
D.~Lacour$^\textrm{\scriptsize 83}$,
E.~Ladygin$^\textrm{\scriptsize 68}$,
R.~Lafaye$^\textrm{\scriptsize 5}$,
B.~Laforge$^\textrm{\scriptsize 83}$,
T.~Lagouri$^\textrm{\scriptsize 179}$,
S.~Lai$^\textrm{\scriptsize 57}$,
S.~Lammers$^\textrm{\scriptsize 64}$,
W.~Lampl$^\textrm{\scriptsize 7}$,
E.~Lan\c{c}on$^\textrm{\scriptsize 27}$,
U.~Landgraf$^\textrm{\scriptsize 51}$,
M.P.J.~Landon$^\textrm{\scriptsize 79}$,
M.C.~Lanfermann$^\textrm{\scriptsize 52}$,
V.S.~Lang$^\textrm{\scriptsize 60a}$,
J.C.~Lange$^\textrm{\scriptsize 13}$,
A.J.~Lankford$^\textrm{\scriptsize 166}$,
F.~Lanni$^\textrm{\scriptsize 27}$,
K.~Lantzsch$^\textrm{\scriptsize 23}$,
A.~Lanza$^\textrm{\scriptsize 123a}$,
A.~Lapertosa$^\textrm{\scriptsize 53a,53b}$,
S.~Laplace$^\textrm{\scriptsize 83}$,
J.F.~Laporte$^\textrm{\scriptsize 138}$,
T.~Lari$^\textrm{\scriptsize 94a}$,
F.~Lasagni~Manghi$^\textrm{\scriptsize 22a,22b}$,
M.~Lassnig$^\textrm{\scriptsize 32}$,
P.~Laurelli$^\textrm{\scriptsize 50}$,
W.~Lavrijsen$^\textrm{\scriptsize 16}$,
A.T.~Law$^\textrm{\scriptsize 139}$,
P.~Laycock$^\textrm{\scriptsize 77}$,
T.~Lazovich$^\textrm{\scriptsize 59}$,
M.~Lazzaroni$^\textrm{\scriptsize 94a,94b}$,
B.~Le$^\textrm{\scriptsize 91}$,
O.~Le~Dortz$^\textrm{\scriptsize 83}$,
E.~Le~Guirriec$^\textrm{\scriptsize 88}$,
E.P.~Le~Quilleuc$^\textrm{\scriptsize 138}$,
M.~LeBlanc$^\textrm{\scriptsize 172}$,
T.~LeCompte$^\textrm{\scriptsize 6}$,
F.~Ledroit-Guillon$^\textrm{\scriptsize 58}$,
C.A.~Lee$^\textrm{\scriptsize 27}$,
S.C.~Lee$^\textrm{\scriptsize 153}$,
L.~Lee$^\textrm{\scriptsize 1}$,
B.~Lefebvre$^\textrm{\scriptsize 90}$,
G.~Lefebvre$^\textrm{\scriptsize 83}$,
M.~Lefebvre$^\textrm{\scriptsize 172}$,
F.~Legger$^\textrm{\scriptsize 102}$,
C.~Leggett$^\textrm{\scriptsize 16}$,
A.~Lehan$^\textrm{\scriptsize 77}$,
G.~Lehmann~Miotto$^\textrm{\scriptsize 32}$,
X.~Lei$^\textrm{\scriptsize 7}$,
W.A.~Leight$^\textrm{\scriptsize 31}$,
A.G.~Leister$^\textrm{\scriptsize 179}$,
M.A.L.~Leite$^\textrm{\scriptsize 26d}$,
R.~Leitner$^\textrm{\scriptsize 131}$,
D.~Lellouch$^\textrm{\scriptsize 175}$,
B.~Lemmer$^\textrm{\scriptsize 57}$,
K.J.C.~Leney$^\textrm{\scriptsize 81}$,
T.~Lenz$^\textrm{\scriptsize 23}$,
B.~Lenzi$^\textrm{\scriptsize 32}$,
R.~Leone$^\textrm{\scriptsize 7}$,
S.~Leone$^\textrm{\scriptsize 126a,126b}$,
C.~Leonidopoulos$^\textrm{\scriptsize 49}$,
S.~Leontsinis$^\textrm{\scriptsize 10}$,
G.~Lerner$^\textrm{\scriptsize 151}$,
C.~Leroy$^\textrm{\scriptsize 97}$,
A.A.J.~Lesage$^\textrm{\scriptsize 138}$,
C.G.~Lester$^\textrm{\scriptsize 30}$,
M.~Levchenko$^\textrm{\scriptsize 125}$,
J.~Lev\^eque$^\textrm{\scriptsize 5}$,
D.~Levin$^\textrm{\scriptsize 92}$,
L.J.~Levinson$^\textrm{\scriptsize 175}$,
M.~Levy$^\textrm{\scriptsize 19}$,
D.~Lewis$^\textrm{\scriptsize 79}$,
M.~Leyton$^\textrm{\scriptsize 44}$,
B.~Li$^\textrm{\scriptsize 36a}$$^{,q}$,
C.~Li$^\textrm{\scriptsize 36a}$,
H.~Li$^\textrm{\scriptsize 150}$,
L.~Li$^\textrm{\scriptsize 48}$,
L.~Li$^\textrm{\scriptsize 36c}$,
Q.~Li$^\textrm{\scriptsize 35a}$,
S.~Li$^\textrm{\scriptsize 48}$,
X.~Li$^\textrm{\scriptsize 87}$,
Y.~Li$^\textrm{\scriptsize 143}$,
Z.~Liang$^\textrm{\scriptsize 35a}$,
B.~Liberti$^\textrm{\scriptsize 135a}$,
A.~Liblong$^\textrm{\scriptsize 161}$,
K.~Lie$^\textrm{\scriptsize 169}$,
J.~Liebal$^\textrm{\scriptsize 23}$,
W.~Liebig$^\textrm{\scriptsize 15}$,
A.~Limosani$^\textrm{\scriptsize 152}$,
S.C.~Lin$^\textrm{\scriptsize 153}$$^{,ad}$,
T.H.~Lin$^\textrm{\scriptsize 86}$,
B.E.~Lindquist$^\textrm{\scriptsize 150}$,
A.E.~Lionti$^\textrm{\scriptsize 52}$,
E.~Lipeles$^\textrm{\scriptsize 124}$,
A.~Lipniacka$^\textrm{\scriptsize 15}$,
M.~Lisovyi$^\textrm{\scriptsize 60b}$,
T.M.~Liss$^\textrm{\scriptsize 169}$,
A.~Lister$^\textrm{\scriptsize 171}$,
A.M.~Litke$^\textrm{\scriptsize 139}$,
B.~Liu$^\textrm{\scriptsize 153}$$^{,ae}$,
H.~Liu$^\textrm{\scriptsize 92}$,
H.~Liu$^\textrm{\scriptsize 27}$,
J.~Liu$^\textrm{\scriptsize 36b}$,
J.B.~Liu$^\textrm{\scriptsize 36a}$,
K.~Liu$^\textrm{\scriptsize 88}$,
L.~Liu$^\textrm{\scriptsize 169}$,
M.~Liu$^\textrm{\scriptsize 36a}$,
Y.L.~Liu$^\textrm{\scriptsize 36a}$,
Y.~Liu$^\textrm{\scriptsize 36a}$,
M.~Livan$^\textrm{\scriptsize 123a,123b}$,
A.~Lleres$^\textrm{\scriptsize 58}$,
J.~Llorente~Merino$^\textrm{\scriptsize 35a}$,
S.L.~Lloyd$^\textrm{\scriptsize 79}$,
F.~Lo~Sterzo$^\textrm{\scriptsize 153}$,
E.M.~Lobodzinska$^\textrm{\scriptsize 45}$,
P.~Loch$^\textrm{\scriptsize 7}$,
F.K.~Loebinger$^\textrm{\scriptsize 87}$,
K.M.~Loew$^\textrm{\scriptsize 25}$,
A.~Loginov$^\textrm{\scriptsize 179}$$^{,*}$,
T.~Lohse$^\textrm{\scriptsize 17}$,
K.~Lohwasser$^\textrm{\scriptsize 45}$,
M.~Lokajicek$^\textrm{\scriptsize 129}$,
B.A.~Long$^\textrm{\scriptsize 24}$,
J.D.~Long$^\textrm{\scriptsize 169}$,
R.E.~Long$^\textrm{\scriptsize 75}$,
L.~Longo$^\textrm{\scriptsize 76a,76b}$,
K.A.~Looper$^\textrm{\scriptsize 113}$,
J.A.~Lopez$^\textrm{\scriptsize 34b}$,
D.~Lopez~Mateos$^\textrm{\scriptsize 59}$,
B.~Lopez~Paredes$^\textrm{\scriptsize 141}$,
I.~Lopez~Paz$^\textrm{\scriptsize 13}$,
A.~Lopez~Solis$^\textrm{\scriptsize 83}$,
J.~Lorenz$^\textrm{\scriptsize 102}$,
N.~Lorenzo~Martinez$^\textrm{\scriptsize 64}$,
M.~Losada$^\textrm{\scriptsize 21}$,
P.J.~L{\"o}sel$^\textrm{\scriptsize 102}$,
X.~Lou$^\textrm{\scriptsize 35a}$,
A.~Lounis$^\textrm{\scriptsize 119}$,
J.~Love$^\textrm{\scriptsize 6}$,
P.A.~Love$^\textrm{\scriptsize 75}$,
H.~Lu$^\textrm{\scriptsize 62a}$,
N.~Lu$^\textrm{\scriptsize 92}$,
H.J.~Lubatti$^\textrm{\scriptsize 140}$,
C.~Luci$^\textrm{\scriptsize 134a,134b}$,
A.~Lucotte$^\textrm{\scriptsize 58}$,
C.~Luedtke$^\textrm{\scriptsize 51}$,
F.~Luehring$^\textrm{\scriptsize 64}$,
W.~Lukas$^\textrm{\scriptsize 65}$,
L.~Luminari$^\textrm{\scriptsize 134a}$,
O.~Lundberg$^\textrm{\scriptsize 148a,148b}$,
B.~Lund-Jensen$^\textrm{\scriptsize 149}$,
P.M.~Luzi$^\textrm{\scriptsize 83}$,
D.~Lynn$^\textrm{\scriptsize 27}$,
R.~Lysak$^\textrm{\scriptsize 129}$,
E.~Lytken$^\textrm{\scriptsize 84}$,
V.~Lyubushkin$^\textrm{\scriptsize 68}$,
H.~Ma$^\textrm{\scriptsize 27}$,
L.L.~Ma$^\textrm{\scriptsize 36b}$,
Y.~Ma$^\textrm{\scriptsize 36b}$,
G.~Maccarrone$^\textrm{\scriptsize 50}$,
A.~Macchiolo$^\textrm{\scriptsize 103}$,
C.M.~Macdonald$^\textrm{\scriptsize 141}$,
B.~Ma\v{c}ek$^\textrm{\scriptsize 78}$,
J.~Machado~Miguens$^\textrm{\scriptsize 124,128b}$,
D.~Madaffari$^\textrm{\scriptsize 88}$,
R.~Madar$^\textrm{\scriptsize 37}$,
H.J.~Maddocks$^\textrm{\scriptsize 168}$,
W.F.~Mader$^\textrm{\scriptsize 47}$,
A.~Madsen$^\textrm{\scriptsize 45}$,
J.~Maeda$^\textrm{\scriptsize 70}$,
S.~Maeland$^\textrm{\scriptsize 15}$,
T.~Maeno$^\textrm{\scriptsize 27}$,
A.~Maevskiy$^\textrm{\scriptsize 101}$,
E.~Magradze$^\textrm{\scriptsize 57}$,
J.~Mahlstedt$^\textrm{\scriptsize 109}$,
C.~Maiani$^\textrm{\scriptsize 119}$,
C.~Maidantchik$^\textrm{\scriptsize 26a}$,
A.A.~Maier$^\textrm{\scriptsize 103}$,
T.~Maier$^\textrm{\scriptsize 102}$,
A.~Maio$^\textrm{\scriptsize 128a,128b,128d}$,
S.~Majewski$^\textrm{\scriptsize 118}$,
Y.~Makida$^\textrm{\scriptsize 69}$,
N.~Makovec$^\textrm{\scriptsize 119}$,
B.~Malaescu$^\textrm{\scriptsize 83}$,
Pa.~Malecki$^\textrm{\scriptsize 42}$,
V.P.~Maleev$^\textrm{\scriptsize 125}$,
F.~Malek$^\textrm{\scriptsize 58}$,
U.~Mallik$^\textrm{\scriptsize 66}$,
D.~Malon$^\textrm{\scriptsize 6}$,
C.~Malone$^\textrm{\scriptsize 30}$,
S.~Maltezos$^\textrm{\scriptsize 10}$,
S.~Malyukov$^\textrm{\scriptsize 32}$,
J.~Mamuzic$^\textrm{\scriptsize 170}$,
G.~Mancini$^\textrm{\scriptsize 50}$,
L.~Mandelli$^\textrm{\scriptsize 94a}$,
I.~Mandi\'{c}$^\textrm{\scriptsize 78}$,
J.~Maneira$^\textrm{\scriptsize 128a,128b}$,
L.~Manhaes~de~Andrade~Filho$^\textrm{\scriptsize 26b}$,
J.~Manjarres~Ramos$^\textrm{\scriptsize 163b}$,
A.~Mann$^\textrm{\scriptsize 102}$,
A.~Manousos$^\textrm{\scriptsize 32}$,
B.~Mansoulie$^\textrm{\scriptsize 138}$,
J.D.~Mansour$^\textrm{\scriptsize 35a}$,
R.~Mantifel$^\textrm{\scriptsize 90}$,
M.~Mantoani$^\textrm{\scriptsize 57}$,
S.~Manzoni$^\textrm{\scriptsize 94a,94b}$,
L.~Mapelli$^\textrm{\scriptsize 32}$,
G.~Marceca$^\textrm{\scriptsize 29}$,
L.~March$^\textrm{\scriptsize 52}$,
G.~Marchiori$^\textrm{\scriptsize 83}$,
M.~Marcisovsky$^\textrm{\scriptsize 129}$,
M.~Marjanovic$^\textrm{\scriptsize 14}$,
D.E.~Marley$^\textrm{\scriptsize 92}$,
F.~Marroquim$^\textrm{\scriptsize 26a}$,
S.P.~Marsden$^\textrm{\scriptsize 87}$,
Z.~Marshall$^\textrm{\scriptsize 16}$,
M.U.F~Martensson$^\textrm{\scriptsize 168}$,
S.~Marti-Garcia$^\textrm{\scriptsize 170}$,
T.A.~Martin$^\textrm{\scriptsize 173}$,
V.J.~Martin$^\textrm{\scriptsize 49}$,
B.~Martin~dit~Latour$^\textrm{\scriptsize 15}$,
M.~Martinez$^\textrm{\scriptsize 13}$$^{,t}$,
V.I.~Martinez~Outschoorn$^\textrm{\scriptsize 169}$,
S.~Martin-Haugh$^\textrm{\scriptsize 133}$,
V.S.~Martoiu$^\textrm{\scriptsize 28b}$,
A.C.~Martyniuk$^\textrm{\scriptsize 81}$,
A.~Marzin$^\textrm{\scriptsize 32}$,
L.~Masetti$^\textrm{\scriptsize 86}$,
T.~Mashimo$^\textrm{\scriptsize 157}$,
R.~Mashinistov$^\textrm{\scriptsize 98}$,
J.~Masik$^\textrm{\scriptsize 87}$,
A.L.~Maslennikov$^\textrm{\scriptsize 111}$$^{,c}$,
L.~Massa$^\textrm{\scriptsize 135a,135b}$,
P.~Mastrandrea$^\textrm{\scriptsize 5}$,
A.~Mastroberardino$^\textrm{\scriptsize 40a,40b}$,
T.~Masubuchi$^\textrm{\scriptsize 157}$,
P.~M\"attig$^\textrm{\scriptsize 178}$,
J.~Mattmann$^\textrm{\scriptsize 86}$,
J.~Maurer$^\textrm{\scriptsize 28b}$,
S.J.~Maxfield$^\textrm{\scriptsize 77}$,
D.A.~Maximov$^\textrm{\scriptsize 111}$$^{,c}$,
R.~Mazini$^\textrm{\scriptsize 153}$,
I.~Maznas$^\textrm{\scriptsize 156}$,
S.M.~Mazza$^\textrm{\scriptsize 94a,94b}$,
N.C.~Mc~Fadden$^\textrm{\scriptsize 107}$,
G.~Mc~Goldrick$^\textrm{\scriptsize 161}$,
S.P.~Mc~Kee$^\textrm{\scriptsize 92}$,
A.~McCarn$^\textrm{\scriptsize 92}$,
R.L.~McCarthy$^\textrm{\scriptsize 150}$,
T.G.~McCarthy$^\textrm{\scriptsize 103}$,
L.I.~McClymont$^\textrm{\scriptsize 81}$,
E.F.~McDonald$^\textrm{\scriptsize 91}$,
J.A.~Mcfayden$^\textrm{\scriptsize 81}$,
G.~Mchedlidze$^\textrm{\scriptsize 57}$,
S.J.~McMahon$^\textrm{\scriptsize 133}$,
P.C.~McNamara$^\textrm{\scriptsize 91}$,
R.A.~McPherson$^\textrm{\scriptsize 172}$$^{,n}$,
S.~Meehan$^\textrm{\scriptsize 140}$,
S.~Mehlhase$^\textrm{\scriptsize 102}$,
A.~Mehta$^\textrm{\scriptsize 77}$,
K.~Meier$^\textrm{\scriptsize 60a}$,
C.~Meineck$^\textrm{\scriptsize 102}$,
B.~Meirose$^\textrm{\scriptsize 44}$,
D.~Melini$^\textrm{\scriptsize 170}$$^{,af}$,
B.R.~Mellado~Garcia$^\textrm{\scriptsize 147c}$,
M.~Melo$^\textrm{\scriptsize 146a}$,
F.~Meloni$^\textrm{\scriptsize 18}$,
S.B.~Menary$^\textrm{\scriptsize 87}$,
L.~Meng$^\textrm{\scriptsize 77}$,
X.T.~Meng$^\textrm{\scriptsize 92}$,
A.~Mengarelli$^\textrm{\scriptsize 22a,22b}$,
S.~Menke$^\textrm{\scriptsize 103}$,
E.~Meoni$^\textrm{\scriptsize 165}$,
S.~Mergelmeyer$^\textrm{\scriptsize 17}$,
P.~Mermod$^\textrm{\scriptsize 52}$,
L.~Merola$^\textrm{\scriptsize 106a,106b}$,
C.~Meroni$^\textrm{\scriptsize 94a}$,
F.S.~Merritt$^\textrm{\scriptsize 33}$,
A.~Messina$^\textrm{\scriptsize 134a,134b}$,
J.~Metcalfe$^\textrm{\scriptsize 6}$,
A.S.~Mete$^\textrm{\scriptsize 166}$,
C.~Meyer$^\textrm{\scriptsize 124}$,
J-P.~Meyer$^\textrm{\scriptsize 138}$,
J.~Meyer$^\textrm{\scriptsize 109}$,
H.~Meyer~Zu~Theenhausen$^\textrm{\scriptsize 60a}$,
F.~Miano$^\textrm{\scriptsize 151}$,
R.P.~Middleton$^\textrm{\scriptsize 133}$,
S.~Miglioranzi$^\textrm{\scriptsize 53a,53b}$,
L.~Mijovi\'{c}$^\textrm{\scriptsize 49}$,
G.~Mikenberg$^\textrm{\scriptsize 175}$,
M.~Mikestikova$^\textrm{\scriptsize 129}$,
M.~Miku\v{z}$^\textrm{\scriptsize 78}$,
M.~Milesi$^\textrm{\scriptsize 91}$,
A.~Milic$^\textrm{\scriptsize 27}$,
D.W.~Miller$^\textrm{\scriptsize 33}$,
C.~Mills$^\textrm{\scriptsize 49}$,
A.~Milov$^\textrm{\scriptsize 175}$,
D.A.~Milstead$^\textrm{\scriptsize 148a,148b}$,
A.A.~Minaenko$^\textrm{\scriptsize 132}$,
Y.~Minami$^\textrm{\scriptsize 157}$,
I.A.~Minashvili$^\textrm{\scriptsize 68}$,
A.I.~Mincer$^\textrm{\scriptsize 112}$,
B.~Mindur$^\textrm{\scriptsize 41a}$,
M.~Mineev$^\textrm{\scriptsize 68}$,
Y.~Minegishi$^\textrm{\scriptsize 157}$,
Y.~Ming$^\textrm{\scriptsize 176}$,
L.M.~Mir$^\textrm{\scriptsize 13}$,
K.P.~Mistry$^\textrm{\scriptsize 124}$,
T.~Mitani$^\textrm{\scriptsize 174}$,
J.~Mitrevski$^\textrm{\scriptsize 102}$,
V.A.~Mitsou$^\textrm{\scriptsize 170}$,
A.~Miucci$^\textrm{\scriptsize 18}$,
P.S.~Miyagawa$^\textrm{\scriptsize 141}$,
A.~Mizukami$^\textrm{\scriptsize 69}$,
J.U.~Mj\"ornmark$^\textrm{\scriptsize 84}$,
M.~Mlynarikova$^\textrm{\scriptsize 131}$,
T.~Moa$^\textrm{\scriptsize 148a,148b}$,
K.~Mochizuki$^\textrm{\scriptsize 97}$,
P.~Mogg$^\textrm{\scriptsize 51}$,
S.~Mohapatra$^\textrm{\scriptsize 38}$,
S.~Molander$^\textrm{\scriptsize 148a,148b}$,
R.~Moles-Valls$^\textrm{\scriptsize 23}$,
R.~Monden$^\textrm{\scriptsize 71}$,
M.C.~Mondragon$^\textrm{\scriptsize 93}$,
K.~M\"onig$^\textrm{\scriptsize 45}$,
J.~Monk$^\textrm{\scriptsize 39}$,
E.~Monnier$^\textrm{\scriptsize 88}$,
A.~Montalbano$^\textrm{\scriptsize 150}$,
J.~Montejo~Berlingen$^\textrm{\scriptsize 32}$,
F.~Monticelli$^\textrm{\scriptsize 74}$,
S.~Monzani$^\textrm{\scriptsize 94a,94b}$,
R.W.~Moore$^\textrm{\scriptsize 3}$,
N.~Morange$^\textrm{\scriptsize 119}$,
D.~Moreno$^\textrm{\scriptsize 21}$,
M.~Moreno~Ll\'acer$^\textrm{\scriptsize 57}$,
P.~Morettini$^\textrm{\scriptsize 53a}$,
S.~Morgenstern$^\textrm{\scriptsize 32}$,
D.~Mori$^\textrm{\scriptsize 144}$,
T.~Mori$^\textrm{\scriptsize 157}$,
M.~Morii$^\textrm{\scriptsize 59}$,
M.~Morinaga$^\textrm{\scriptsize 157}$,
V.~Morisbak$^\textrm{\scriptsize 121}$,
S.~Moritz$^\textrm{\scriptsize 86}$,
A.K.~Morley$^\textrm{\scriptsize 152}$,
G.~Mornacchi$^\textrm{\scriptsize 32}$,
J.D.~Morris$^\textrm{\scriptsize 79}$,
L.~Morvaj$^\textrm{\scriptsize 150}$,
P.~Moschovakos$^\textrm{\scriptsize 10}$,
M.~Mosidze$^\textrm{\scriptsize 54b}$,
H.J.~Moss$^\textrm{\scriptsize 141}$,
J.~Moss$^\textrm{\scriptsize 145}$$^{,ag}$,
K.~Motohashi$^\textrm{\scriptsize 159}$,
R.~Mount$^\textrm{\scriptsize 145}$,
E.~Mountricha$^\textrm{\scriptsize 27}$,
E.J.W.~Moyse$^\textrm{\scriptsize 89}$,
S.~Muanza$^\textrm{\scriptsize 88}$,
R.D.~Mudd$^\textrm{\scriptsize 19}$,
F.~Mueller$^\textrm{\scriptsize 103}$,
J.~Mueller$^\textrm{\scriptsize 127}$,
R.S.P.~Mueller$^\textrm{\scriptsize 102}$,
T.~Mueller$^\textrm{\scriptsize 30}$,
D.~Muenstermann$^\textrm{\scriptsize 75}$,
P.~Mullen$^\textrm{\scriptsize 56}$,
G.A.~Mullier$^\textrm{\scriptsize 18}$,
F.J.~Munoz~Sanchez$^\textrm{\scriptsize 87}$,
J.A.~Murillo~Quijada$^\textrm{\scriptsize 19}$,
W.J.~Murray$^\textrm{\scriptsize 173,133}$,
H.~Musheghyan$^\textrm{\scriptsize 57}$,
M.~Mu\v{s}kinja$^\textrm{\scriptsize 78}$,
A.G.~Myagkov$^\textrm{\scriptsize 132}$$^{,ah}$,
M.~Myska$^\textrm{\scriptsize 130}$,
B.P.~Nachman$^\textrm{\scriptsize 16}$,
O.~Nackenhorst$^\textrm{\scriptsize 52}$,
K.~Nagai$^\textrm{\scriptsize 122}$,
R.~Nagai$^\textrm{\scriptsize 69}$$^{,ab}$,
K.~Nagano$^\textrm{\scriptsize 69}$,
Y.~Nagasaka$^\textrm{\scriptsize 61}$,
K.~Nagata$^\textrm{\scriptsize 164}$,
M.~Nagel$^\textrm{\scriptsize 51}$,
E.~Nagy$^\textrm{\scriptsize 88}$,
A.M.~Nairz$^\textrm{\scriptsize 32}$,
Y.~Nakahama$^\textrm{\scriptsize 105}$,
K.~Nakamura$^\textrm{\scriptsize 69}$,
T.~Nakamura$^\textrm{\scriptsize 157}$,
I.~Nakano$^\textrm{\scriptsize 114}$,
R.F.~Naranjo~Garcia$^\textrm{\scriptsize 45}$,
R.~Narayan$^\textrm{\scriptsize 11}$,
D.I.~Narrias~Villar$^\textrm{\scriptsize 60a}$,
I.~Naryshkin$^\textrm{\scriptsize 125}$,
T.~Naumann$^\textrm{\scriptsize 45}$,
G.~Navarro$^\textrm{\scriptsize 21}$,
R.~Nayyar$^\textrm{\scriptsize 7}$,
H.A.~Neal$^\textrm{\scriptsize 92}$,
P.Yu.~Nechaeva$^\textrm{\scriptsize 98}$,
T.J.~Neep$^\textrm{\scriptsize 87}$,
A.~Negri$^\textrm{\scriptsize 123a,123b}$,
M.~Negrini$^\textrm{\scriptsize 22a}$,
S.~Nektarijevic$^\textrm{\scriptsize 108}$,
C.~Nellist$^\textrm{\scriptsize 119}$,
A.~Nelson$^\textrm{\scriptsize 166}$,
S.~Nemecek$^\textrm{\scriptsize 129}$,
P.~Nemethy$^\textrm{\scriptsize 112}$,
A.A.~Nepomuceno$^\textrm{\scriptsize 26a}$,
M.~Nessi$^\textrm{\scriptsize 32}$$^{,ai}$,
M.S.~Neubauer$^\textrm{\scriptsize 169}$,
M.~Neumann$^\textrm{\scriptsize 178}$,
R.M.~Neves$^\textrm{\scriptsize 112}$,
P.~Nevski$^\textrm{\scriptsize 27}$,
P.R.~Newman$^\textrm{\scriptsize 19}$,
T.~Nguyen~Manh$^\textrm{\scriptsize 97}$,
R.B.~Nickerson$^\textrm{\scriptsize 122}$,
R.~Nicolaidou$^\textrm{\scriptsize 138}$,
J.~Nielsen$^\textrm{\scriptsize 139}$,
V.~Nikolaenko$^\textrm{\scriptsize 132}$$^{,ah}$,
I.~Nikolic-Audit$^\textrm{\scriptsize 83}$,
K.~Nikolopoulos$^\textrm{\scriptsize 19}$,
J.K.~Nilsen$^\textrm{\scriptsize 121}$,
P.~Nilsson$^\textrm{\scriptsize 27}$,
Y.~Ninomiya$^\textrm{\scriptsize 157}$,
A.~Nisati$^\textrm{\scriptsize 134a}$,
R.~Nisius$^\textrm{\scriptsize 103}$,
T.~Nobe$^\textrm{\scriptsize 157}$,
Y.~Noguchi$^\textrm{\scriptsize 71}$,
M.~Nomachi$^\textrm{\scriptsize 120}$,
I.~Nomidis$^\textrm{\scriptsize 31}$,
T.~Nooney$^\textrm{\scriptsize 79}$,
M.~Nordberg$^\textrm{\scriptsize 32}$,
N.~Norjoharuddeen$^\textrm{\scriptsize 122}$,
O.~Novgorodova$^\textrm{\scriptsize 47}$,
S.~Nowak$^\textrm{\scriptsize 103}$,
M.~Nozaki$^\textrm{\scriptsize 69}$,
L.~Nozka$^\textrm{\scriptsize 117}$,
K.~Ntekas$^\textrm{\scriptsize 166}$,
E.~Nurse$^\textrm{\scriptsize 81}$,
F.~Nuti$^\textrm{\scriptsize 91}$,
D.C.~O'Neil$^\textrm{\scriptsize 144}$,
A.A.~O'Rourke$^\textrm{\scriptsize 45}$,
V.~O'Shea$^\textrm{\scriptsize 56}$,
F.G.~Oakham$^\textrm{\scriptsize 31}$$^{,d}$,
H.~Oberlack$^\textrm{\scriptsize 103}$,
T.~Obermann$^\textrm{\scriptsize 23}$,
J.~Ocariz$^\textrm{\scriptsize 83}$,
A.~Ochi$^\textrm{\scriptsize 70}$,
I.~Ochoa$^\textrm{\scriptsize 38}$,
J.P.~Ochoa-Ricoux$^\textrm{\scriptsize 34a}$,
S.~Oda$^\textrm{\scriptsize 73}$,
S.~Odaka$^\textrm{\scriptsize 69}$,
H.~Ogren$^\textrm{\scriptsize 64}$,
A.~Oh$^\textrm{\scriptsize 87}$,
S.H.~Oh$^\textrm{\scriptsize 48}$,
C.C.~Ohm$^\textrm{\scriptsize 16}$,
H.~Ohman$^\textrm{\scriptsize 168}$,
H.~Oide$^\textrm{\scriptsize 53a,53b}$,
H.~Okawa$^\textrm{\scriptsize 164}$,
Y.~Okumura$^\textrm{\scriptsize 157}$,
T.~Okuyama$^\textrm{\scriptsize 69}$,
A.~Olariu$^\textrm{\scriptsize 28b}$,
L.F.~Oleiro~Seabra$^\textrm{\scriptsize 128a}$,
S.A.~Olivares~Pino$^\textrm{\scriptsize 49}$,
D.~Oliveira~Damazio$^\textrm{\scriptsize 27}$,
A.~Olszewski$^\textrm{\scriptsize 42}$,
J.~Olszowska$^\textrm{\scriptsize 42}$,
A.~Onofre$^\textrm{\scriptsize 128a,128e}$,
K.~Onogi$^\textrm{\scriptsize 105}$,
P.U.E.~Onyisi$^\textrm{\scriptsize 11}$$^{,x}$,
M.J.~Oreglia$^\textrm{\scriptsize 33}$,
Y.~Oren$^\textrm{\scriptsize 155}$,
D.~Orestano$^\textrm{\scriptsize 136a,136b}$,
N.~Orlando$^\textrm{\scriptsize 62b}$,
R.S.~Orr$^\textrm{\scriptsize 161}$,
B.~Osculati$^\textrm{\scriptsize 53a,53b}$$^{,*}$,
R.~Ospanov$^\textrm{\scriptsize 87}$,
G.~Otero~y~Garzon$^\textrm{\scriptsize 29}$,
H.~Otono$^\textrm{\scriptsize 73}$,
M.~Ouchrif$^\textrm{\scriptsize 137d}$,
F.~Ould-Saada$^\textrm{\scriptsize 121}$,
A.~Ouraou$^\textrm{\scriptsize 138}$,
K.P.~Oussoren$^\textrm{\scriptsize 109}$,
Q.~Ouyang$^\textrm{\scriptsize 35a}$,
M.~Owen$^\textrm{\scriptsize 56}$,
R.E.~Owen$^\textrm{\scriptsize 19}$,
V.E.~Ozcan$^\textrm{\scriptsize 20a}$,
N.~Ozturk$^\textrm{\scriptsize 8}$,
K.~Pachal$^\textrm{\scriptsize 144}$,
A.~Pacheco~Pages$^\textrm{\scriptsize 13}$,
L.~Pacheco~Rodriguez$^\textrm{\scriptsize 138}$,
C.~Padilla~Aranda$^\textrm{\scriptsize 13}$,
S.~Pagan~Griso$^\textrm{\scriptsize 16}$,
M.~Paganini$^\textrm{\scriptsize 179}$,
F.~Paige$^\textrm{\scriptsize 27}$,
P.~Pais$^\textrm{\scriptsize 89}$,
G.~Palacino$^\textrm{\scriptsize 64}$,
S.~Palazzo$^\textrm{\scriptsize 40a,40b}$,
S.~Palestini$^\textrm{\scriptsize 32}$,
M.~Palka$^\textrm{\scriptsize 41b}$,
D.~Pallin$^\textrm{\scriptsize 37}$,
E.St.~Panagiotopoulou$^\textrm{\scriptsize 10}$,
I.~Panagoulias$^\textrm{\scriptsize 10}$,
C.E.~Pandini$^\textrm{\scriptsize 83}$,
J.G.~Panduro~Vazquez$^\textrm{\scriptsize 80}$,
P.~Pani$^\textrm{\scriptsize 148a,148b}$,
S.~Panitkin$^\textrm{\scriptsize 27}$,
D.~Pantea$^\textrm{\scriptsize 28b}$,
L.~Paolozzi$^\textrm{\scriptsize 52}$,
Th.D.~Papadopoulou$^\textrm{\scriptsize 10}$,
K.~Papageorgiou$^\textrm{\scriptsize 9}$,
A.~Paramonov$^\textrm{\scriptsize 6}$,
D.~Paredes~Hernandez$^\textrm{\scriptsize 179}$,
A.J.~Parker$^\textrm{\scriptsize 75}$,
M.A.~Parker$^\textrm{\scriptsize 30}$,
K.A.~Parker$^\textrm{\scriptsize 45}$,
F.~Parodi$^\textrm{\scriptsize 53a,53b}$,
J.A.~Parsons$^\textrm{\scriptsize 38}$,
U.~Parzefall$^\textrm{\scriptsize 51}$,
V.R.~Pascuzzi$^\textrm{\scriptsize 161}$,
E.~Pasqualucci$^\textrm{\scriptsize 134a}$,
S.~Passaggio$^\textrm{\scriptsize 53a}$,
Fr.~Pastore$^\textrm{\scriptsize 80}$,
S.~Pataraia$^\textrm{\scriptsize 178}$,
J.R.~Pater$^\textrm{\scriptsize 87}$,
T.~Pauly$^\textrm{\scriptsize 32}$,
J.~Pearce$^\textrm{\scriptsize 172}$,
B.~Pearson$^\textrm{\scriptsize 115}$,
L.E.~Pedersen$^\textrm{\scriptsize 39}$,
S.~Pedraza~Lopez$^\textrm{\scriptsize 170}$,
R.~Pedro$^\textrm{\scriptsize 128a,128b}$,
S.V.~Peleganchuk$^\textrm{\scriptsize 111}$$^{,c}$,
O.~Penc$^\textrm{\scriptsize 129}$,
C.~Peng$^\textrm{\scriptsize 35a}$,
H.~Peng$^\textrm{\scriptsize 36a}$,
J.~Penwell$^\textrm{\scriptsize 64}$,
B.S.~Peralva$^\textrm{\scriptsize 26b}$,
M.M.~Perego$^\textrm{\scriptsize 138}$,
D.V.~Perepelitsa$^\textrm{\scriptsize 27}$,
L.~Perini$^\textrm{\scriptsize 94a,94b}$,
H.~Pernegger$^\textrm{\scriptsize 32}$,
S.~Perrella$^\textrm{\scriptsize 106a,106b}$,
R.~Peschke$^\textrm{\scriptsize 45}$,
V.D.~Peshekhonov$^\textrm{\scriptsize 68}$,
K.~Peters$^\textrm{\scriptsize 45}$,
R.F.Y.~Peters$^\textrm{\scriptsize 87}$,
B.A.~Petersen$^\textrm{\scriptsize 32}$,
T.C.~Petersen$^\textrm{\scriptsize 39}$,
E.~Petit$^\textrm{\scriptsize 58}$,
A.~Petridis$^\textrm{\scriptsize 1}$,
C.~Petridou$^\textrm{\scriptsize 156}$,
P.~Petroff$^\textrm{\scriptsize 119}$,
E.~Petrolo$^\textrm{\scriptsize 134a}$,
M.~Petrov$^\textrm{\scriptsize 122}$,
F.~Petrucci$^\textrm{\scriptsize 136a,136b}$,
N.E.~Pettersson$^\textrm{\scriptsize 89}$,
A.~Peyaud$^\textrm{\scriptsize 138}$,
R.~Pezoa$^\textrm{\scriptsize 34b}$,
P.W.~Phillips$^\textrm{\scriptsize 133}$,
G.~Piacquadio$^\textrm{\scriptsize 150}$,
E.~Pianori$^\textrm{\scriptsize 173}$,
A.~Picazio$^\textrm{\scriptsize 89}$,
E.~Piccaro$^\textrm{\scriptsize 79}$,
M.A.~Pickering$^\textrm{\scriptsize 122}$,
R.~Piegaia$^\textrm{\scriptsize 29}$,
J.E.~Pilcher$^\textrm{\scriptsize 33}$,
A.D.~Pilkington$^\textrm{\scriptsize 87}$,
A.W.J.~Pin$^\textrm{\scriptsize 87}$,
M.~Pinamonti$^\textrm{\scriptsize 167a,167c}$$^{,aj}$,
J.L.~Pinfold$^\textrm{\scriptsize 3}$,
S.~Pires$^\textrm{\scriptsize 83}$,
H.~Pirumov$^\textrm{\scriptsize 45}$,
M.~Pitt$^\textrm{\scriptsize 175}$,
L.~Plazak$^\textrm{\scriptsize 146a}$,
M.-A.~Pleier$^\textrm{\scriptsize 27}$,
V.~Pleskot$^\textrm{\scriptsize 86}$,
E.~Plotnikova$^\textrm{\scriptsize 68}$,
D.~Pluth$^\textrm{\scriptsize 67}$,
P.~Podberezko$^\textrm{\scriptsize 111}$,
R.~Poettgen$^\textrm{\scriptsize 148a,148b}$,
L.~Poggioli$^\textrm{\scriptsize 119}$,
D.~Pohl$^\textrm{\scriptsize 23}$,
G.~Polesello$^\textrm{\scriptsize 123a}$,
A.~Poley$^\textrm{\scriptsize 45}$,
A.~Policicchio$^\textrm{\scriptsize 40a,40b}$,
R.~Polifka$^\textrm{\scriptsize 32}$,
A.~Polini$^\textrm{\scriptsize 22a}$,
C.S.~Pollard$^\textrm{\scriptsize 56}$,
V.~Polychronakos$^\textrm{\scriptsize 27}$,
K.~Pomm\`es$^\textrm{\scriptsize 32}$,
L.~Pontecorvo$^\textrm{\scriptsize 134a}$,
B.G.~Pope$^\textrm{\scriptsize 93}$,
G.A.~Popeneciu$^\textrm{\scriptsize 28c}$,
A.~Poppleton$^\textrm{\scriptsize 32}$,
S.~Pospisil$^\textrm{\scriptsize 130}$,
K.~Potamianos$^\textrm{\scriptsize 16}$,
I.N.~Potrap$^\textrm{\scriptsize 68}$,
C.J.~Potter$^\textrm{\scriptsize 30}$,
C.T.~Potter$^\textrm{\scriptsize 118}$,
G.~Poulard$^\textrm{\scriptsize 32}$,
J.~Poveda$^\textrm{\scriptsize 32}$,
V.~Pozdnyakov$^\textrm{\scriptsize 68}$,
M.E.~Pozo~Astigarraga$^\textrm{\scriptsize 32}$,
P.~Pralavorio$^\textrm{\scriptsize 88}$,
A.~Pranko$^\textrm{\scriptsize 16}$,
S.~Prell$^\textrm{\scriptsize 67}$,
D.~Price$^\textrm{\scriptsize 87}$,
L.E.~Price$^\textrm{\scriptsize 6}$,
M.~Primavera$^\textrm{\scriptsize 76a}$,
S.~Prince$^\textrm{\scriptsize 90}$,
K.~Prokofiev$^\textrm{\scriptsize 62c}$,
F.~Prokoshin$^\textrm{\scriptsize 34b}$,
S.~Protopopescu$^\textrm{\scriptsize 27}$,
J.~Proudfoot$^\textrm{\scriptsize 6}$,
M.~Przybycien$^\textrm{\scriptsize 41a}$,
D.~Puddu$^\textrm{\scriptsize 136a,136b}$,
M.~Purohit$^\textrm{\scriptsize 27}$$^{,ak}$,
P.~Puzo$^\textrm{\scriptsize 119}$,
J.~Qian$^\textrm{\scriptsize 92}$,
G.~Qin$^\textrm{\scriptsize 56}$,
Y.~Qin$^\textrm{\scriptsize 87}$,
A.~Quadt$^\textrm{\scriptsize 57}$,
W.B.~Quayle$^\textrm{\scriptsize 167a,167b}$,
M.~Queitsch-Maitland$^\textrm{\scriptsize 45}$,
D.~Quilty$^\textrm{\scriptsize 56}$,
S.~Raddum$^\textrm{\scriptsize 121}$,
V.~Radeka$^\textrm{\scriptsize 27}$,
V.~Radescu$^\textrm{\scriptsize 122}$,
S.K.~Radhakrishnan$^\textrm{\scriptsize 150}$,
P.~Radloff$^\textrm{\scriptsize 118}$,
P.~Rados$^\textrm{\scriptsize 91}$,
F.~Ragusa$^\textrm{\scriptsize 94a,94b}$,
G.~Rahal$^\textrm{\scriptsize 181}$,
J.A.~Raine$^\textrm{\scriptsize 87}$,
S.~Rajagopalan$^\textrm{\scriptsize 27}$,
M.~Rammensee$^\textrm{\scriptsize 32}$,
C.~Rangel-Smith$^\textrm{\scriptsize 168}$,
M.G.~Ratti$^\textrm{\scriptsize 94a,94b}$,
D.M.~Rauch$^\textrm{\scriptsize 45}$,
F.~Rauscher$^\textrm{\scriptsize 102}$,
S.~Rave$^\textrm{\scriptsize 86}$,
T.~Ravenscroft$^\textrm{\scriptsize 56}$,
I.~Ravinovich$^\textrm{\scriptsize 175}$,
M.~Raymond$^\textrm{\scriptsize 32}$,
A.L.~Read$^\textrm{\scriptsize 121}$,
N.P.~Readioff$^\textrm{\scriptsize 77}$,
M.~Reale$^\textrm{\scriptsize 76a,76b}$,
D.M.~Rebuzzi$^\textrm{\scriptsize 123a,123b}$,
A.~Redelbach$^\textrm{\scriptsize 177}$,
G.~Redlinger$^\textrm{\scriptsize 27}$,
R.~Reece$^\textrm{\scriptsize 139}$,
R.G.~Reed$^\textrm{\scriptsize 147c}$,
K.~Reeves$^\textrm{\scriptsize 44}$,
L.~Rehnisch$^\textrm{\scriptsize 17}$,
J.~Reichert$^\textrm{\scriptsize 124}$,
A.~Reiss$^\textrm{\scriptsize 86}$,
C.~Rembser$^\textrm{\scriptsize 32}$,
H.~Ren$^\textrm{\scriptsize 35a}$,
M.~Rescigno$^\textrm{\scriptsize 134a}$,
S.~Resconi$^\textrm{\scriptsize 94a}$,
E.D.~Resseguie$^\textrm{\scriptsize 124}$,
O.L.~Rezanova$^\textrm{\scriptsize 111}$$^{,c}$,
P.~Reznicek$^\textrm{\scriptsize 131}$,
R.~Rezvani$^\textrm{\scriptsize 97}$,
R.~Richter$^\textrm{\scriptsize 103}$,
S.~Richter$^\textrm{\scriptsize 81}$,
E.~Richter-Was$^\textrm{\scriptsize 41b}$,
O.~Ricken$^\textrm{\scriptsize 23}$,
M.~Ridel$^\textrm{\scriptsize 83}$,
P.~Rieck$^\textrm{\scriptsize 103}$,
C.J.~Riegel$^\textrm{\scriptsize 178}$,
J.~Rieger$^\textrm{\scriptsize 57}$,
O.~Rifki$^\textrm{\scriptsize 115}$,
M.~Rijssenbeek$^\textrm{\scriptsize 150}$,
A.~Rimoldi$^\textrm{\scriptsize 123a,123b}$,
M.~Rimoldi$^\textrm{\scriptsize 18}$,
L.~Rinaldi$^\textrm{\scriptsize 22a}$,
B.~Risti\'{c}$^\textrm{\scriptsize 52}$,
E.~Ritsch$^\textrm{\scriptsize 32}$,
I.~Riu$^\textrm{\scriptsize 13}$,
F.~Rizatdinova$^\textrm{\scriptsize 116}$,
E.~Rizvi$^\textrm{\scriptsize 79}$,
C.~Rizzi$^\textrm{\scriptsize 13}$,
R.T.~Roberts$^\textrm{\scriptsize 87}$,
S.H.~Robertson$^\textrm{\scriptsize 90}$$^{,n}$,
A.~Robichaud-Veronneau$^\textrm{\scriptsize 90}$,
D.~Robinson$^\textrm{\scriptsize 30}$,
J.E.M.~Robinson$^\textrm{\scriptsize 45}$,
A.~Robson$^\textrm{\scriptsize 56}$,
C.~Roda$^\textrm{\scriptsize 126a,126b}$,
Y.~Rodina$^\textrm{\scriptsize 88}$$^{,al}$,
A.~Rodriguez~Perez$^\textrm{\scriptsize 13}$,
D.~Rodriguez~Rodriguez$^\textrm{\scriptsize 170}$,
S.~Roe$^\textrm{\scriptsize 32}$,
C.S.~Rogan$^\textrm{\scriptsize 59}$,
O.~R{\o}hne$^\textrm{\scriptsize 121}$,
J.~Roloff$^\textrm{\scriptsize 59}$,
A.~Romaniouk$^\textrm{\scriptsize 100}$,
M.~Romano$^\textrm{\scriptsize 22a,22b}$,
S.M.~Romano~Saez$^\textrm{\scriptsize 37}$,
E.~Romero~Adam$^\textrm{\scriptsize 170}$,
N.~Rompotis$^\textrm{\scriptsize 77}$,
M.~Ronzani$^\textrm{\scriptsize 51}$,
L.~Roos$^\textrm{\scriptsize 83}$,
E.~Ros$^\textrm{\scriptsize 170}$,
S.~Rosati$^\textrm{\scriptsize 134a}$,
K.~Rosbach$^\textrm{\scriptsize 51}$,
P.~Rose$^\textrm{\scriptsize 139}$,
N.-A.~Rosien$^\textrm{\scriptsize 57}$,
V.~Rossetti$^\textrm{\scriptsize 148a,148b}$,
E.~Rossi$^\textrm{\scriptsize 106a,106b}$,
L.P.~Rossi$^\textrm{\scriptsize 53a}$,
J.H.N.~Rosten$^\textrm{\scriptsize 30}$,
R.~Rosten$^\textrm{\scriptsize 140}$,
M.~Rotaru$^\textrm{\scriptsize 28b}$,
I.~Roth$^\textrm{\scriptsize 175}$,
J.~Rothberg$^\textrm{\scriptsize 140}$,
D.~Rousseau$^\textrm{\scriptsize 119}$,
A.~Rozanov$^\textrm{\scriptsize 88}$,
Y.~Rozen$^\textrm{\scriptsize 154}$,
X.~Ruan$^\textrm{\scriptsize 147c}$,
F.~Rubbo$^\textrm{\scriptsize 145}$,
F.~R\"uhr$^\textrm{\scriptsize 51}$,
A.~Ruiz-Martinez$^\textrm{\scriptsize 31}$,
Z.~Rurikova$^\textrm{\scriptsize 51}$,
N.A.~Rusakovich$^\textrm{\scriptsize 68}$,
A.~Ruschke$^\textrm{\scriptsize 102}$,
H.L.~Russell$^\textrm{\scriptsize 140}$,
J.P.~Rutherfoord$^\textrm{\scriptsize 7}$,
N.~Ruthmann$^\textrm{\scriptsize 32}$,
Y.F.~Ryabov$^\textrm{\scriptsize 125}$,
M.~Rybar$^\textrm{\scriptsize 169}$,
G.~Rybkin$^\textrm{\scriptsize 119}$,
S.~Ryu$^\textrm{\scriptsize 6}$,
A.~Ryzhov$^\textrm{\scriptsize 132}$,
G.F.~Rzehorz$^\textrm{\scriptsize 57}$,
A.F.~Saavedra$^\textrm{\scriptsize 152}$,
G.~Sabato$^\textrm{\scriptsize 109}$,
S.~Sacerdoti$^\textrm{\scriptsize 29}$,
H.F-W.~Sadrozinski$^\textrm{\scriptsize 139}$,
R.~Sadykov$^\textrm{\scriptsize 68}$,
F.~Safai~Tehrani$^\textrm{\scriptsize 134a}$,
P.~Saha$^\textrm{\scriptsize 110}$,
M.~Sahinsoy$^\textrm{\scriptsize 60a}$,
M.~Saimpert$^\textrm{\scriptsize 138}$,
T.~Saito$^\textrm{\scriptsize 157}$,
H.~Sakamoto$^\textrm{\scriptsize 157}$,
Y.~Sakurai$^\textrm{\scriptsize 174}$,
G.~Salamanna$^\textrm{\scriptsize 136a,136b}$,
J.E.~Salazar~Loyola$^\textrm{\scriptsize 34b}$,
D.~Salek$^\textrm{\scriptsize 109}$,
P.H.~Sales~De~Bruin$^\textrm{\scriptsize 140}$,
D.~Salihagic$^\textrm{\scriptsize 103}$,
A.~Salnikov$^\textrm{\scriptsize 145}$,
J.~Salt$^\textrm{\scriptsize 170}$,
D.~Salvatore$^\textrm{\scriptsize 40a,40b}$,
F.~Salvatore$^\textrm{\scriptsize 151}$,
A.~Salvucci$^\textrm{\scriptsize 62a,62b,62c}$,
A.~Salzburger$^\textrm{\scriptsize 32}$,
D.~Sammel$^\textrm{\scriptsize 51}$,
D.~Sampsonidis$^\textrm{\scriptsize 156}$,
J.~S\'anchez$^\textrm{\scriptsize 170}$,
V.~Sanchez~Martinez$^\textrm{\scriptsize 170}$,
A.~Sanchez~Pineda$^\textrm{\scriptsize 106a,106b}$,
H.~Sandaker$^\textrm{\scriptsize 121}$,
R.L.~Sandbach$^\textrm{\scriptsize 79}$,
M.~Sandhoff$^\textrm{\scriptsize 178}$,
C.~Sandoval$^\textrm{\scriptsize 21}$,
D.P.C.~Sankey$^\textrm{\scriptsize 133}$,
M.~Sannino$^\textrm{\scriptsize 53a,53b}$,
A.~Sansoni$^\textrm{\scriptsize 50}$,
C.~Santoni$^\textrm{\scriptsize 37}$,
R.~Santonico$^\textrm{\scriptsize 135a,135b}$,
H.~Santos$^\textrm{\scriptsize 128a}$,
I.~Santoyo~Castillo$^\textrm{\scriptsize 151}$,
K.~Sapp$^\textrm{\scriptsize 127}$,
A.~Sapronov$^\textrm{\scriptsize 68}$,
J.G.~Saraiva$^\textrm{\scriptsize 128a,128d}$,
B.~Sarrazin$^\textrm{\scriptsize 23}$,
O.~Sasaki$^\textrm{\scriptsize 69}$,
K.~Sato$^\textrm{\scriptsize 164}$,
E.~Sauvan$^\textrm{\scriptsize 5}$,
G.~Savage$^\textrm{\scriptsize 80}$,
P.~Savard$^\textrm{\scriptsize 161}$$^{,d}$,
N.~Savic$^\textrm{\scriptsize 103}$,
C.~Sawyer$^\textrm{\scriptsize 133}$,
L.~Sawyer$^\textrm{\scriptsize 82}$$^{,s}$,
J.~Saxon$^\textrm{\scriptsize 33}$,
C.~Sbarra$^\textrm{\scriptsize 22a}$,
A.~Sbrizzi$^\textrm{\scriptsize 22a,22b}$,
T.~Scanlon$^\textrm{\scriptsize 81}$,
D.A.~Scannicchio$^\textrm{\scriptsize 166}$,
M.~Scarcella$^\textrm{\scriptsize 152}$,
V.~Scarfone$^\textrm{\scriptsize 40a,40b}$,
J.~Schaarschmidt$^\textrm{\scriptsize 140}$,
P.~Schacht$^\textrm{\scriptsize 103}$,
B.M.~Schachtner$^\textrm{\scriptsize 102}$,
D.~Schaefer$^\textrm{\scriptsize 32}$,
L.~Schaefer$^\textrm{\scriptsize 124}$,
R.~Schaefer$^\textrm{\scriptsize 45}$,
J.~Schaeffer$^\textrm{\scriptsize 86}$,
S.~Schaepe$^\textrm{\scriptsize 23}$,
S.~Schaetzel$^\textrm{\scriptsize 60b}$,
U.~Sch\"afer$^\textrm{\scriptsize 86}$,
A.C.~Schaffer$^\textrm{\scriptsize 119}$,
D.~Schaile$^\textrm{\scriptsize 102}$,
R.D.~Schamberger$^\textrm{\scriptsize 150}$,
V.~Scharf$^\textrm{\scriptsize 60a}$,
V.A.~Schegelsky$^\textrm{\scriptsize 125}$,
D.~Scheirich$^\textrm{\scriptsize 131}$,
M.~Schernau$^\textrm{\scriptsize 166}$,
C.~Schiavi$^\textrm{\scriptsize 53a,53b}$,
S.~Schier$^\textrm{\scriptsize 139}$,
C.~Schillo$^\textrm{\scriptsize 51}$,
M.~Schioppa$^\textrm{\scriptsize 40a,40b}$,
S.~Schlenker$^\textrm{\scriptsize 32}$,
K.R.~Schmidt-Sommerfeld$^\textrm{\scriptsize 103}$,
K.~Schmieden$^\textrm{\scriptsize 32}$,
C.~Schmitt$^\textrm{\scriptsize 86}$,
S.~Schmitt$^\textrm{\scriptsize 45}$,
S.~Schmitz$^\textrm{\scriptsize 86}$,
B.~Schneider$^\textrm{\scriptsize 163a}$,
U.~Schnoor$^\textrm{\scriptsize 51}$,
L.~Schoeffel$^\textrm{\scriptsize 138}$,
A.~Schoening$^\textrm{\scriptsize 60b}$,
B.D.~Schoenrock$^\textrm{\scriptsize 93}$,
E.~Schopf$^\textrm{\scriptsize 23}$,
M.~Schott$^\textrm{\scriptsize 86}$,
J.F.P.~Schouwenberg$^\textrm{\scriptsize 108}$,
J.~Schovancova$^\textrm{\scriptsize 8}$,
S.~Schramm$^\textrm{\scriptsize 52}$,
M.~Schreyer$^\textrm{\scriptsize 177}$,
N.~Schuh$^\textrm{\scriptsize 86}$,
A.~Schulte$^\textrm{\scriptsize 86}$,
M.J.~Schultens$^\textrm{\scriptsize 23}$,
H.-C.~Schultz-Coulon$^\textrm{\scriptsize 60a}$,
H.~Schulz$^\textrm{\scriptsize 17}$,
M.~Schumacher$^\textrm{\scriptsize 51}$,
B.A.~Schumm$^\textrm{\scriptsize 139}$,
Ph.~Schune$^\textrm{\scriptsize 138}$,
A.~Schwartzman$^\textrm{\scriptsize 145}$,
T.A.~Schwarz$^\textrm{\scriptsize 92}$,
H.~Schweiger$^\textrm{\scriptsize 87}$,
Ph.~Schwemling$^\textrm{\scriptsize 138}$,
R.~Schwienhorst$^\textrm{\scriptsize 93}$,
J.~Schwindling$^\textrm{\scriptsize 138}$,
T.~Schwindt$^\textrm{\scriptsize 23}$,
G.~Sciolla$^\textrm{\scriptsize 25}$,
F.~Scuri$^\textrm{\scriptsize 126a,126b}$,
F.~Scutti$^\textrm{\scriptsize 91}$,
J.~Searcy$^\textrm{\scriptsize 92}$,
P.~Seema$^\textrm{\scriptsize 23}$,
S.C.~Seidel$^\textrm{\scriptsize 107}$,
A.~Seiden$^\textrm{\scriptsize 139}$,
J.M.~Seixas$^\textrm{\scriptsize 26a}$,
G.~Sekhniaidze$^\textrm{\scriptsize 106a}$,
K.~Sekhon$^\textrm{\scriptsize 92}$,
S.J.~Sekula$^\textrm{\scriptsize 43}$,
N.~Semprini-Cesari$^\textrm{\scriptsize 22a,22b}$,
C.~Serfon$^\textrm{\scriptsize 121}$,
L.~Serin$^\textrm{\scriptsize 119}$,
L.~Serkin$^\textrm{\scriptsize 167a,167b}$,
M.~Sessa$^\textrm{\scriptsize 136a,136b}$,
R.~Seuster$^\textrm{\scriptsize 172}$,
H.~Severini$^\textrm{\scriptsize 115}$,
T.~Sfiligoj$^\textrm{\scriptsize 78}$,
F.~Sforza$^\textrm{\scriptsize 32}$,
A.~Sfyrla$^\textrm{\scriptsize 52}$,
E.~Shabalina$^\textrm{\scriptsize 57}$,
N.W.~Shaikh$^\textrm{\scriptsize 148a,148b}$,
L.Y.~Shan$^\textrm{\scriptsize 35a}$,
R.~Shang$^\textrm{\scriptsize 169}$,
J.T.~Shank$^\textrm{\scriptsize 24}$,
M.~Shapiro$^\textrm{\scriptsize 16}$,
P.B.~Shatalov$^\textrm{\scriptsize 99}$,
K.~Shaw$^\textrm{\scriptsize 167a,167b}$,
S.M.~Shaw$^\textrm{\scriptsize 87}$,
A.~Shcherbakova$^\textrm{\scriptsize 148a,148b}$,
C.Y.~Shehu$^\textrm{\scriptsize 151}$,
Y.~Shen$^\textrm{\scriptsize 115}$,
P.~Sherwood$^\textrm{\scriptsize 81}$,
L.~Shi$^\textrm{\scriptsize 153}$$^{,am}$,
S.~Shimizu$^\textrm{\scriptsize 70}$,
C.O.~Shimmin$^\textrm{\scriptsize 166}$,
M.~Shimojima$^\textrm{\scriptsize 104}$,
S.~Shirabe$^\textrm{\scriptsize 73}$,
M.~Shiyakova$^\textrm{\scriptsize 68}$$^{,an}$,
J.~Shlomi$^\textrm{\scriptsize 175}$,
A.~Shmeleva$^\textrm{\scriptsize 98}$,
D.~Shoaleh~Saadi$^\textrm{\scriptsize 97}$,
M.J.~Shochet$^\textrm{\scriptsize 33}$,
S.~Shojaii$^\textrm{\scriptsize 94a}$,
D.R.~Shope$^\textrm{\scriptsize 115}$,
S.~Shrestha$^\textrm{\scriptsize 113}$,
E.~Shulga$^\textrm{\scriptsize 100}$,
M.A.~Shupe$^\textrm{\scriptsize 7}$,
P.~Sicho$^\textrm{\scriptsize 129}$,
A.M.~Sickles$^\textrm{\scriptsize 169}$,
P.E.~Sidebo$^\textrm{\scriptsize 149}$,
E.~Sideras~Haddad$^\textrm{\scriptsize 147c}$,
O.~Sidiropoulou$^\textrm{\scriptsize 177}$,
D.~Sidorov$^\textrm{\scriptsize 116}$,
A.~Sidoti$^\textrm{\scriptsize 22a,22b}$,
F.~Siegert$^\textrm{\scriptsize 47}$,
Dj.~Sijacki$^\textrm{\scriptsize 14}$,
J.~Silva$^\textrm{\scriptsize 128a,128d}$,
S.B.~Silverstein$^\textrm{\scriptsize 148a}$,
V.~Simak$^\textrm{\scriptsize 130}$,
Lj.~Simic$^\textrm{\scriptsize 14}$,
S.~Simion$^\textrm{\scriptsize 119}$,
E.~Simioni$^\textrm{\scriptsize 86}$,
B.~Simmons$^\textrm{\scriptsize 81}$,
M.~Simon$^\textrm{\scriptsize 86}$,
P.~Sinervo$^\textrm{\scriptsize 161}$,
N.B.~Sinev$^\textrm{\scriptsize 118}$,
M.~Sioli$^\textrm{\scriptsize 22a,22b}$,
G.~Siragusa$^\textrm{\scriptsize 177}$,
I.~Siral$^\textrm{\scriptsize 92}$,
S.Yu.~Sivoklokov$^\textrm{\scriptsize 101}$,
J.~Sj\"{o}lin$^\textrm{\scriptsize 148a,148b}$,
M.B.~Skinner$^\textrm{\scriptsize 75}$,
P.~Skubic$^\textrm{\scriptsize 115}$,
M.~Slater$^\textrm{\scriptsize 19}$,
T.~Slavicek$^\textrm{\scriptsize 130}$,
M.~Slawinska$^\textrm{\scriptsize 109}$,
K.~Sliwa$^\textrm{\scriptsize 165}$,
R.~Slovak$^\textrm{\scriptsize 131}$,
V.~Smakhtin$^\textrm{\scriptsize 175}$,
B.H.~Smart$^\textrm{\scriptsize 5}$,
L.~Smestad$^\textrm{\scriptsize 15}$,
J.~Smiesko$^\textrm{\scriptsize 146a}$,
S.Yu.~Smirnov$^\textrm{\scriptsize 100}$,
Y.~Smirnov$^\textrm{\scriptsize 100}$,
L.N.~Smirnova$^\textrm{\scriptsize 101}$$^{,ao}$,
O.~Smirnova$^\textrm{\scriptsize 84}$,
J.W.~Smith$^\textrm{\scriptsize 57}$,
M.N.K.~Smith$^\textrm{\scriptsize 38}$,
R.W.~Smith$^\textrm{\scriptsize 38}$,
M.~Smizanska$^\textrm{\scriptsize 75}$,
K.~Smolek$^\textrm{\scriptsize 130}$,
A.A.~Snesarev$^\textrm{\scriptsize 98}$,
I.M.~Snyder$^\textrm{\scriptsize 118}$,
S.~Snyder$^\textrm{\scriptsize 27}$,
R.~Sobie$^\textrm{\scriptsize 172}$$^{,n}$,
F.~Socher$^\textrm{\scriptsize 47}$,
A.~Soffer$^\textrm{\scriptsize 155}$,
D.A.~Soh$^\textrm{\scriptsize 153}$,
G.~Sokhrannyi$^\textrm{\scriptsize 78}$,
C.A.~Solans~Sanchez$^\textrm{\scriptsize 32}$,
M.~Solar$^\textrm{\scriptsize 130}$,
E.Yu.~Soldatov$^\textrm{\scriptsize 100}$,
U.~Soldevila$^\textrm{\scriptsize 170}$,
A.A.~Solodkov$^\textrm{\scriptsize 132}$,
A.~Soloshenko$^\textrm{\scriptsize 68}$,
O.V.~Solovyanov$^\textrm{\scriptsize 132}$,
V.~Solovyev$^\textrm{\scriptsize 125}$,
P.~Sommer$^\textrm{\scriptsize 51}$,
H.~Son$^\textrm{\scriptsize 165}$,
H.Y.~Song$^\textrm{\scriptsize 36a}$$^{,ap}$,
A.~Sopczak$^\textrm{\scriptsize 130}$,
V.~Sorin$^\textrm{\scriptsize 13}$,
D.~Sosa$^\textrm{\scriptsize 60b}$,
C.L.~Sotiropoulou$^\textrm{\scriptsize 126a,126b}$,
R.~Soualah$^\textrm{\scriptsize 167a,167c}$,
A.M.~Soukharev$^\textrm{\scriptsize 111}$$^{,c}$,
D.~South$^\textrm{\scriptsize 45}$,
B.C.~Sowden$^\textrm{\scriptsize 80}$,
S.~Spagnolo$^\textrm{\scriptsize 76a,76b}$,
M.~Spalla$^\textrm{\scriptsize 126a,126b}$,
M.~Spangenberg$^\textrm{\scriptsize 173}$,
F.~Span\`o$^\textrm{\scriptsize 80}$,
D.~Sperlich$^\textrm{\scriptsize 17}$,
F.~Spettel$^\textrm{\scriptsize 103}$,
T.M.~Spieker$^\textrm{\scriptsize 60a}$,
R.~Spighi$^\textrm{\scriptsize 22a}$,
G.~Spigo$^\textrm{\scriptsize 32}$,
L.A.~Spiller$^\textrm{\scriptsize 91}$,
M.~Spousta$^\textrm{\scriptsize 131}$,
R.D.~St.~Denis$^\textrm{\scriptsize 56}$$^{,*}$,
A.~Stabile$^\textrm{\scriptsize 94a}$,
R.~Stamen$^\textrm{\scriptsize 60a}$,
S.~Stamm$^\textrm{\scriptsize 17}$,
E.~Stanecka$^\textrm{\scriptsize 42}$,
R.W.~Stanek$^\textrm{\scriptsize 6}$,
C.~Stanescu$^\textrm{\scriptsize 136a}$,
M.M.~Stanitzki$^\textrm{\scriptsize 45}$,
S.~Stapnes$^\textrm{\scriptsize 121}$,
E.A.~Starchenko$^\textrm{\scriptsize 132}$,
G.H.~Stark$^\textrm{\scriptsize 33}$,
J.~Stark$^\textrm{\scriptsize 58}$,
S.H~Stark$^\textrm{\scriptsize 39}$,
P.~Staroba$^\textrm{\scriptsize 129}$,
P.~Starovoitov$^\textrm{\scriptsize 60a}$,
S.~St\"arz$^\textrm{\scriptsize 32}$,
R.~Staszewski$^\textrm{\scriptsize 42}$,
P.~Steinberg$^\textrm{\scriptsize 27}$,
B.~Stelzer$^\textrm{\scriptsize 144}$,
H.J.~Stelzer$^\textrm{\scriptsize 32}$,
O.~Stelzer-Chilton$^\textrm{\scriptsize 163a}$,
H.~Stenzel$^\textrm{\scriptsize 55}$,
G.A.~Stewart$^\textrm{\scriptsize 56}$,
J.A.~Stillings$^\textrm{\scriptsize 23}$,
M.C.~Stockton$^\textrm{\scriptsize 90}$,
M.~Stoebe$^\textrm{\scriptsize 90}$,
G.~Stoicea$^\textrm{\scriptsize 28b}$,
P.~Stolte$^\textrm{\scriptsize 57}$,
S.~Stonjek$^\textrm{\scriptsize 103}$,
A.R.~Stradling$^\textrm{\scriptsize 8}$,
A.~Straessner$^\textrm{\scriptsize 47}$,
M.E.~Stramaglia$^\textrm{\scriptsize 18}$,
J.~Strandberg$^\textrm{\scriptsize 149}$,
S.~Strandberg$^\textrm{\scriptsize 148a,148b}$,
A.~Strandlie$^\textrm{\scriptsize 121}$,
M.~Strauss$^\textrm{\scriptsize 115}$,
P.~Strizenec$^\textrm{\scriptsize 146b}$,
R.~Str\"ohmer$^\textrm{\scriptsize 177}$,
D.M.~Strom$^\textrm{\scriptsize 118}$,
R.~Stroynowski$^\textrm{\scriptsize 43}$,
A.~Strubig$^\textrm{\scriptsize 108}$,
S.A.~Stucci$^\textrm{\scriptsize 27}$,
B.~Stugu$^\textrm{\scriptsize 15}$,
N.A.~Styles$^\textrm{\scriptsize 45}$,
D.~Su$^\textrm{\scriptsize 145}$,
J.~Su$^\textrm{\scriptsize 127}$,
S.~Suchek$^\textrm{\scriptsize 60a}$,
Y.~Sugaya$^\textrm{\scriptsize 120}$,
M.~Suk$^\textrm{\scriptsize 130}$,
V.V.~Sulin$^\textrm{\scriptsize 98}$,
S.~Sultansoy$^\textrm{\scriptsize 4c}$,
T.~Sumida$^\textrm{\scriptsize 71}$,
S.~Sun$^\textrm{\scriptsize 59}$,
X.~Sun$^\textrm{\scriptsize 3}$,
K.~Suruliz$^\textrm{\scriptsize 151}$,
C.J.E.~Suster$^\textrm{\scriptsize 152}$,
M.R.~Sutton$^\textrm{\scriptsize 151}$,
S.~Suzuki$^\textrm{\scriptsize 69}$,
M.~Svatos$^\textrm{\scriptsize 129}$,
M.~Swiatlowski$^\textrm{\scriptsize 33}$,
S.P.~Swift$^\textrm{\scriptsize 2}$,
I.~Sykora$^\textrm{\scriptsize 146a}$,
T.~Sykora$^\textrm{\scriptsize 131}$,
D.~Ta$^\textrm{\scriptsize 51}$,
K.~Tackmann$^\textrm{\scriptsize 45}$,
J.~Taenzer$^\textrm{\scriptsize 155}$,
A.~Taffard$^\textrm{\scriptsize 166}$,
R.~Tafirout$^\textrm{\scriptsize 163a}$,
N.~Taiblum$^\textrm{\scriptsize 155}$,
H.~Takai$^\textrm{\scriptsize 27}$,
R.~Takashima$^\textrm{\scriptsize 72}$,
T.~Takeshita$^\textrm{\scriptsize 142}$,
Y.~Takubo$^\textrm{\scriptsize 69}$,
M.~Talby$^\textrm{\scriptsize 88}$,
A.A.~Talyshev$^\textrm{\scriptsize 111}$$^{,c}$,
J.~Tanaka$^\textrm{\scriptsize 157}$,
M.~Tanaka$^\textrm{\scriptsize 159}$,
R.~Tanaka$^\textrm{\scriptsize 119}$,
S.~Tanaka$^\textrm{\scriptsize 69}$,
R.~Tanioka$^\textrm{\scriptsize 70}$,
B.B.~Tannenwald$^\textrm{\scriptsize 113}$,
S.~Tapia~Araya$^\textrm{\scriptsize 34b}$,
S.~Tapprogge$^\textrm{\scriptsize 86}$,
S.~Tarem$^\textrm{\scriptsize 154}$,
G.F.~Tartarelli$^\textrm{\scriptsize 94a}$,
P.~Tas$^\textrm{\scriptsize 131}$,
M.~Tasevsky$^\textrm{\scriptsize 129}$,
T.~Tashiro$^\textrm{\scriptsize 71}$,
E.~Tassi$^\textrm{\scriptsize 40a,40b}$,
A.~Tavares~Delgado$^\textrm{\scriptsize 128a,128b}$,
Y.~Tayalati$^\textrm{\scriptsize 137e}$,
A.C.~Taylor$^\textrm{\scriptsize 107}$,
G.N.~Taylor$^\textrm{\scriptsize 91}$,
P.T.E.~Taylor$^\textrm{\scriptsize 91}$,
W.~Taylor$^\textrm{\scriptsize 163b}$,
P.~Teixeira-Dias$^\textrm{\scriptsize 80}$,
K.K.~Temming$^\textrm{\scriptsize 51}$,
D.~Temple$^\textrm{\scriptsize 144}$,
H.~Ten~Kate$^\textrm{\scriptsize 32}$,
P.K.~Teng$^\textrm{\scriptsize 153}$,
J.J.~Teoh$^\textrm{\scriptsize 120}$,
F.~Tepel$^\textrm{\scriptsize 178}$,
S.~Terada$^\textrm{\scriptsize 69}$,
K.~Terashi$^\textrm{\scriptsize 157}$,
J.~Terron$^\textrm{\scriptsize 85}$,
S.~Terzo$^\textrm{\scriptsize 13}$,
M.~Testa$^\textrm{\scriptsize 50}$,
R.J.~Teuscher$^\textrm{\scriptsize 161}$$^{,n}$,
T.~Theveneaux-Pelzer$^\textrm{\scriptsize 88}$,
J.P.~Thomas$^\textrm{\scriptsize 19}$,
J.~Thomas-Wilsker$^\textrm{\scriptsize 80}$,
P.D.~Thompson$^\textrm{\scriptsize 19}$,
A.S.~Thompson$^\textrm{\scriptsize 56}$,
L.A.~Thomsen$^\textrm{\scriptsize 179}$,
E.~Thomson$^\textrm{\scriptsize 124}$,
M.J.~Tibbetts$^\textrm{\scriptsize 16}$,
R.E.~Ticse~Torres$^\textrm{\scriptsize 88}$,
V.O.~Tikhomirov$^\textrm{\scriptsize 98}$$^{,aq}$,
Yu.A.~Tikhonov$^\textrm{\scriptsize 111}$$^{,c}$,
S.~Timoshenko$^\textrm{\scriptsize 100}$,
P.~Tipton$^\textrm{\scriptsize 179}$,
S.~Tisserant$^\textrm{\scriptsize 88}$,
K.~Todome$^\textrm{\scriptsize 159}$,
S.~Todorova-Nova$^\textrm{\scriptsize 5}$,
J.~Tojo$^\textrm{\scriptsize 73}$,
S.~Tok\'ar$^\textrm{\scriptsize 146a}$,
K.~Tokushuku$^\textrm{\scriptsize 69}$,
E.~Tolley$^\textrm{\scriptsize 59}$,
L.~Tomlinson$^\textrm{\scriptsize 87}$,
M.~Tomoto$^\textrm{\scriptsize 105}$,
L.~Tompkins$^\textrm{\scriptsize 145}$$^{,ar}$,
K.~Toms$^\textrm{\scriptsize 107}$,
B.~Tong$^\textrm{\scriptsize 59}$,
P.~Tornambe$^\textrm{\scriptsize 51}$,
E.~Torrence$^\textrm{\scriptsize 118}$,
H.~Torres$^\textrm{\scriptsize 144}$,
E.~Torr\'o~Pastor$^\textrm{\scriptsize 140}$,
J.~Toth$^\textrm{\scriptsize 88}$$^{,as}$,
F.~Touchard$^\textrm{\scriptsize 88}$,
D.R.~Tovey$^\textrm{\scriptsize 141}$,
C.J.~Treado$^\textrm{\scriptsize 112}$,
T.~Trefzger$^\textrm{\scriptsize 177}$,
A.~Tricoli$^\textrm{\scriptsize 27}$,
I.M.~Trigger$^\textrm{\scriptsize 163a}$,
S.~Trincaz-Duvoid$^\textrm{\scriptsize 83}$,
M.F.~Tripiana$^\textrm{\scriptsize 13}$,
W.~Trischuk$^\textrm{\scriptsize 161}$,
B.~Trocm\'e$^\textrm{\scriptsize 58}$,
A.~Trofymov$^\textrm{\scriptsize 45}$,
C.~Troncon$^\textrm{\scriptsize 94a}$,
M.~Trottier-McDonald$^\textrm{\scriptsize 16}$,
M.~Trovatelli$^\textrm{\scriptsize 172}$,
L.~Truong$^\textrm{\scriptsize 167a,167c}$,
M.~Trzebinski$^\textrm{\scriptsize 42}$,
A.~Trzupek$^\textrm{\scriptsize 42}$,
K.W.~Tsang$^\textrm{\scriptsize 62a}$,
J.C-L.~Tseng$^\textrm{\scriptsize 122}$,
P.V.~Tsiareshka$^\textrm{\scriptsize 95}$,
G.~Tsipolitis$^\textrm{\scriptsize 10}$,
N.~Tsirintanis$^\textrm{\scriptsize 9}$,
S.~Tsiskaridze$^\textrm{\scriptsize 13}$,
V.~Tsiskaridze$^\textrm{\scriptsize 51}$,
E.G.~Tskhadadze$^\textrm{\scriptsize 54a}$,
K.M.~Tsui$^\textrm{\scriptsize 62a}$,
I.I.~Tsukerman$^\textrm{\scriptsize 99}$,
V.~Tsulaia$^\textrm{\scriptsize 16}$,
S.~Tsuno$^\textrm{\scriptsize 69}$,
D.~Tsybychev$^\textrm{\scriptsize 150}$,
Y.~Tu$^\textrm{\scriptsize 62b}$,
A.~Tudorache$^\textrm{\scriptsize 28b}$,
V.~Tudorache$^\textrm{\scriptsize 28b}$,
T.T.~Tulbure$^\textrm{\scriptsize 28a}$,
A.N.~Tuna$^\textrm{\scriptsize 59}$,
S.A.~Tupputi$^\textrm{\scriptsize 22a,22b}$,
S.~Turchikhin$^\textrm{\scriptsize 68}$,
D.~Turgeman$^\textrm{\scriptsize 175}$,
I.~Turk~Cakir$^\textrm{\scriptsize 4b}$$^{,at}$,
R.~Turra$^\textrm{\scriptsize 94a,94b}$,
P.M.~Tuts$^\textrm{\scriptsize 38}$,
G.~Ucchielli$^\textrm{\scriptsize 22a,22b}$,
I.~Ueda$^\textrm{\scriptsize 69}$,
M.~Ughetto$^\textrm{\scriptsize 148a,148b}$,
F.~Ukegawa$^\textrm{\scriptsize 164}$,
G.~Unal$^\textrm{\scriptsize 32}$,
A.~Undrus$^\textrm{\scriptsize 27}$,
G.~Unel$^\textrm{\scriptsize 166}$,
F.C.~Ungaro$^\textrm{\scriptsize 91}$,
Y.~Unno$^\textrm{\scriptsize 69}$,
C.~Unverdorben$^\textrm{\scriptsize 102}$,
J.~Urban$^\textrm{\scriptsize 146b}$,
P.~Urquijo$^\textrm{\scriptsize 91}$,
P.~Urrejola$^\textrm{\scriptsize 86}$,
G.~Usai$^\textrm{\scriptsize 8}$,
J.~Usui$^\textrm{\scriptsize 69}$,
L.~Vacavant$^\textrm{\scriptsize 88}$,
V.~Vacek$^\textrm{\scriptsize 130}$,
B.~Vachon$^\textrm{\scriptsize 90}$,
C.~Valderanis$^\textrm{\scriptsize 102}$,
E.~Valdes~Santurio$^\textrm{\scriptsize 148a,148b}$,
N.~Valencic$^\textrm{\scriptsize 109}$,
S.~Valentinetti$^\textrm{\scriptsize 22a,22b}$,
A.~Valero$^\textrm{\scriptsize 170}$,
L.~Valery$^\textrm{\scriptsize 13}$,
S.~Valkar$^\textrm{\scriptsize 131}$,
J.A.~Valls~Ferrer$^\textrm{\scriptsize 170}$,
W.~Van~Den~Wollenberg$^\textrm{\scriptsize 109}$,
P.C.~Van~Der~Deijl$^\textrm{\scriptsize 109}$,
H.~van~der~Graaf$^\textrm{\scriptsize 109}$,
N.~van~Eldik$^\textrm{\scriptsize 154}$,
P.~van~Gemmeren$^\textrm{\scriptsize 6}$,
J.~Van~Nieuwkoop$^\textrm{\scriptsize 144}$,
I.~van~Vulpen$^\textrm{\scriptsize 109}$,
M.C.~van~Woerden$^\textrm{\scriptsize 109}$,
M.~Vanadia$^\textrm{\scriptsize 134a,134b}$,
W.~Vandelli$^\textrm{\scriptsize 32}$,
R.~Vanguri$^\textrm{\scriptsize 124}$,
A.~Vaniachine$^\textrm{\scriptsize 160}$,
P.~Vankov$^\textrm{\scriptsize 109}$,
G.~Vardanyan$^\textrm{\scriptsize 180}$,
R.~Vari$^\textrm{\scriptsize 134a}$,
E.W.~Varnes$^\textrm{\scriptsize 7}$,
C.~Varni$^\textrm{\scriptsize 53a,53b}$,
T.~Varol$^\textrm{\scriptsize 43}$,
D.~Varouchas$^\textrm{\scriptsize 83}$,
A.~Vartapetian$^\textrm{\scriptsize 8}$,
K.E.~Varvell$^\textrm{\scriptsize 152}$,
J.G.~Vasquez$^\textrm{\scriptsize 179}$,
G.A.~Vasquez$^\textrm{\scriptsize 34b}$,
F.~Vazeille$^\textrm{\scriptsize 37}$,
T.~Vazquez~Schroeder$^\textrm{\scriptsize 90}$,
J.~Veatch$^\textrm{\scriptsize 57}$,
V.~Veeraraghavan$^\textrm{\scriptsize 7}$,
L.M.~Veloce$^\textrm{\scriptsize 161}$,
F.~Veloso$^\textrm{\scriptsize 128a,128c}$,
S.~Veneziano$^\textrm{\scriptsize 134a}$,
A.~Ventura$^\textrm{\scriptsize 76a,76b}$,
M.~Venturi$^\textrm{\scriptsize 172}$,
N.~Venturi$^\textrm{\scriptsize 161}$,
A.~Venturini$^\textrm{\scriptsize 25}$,
V.~Vercesi$^\textrm{\scriptsize 123a}$,
M.~Verducci$^\textrm{\scriptsize 136a,136b}$,
W.~Verkerke$^\textrm{\scriptsize 109}$,
J.C.~Vermeulen$^\textrm{\scriptsize 109}$,
M.C.~Vetterli$^\textrm{\scriptsize 144}$$^{,d}$,
O.~Viazlo$^\textrm{\scriptsize 84}$,
I.~Vichou$^\textrm{\scriptsize 169}$$^{,*}$,
T.~Vickey$^\textrm{\scriptsize 141}$,
O.E.~Vickey~Boeriu$^\textrm{\scriptsize 141}$,
G.H.A.~Viehhauser$^\textrm{\scriptsize 122}$,
S.~Viel$^\textrm{\scriptsize 16}$,
L.~Vigani$^\textrm{\scriptsize 122}$,
M.~Villa$^\textrm{\scriptsize 22a,22b}$,
M.~Villaplana~Perez$^\textrm{\scriptsize 94a,94b}$,
E.~Vilucchi$^\textrm{\scriptsize 50}$,
M.G.~Vincter$^\textrm{\scriptsize 31}$,
V.B.~Vinogradov$^\textrm{\scriptsize 68}$,
A.~Vishwakarma$^\textrm{\scriptsize 45}$,
C.~Vittori$^\textrm{\scriptsize 22a,22b}$,
I.~Vivarelli$^\textrm{\scriptsize 151}$,
S.~Vlachos$^\textrm{\scriptsize 10}$,
M.~Vlasak$^\textrm{\scriptsize 130}$,
M.~Vogel$^\textrm{\scriptsize 178}$,
P.~Vokac$^\textrm{\scriptsize 130}$,
G.~Volpi$^\textrm{\scriptsize 126a,126b}$,
M.~Volpi$^\textrm{\scriptsize 91}$,
H.~von~der~Schmitt$^\textrm{\scriptsize 103}$,
E.~von~Toerne$^\textrm{\scriptsize 23}$,
V.~Vorobel$^\textrm{\scriptsize 131}$,
K.~Vorobev$^\textrm{\scriptsize 100}$,
M.~Vos$^\textrm{\scriptsize 170}$,
R.~Voss$^\textrm{\scriptsize 32}$,
J.H.~Vossebeld$^\textrm{\scriptsize 77}$,
N.~Vranjes$^\textrm{\scriptsize 14}$,
M.~Vranjes~Milosavljevic$^\textrm{\scriptsize 14}$,
V.~Vrba$^\textrm{\scriptsize 130}$,
M.~Vreeswijk$^\textrm{\scriptsize 109}$,
R.~Vuillermet$^\textrm{\scriptsize 32}$,
I.~Vukotic$^\textrm{\scriptsize 33}$,
P.~Wagner$^\textrm{\scriptsize 23}$,
W.~Wagner$^\textrm{\scriptsize 178}$,
H.~Wahlberg$^\textrm{\scriptsize 74}$,
S.~Wahrmund$^\textrm{\scriptsize 47}$,
J.~Wakabayashi$^\textrm{\scriptsize 105}$,
J.~Walder$^\textrm{\scriptsize 75}$,
R.~Walker$^\textrm{\scriptsize 102}$,
W.~Walkowiak$^\textrm{\scriptsize 143}$,
V.~Wallangen$^\textrm{\scriptsize 148a,148b}$,
C.~Wang$^\textrm{\scriptsize 35b}$,
C.~Wang$^\textrm{\scriptsize 36b}$$^{,au}$,
F.~Wang$^\textrm{\scriptsize 176}$,
H.~Wang$^\textrm{\scriptsize 16}$,
H.~Wang$^\textrm{\scriptsize 3}$,
J.~Wang$^\textrm{\scriptsize 45}$,
J.~Wang$^\textrm{\scriptsize 152}$,
Q.~Wang$^\textrm{\scriptsize 115}$,
R.~Wang$^\textrm{\scriptsize 6}$,
S.M.~Wang$^\textrm{\scriptsize 153}$,
T.~Wang$^\textrm{\scriptsize 38}$,
W.~Wang$^\textrm{\scriptsize 36a}$,
C.~Wanotayaroj$^\textrm{\scriptsize 118}$,
A.~Warburton$^\textrm{\scriptsize 90}$,
C.P.~Ward$^\textrm{\scriptsize 30}$,
D.R.~Wardrope$^\textrm{\scriptsize 81}$,
A.~Washbrook$^\textrm{\scriptsize 49}$,
P.M.~Watkins$^\textrm{\scriptsize 19}$,
A.T.~Watson$^\textrm{\scriptsize 19}$,
M.F.~Watson$^\textrm{\scriptsize 19}$,
G.~Watts$^\textrm{\scriptsize 140}$,
S.~Watts$^\textrm{\scriptsize 87}$,
B.M.~Waugh$^\textrm{\scriptsize 81}$,
S.~Webb$^\textrm{\scriptsize 86}$,
M.S.~Weber$^\textrm{\scriptsize 18}$,
S.W.~Weber$^\textrm{\scriptsize 177}$,
S.A.~Weber$^\textrm{\scriptsize 31}$,
J.S.~Webster$^\textrm{\scriptsize 6}$,
A.R.~Weidberg$^\textrm{\scriptsize 122}$,
B.~Weinert$^\textrm{\scriptsize 64}$,
J.~Weingarten$^\textrm{\scriptsize 57}$,
C.~Weiser$^\textrm{\scriptsize 51}$,
H.~Weits$^\textrm{\scriptsize 109}$,
P.S.~Wells$^\textrm{\scriptsize 32}$,
T.~Wenaus$^\textrm{\scriptsize 27}$,
T.~Wengler$^\textrm{\scriptsize 32}$,
S.~Wenig$^\textrm{\scriptsize 32}$,
N.~Wermes$^\textrm{\scriptsize 23}$,
M.D.~Werner$^\textrm{\scriptsize 67}$,
P.~Werner$^\textrm{\scriptsize 32}$,
M.~Wessels$^\textrm{\scriptsize 60a}$,
J.~Wetter$^\textrm{\scriptsize 165}$,
K.~Whalen$^\textrm{\scriptsize 118}$,
N.L.~Whallon$^\textrm{\scriptsize 140}$,
A.M.~Wharton$^\textrm{\scriptsize 75}$,
A.~White$^\textrm{\scriptsize 8}$,
M.J.~White$^\textrm{\scriptsize 1}$,
R.~White$^\textrm{\scriptsize 34b}$,
D.~Whiteson$^\textrm{\scriptsize 166}$,
F.J.~Wickens$^\textrm{\scriptsize 133}$,
W.~Wiedenmann$^\textrm{\scriptsize 176}$,
M.~Wielers$^\textrm{\scriptsize 133}$,
C.~Wiglesworth$^\textrm{\scriptsize 39}$,
L.A.M.~Wiik-Fuchs$^\textrm{\scriptsize 23}$,
A.~Wildauer$^\textrm{\scriptsize 103}$,
F.~Wilk$^\textrm{\scriptsize 87}$,
H.G.~Wilkens$^\textrm{\scriptsize 32}$,
H.H.~Williams$^\textrm{\scriptsize 124}$,
S.~Williams$^\textrm{\scriptsize 109}$,
C.~Willis$^\textrm{\scriptsize 93}$,
S.~Willocq$^\textrm{\scriptsize 89}$,
J.A.~Wilson$^\textrm{\scriptsize 19}$,
I.~Wingerter-Seez$^\textrm{\scriptsize 5}$,
F.~Winklmeier$^\textrm{\scriptsize 118}$,
O.J.~Winston$^\textrm{\scriptsize 151}$,
B.T.~Winter$^\textrm{\scriptsize 23}$,
M.~Wittgen$^\textrm{\scriptsize 145}$,
M.~Wobisch$^\textrm{\scriptsize 82}$$^{,s}$,
T.M.H.~Wolf$^\textrm{\scriptsize 109}$,
R.~Wolff$^\textrm{\scriptsize 88}$,
M.W.~Wolter$^\textrm{\scriptsize 42}$,
H.~Wolters$^\textrm{\scriptsize 128a,128c}$,
S.D.~Worm$^\textrm{\scriptsize 133}$,
B.K.~Wosiek$^\textrm{\scriptsize 42}$,
J.~Wotschack$^\textrm{\scriptsize 32}$,
M.J.~Woudstra$^\textrm{\scriptsize 87}$,
K.W.~Wozniak$^\textrm{\scriptsize 42}$,
M.~Wu$^\textrm{\scriptsize 58}$,
M.~Wu$^\textrm{\scriptsize 33}$,
S.L.~Wu$^\textrm{\scriptsize 176}$,
X.~Wu$^\textrm{\scriptsize 52}$,
Y.~Wu$^\textrm{\scriptsize 92}$,
T.R.~Wyatt$^\textrm{\scriptsize 87}$,
B.M.~Wynne$^\textrm{\scriptsize 49}$,
S.~Xella$^\textrm{\scriptsize 39}$,
Z.~Xi$^\textrm{\scriptsize 92}$,
L.~Xia$^\textrm{\scriptsize 35c}$,
D.~Xu$^\textrm{\scriptsize 35a}$,
L.~Xu$^\textrm{\scriptsize 27}$,
B.~Yabsley$^\textrm{\scriptsize 152}$,
S.~Yacoob$^\textrm{\scriptsize 147a}$,
D.~Yamaguchi$^\textrm{\scriptsize 159}$,
Y.~Yamaguchi$^\textrm{\scriptsize 120}$,
A.~Yamamoto$^\textrm{\scriptsize 69}$,
S.~Yamamoto$^\textrm{\scriptsize 157}$,
T.~Yamanaka$^\textrm{\scriptsize 157}$,
K.~Yamauchi$^\textrm{\scriptsize 105}$,
Y.~Yamazaki$^\textrm{\scriptsize 70}$,
Z.~Yan$^\textrm{\scriptsize 24}$,
H.~Yang$^\textrm{\scriptsize 36c}$,
H.~Yang$^\textrm{\scriptsize 176}$,
Y.~Yang$^\textrm{\scriptsize 153}$,
Z.~Yang$^\textrm{\scriptsize 15}$,
W-M.~Yao$^\textrm{\scriptsize 16}$,
Y.C.~Yap$^\textrm{\scriptsize 83}$,
Y.~Yasu$^\textrm{\scriptsize 69}$,
E.~Yatsenko$^\textrm{\scriptsize 5}$,
K.H.~Yau~Wong$^\textrm{\scriptsize 23}$,
J.~Ye$^\textrm{\scriptsize 43}$,
S.~Ye$^\textrm{\scriptsize 27}$,
I.~Yeletskikh$^\textrm{\scriptsize 68}$,
E.~Yildirim$^\textrm{\scriptsize 86}$,
K.~Yorita$^\textrm{\scriptsize 174}$,
R.~Yoshida$^\textrm{\scriptsize 6}$,
K.~Yoshihara$^\textrm{\scriptsize 124}$,
C.~Young$^\textrm{\scriptsize 145}$,
C.J.S.~Young$^\textrm{\scriptsize 32}$,
S.~Youssef$^\textrm{\scriptsize 24}$,
D.R.~Yu$^\textrm{\scriptsize 16}$,
J.~Yu$^\textrm{\scriptsize 8}$,
J.~Yu$^\textrm{\scriptsize 67}$,
L.~Yuan$^\textrm{\scriptsize 70}$,
S.P.Y.~Yuen$^\textrm{\scriptsize 23}$,
I.~Yusuff$^\textrm{\scriptsize 30}$$^{,av}$,
B.~Zabinski$^\textrm{\scriptsize 42}$,
G.~Zacharis$^\textrm{\scriptsize 10}$,
R.~Zaidan$^\textrm{\scriptsize 13}$,
A.M.~Zaitsev$^\textrm{\scriptsize 132}$$^{,ah}$,
N.~Zakharchuk$^\textrm{\scriptsize 45}$,
J.~Zalieckas$^\textrm{\scriptsize 15}$,
A.~Zaman$^\textrm{\scriptsize 150}$,
S.~Zambito$^\textrm{\scriptsize 59}$,
D.~Zanzi$^\textrm{\scriptsize 91}$,
C.~Zeitnitz$^\textrm{\scriptsize 178}$,
M.~Zeman$^\textrm{\scriptsize 130}$,
A.~Zemla$^\textrm{\scriptsize 41a}$,
J.C.~Zeng$^\textrm{\scriptsize 169}$,
Q.~Zeng$^\textrm{\scriptsize 145}$,
O.~Zenin$^\textrm{\scriptsize 132}$,
T.~\v{Z}eni\v{s}$^\textrm{\scriptsize 146a}$,
D.~Zerwas$^\textrm{\scriptsize 119}$,
D.~Zhang$^\textrm{\scriptsize 92}$,
F.~Zhang$^\textrm{\scriptsize 176}$,
G.~Zhang$^\textrm{\scriptsize 36a}$$^{,ap}$,
H.~Zhang$^\textrm{\scriptsize 35b}$,
J.~Zhang$^\textrm{\scriptsize 6}$,
L.~Zhang$^\textrm{\scriptsize 51}$,
L.~Zhang$^\textrm{\scriptsize 36a}$,
M.~Zhang$^\textrm{\scriptsize 169}$,
R.~Zhang$^\textrm{\scriptsize 23}$,
R.~Zhang$^\textrm{\scriptsize 36a}$$^{,au}$,
X.~Zhang$^\textrm{\scriptsize 36b}$,
Y.~Zhang$^\textrm{\scriptsize 35a}$,
Z.~Zhang$^\textrm{\scriptsize 119}$,
X.~Zhao$^\textrm{\scriptsize 43}$,
Y.~Zhao$^\textrm{\scriptsize 36b}$$^{,aw}$,
Z.~Zhao$^\textrm{\scriptsize 36a}$,
A.~Zhemchugov$^\textrm{\scriptsize 68}$,
J.~Zhong$^\textrm{\scriptsize 122}$,
B.~Zhou$^\textrm{\scriptsize 92}$,
C.~Zhou$^\textrm{\scriptsize 176}$,
L.~Zhou$^\textrm{\scriptsize 43}$,
M.~Zhou$^\textrm{\scriptsize 35a}$,
M.~Zhou$^\textrm{\scriptsize 150}$,
N.~Zhou$^\textrm{\scriptsize 35c}$,
C.G.~Zhu$^\textrm{\scriptsize 36b}$,
H.~Zhu$^\textrm{\scriptsize 35a}$,
J.~Zhu$^\textrm{\scriptsize 92}$,
Y.~Zhu$^\textrm{\scriptsize 36a}$,
X.~Zhuang$^\textrm{\scriptsize 35a}$,
K.~Zhukov$^\textrm{\scriptsize 98}$,
A.~Zibell$^\textrm{\scriptsize 177}$,
D.~Zieminska$^\textrm{\scriptsize 64}$,
N.I.~Zimine$^\textrm{\scriptsize 68}$,
C.~Zimmermann$^\textrm{\scriptsize 86}$,
S.~Zimmermann$^\textrm{\scriptsize 51}$,
Z.~Zinonos$^\textrm{\scriptsize 103}$,
M.~Zinser$^\textrm{\scriptsize 86}$,
M.~Ziolkowski$^\textrm{\scriptsize 143}$,
L.~\v{Z}ivkovi\'{c}$^\textrm{\scriptsize 14}$,
G.~Zobernig$^\textrm{\scriptsize 176}$,
A.~Zoccoli$^\textrm{\scriptsize 22a,22b}$,
M.~zur~Nedden$^\textrm{\scriptsize 17}$,
L.~Zwalinski$^\textrm{\scriptsize 32}$.
\bigskip
\\
$^{1}$ Department of Physics, University of Adelaide, Adelaide, Australia\\
$^{2}$ Physics Department, SUNY Albany, Albany NY, United States of America\\
$^{3}$ Department of Physics, University of Alberta, Edmonton AB, Canada\\
$^{4}$ $^{(a)}$ Department of Physics, Ankara University, Ankara; $^{(b)}$ Istanbul Aydin University, Istanbul; $^{(c)}$ Division of Physics, TOBB University of Economics and Technology, Ankara, Turkey\\
$^{5}$ LAPP, CNRS/IN2P3 and Universit{\'e} Savoie Mont Blanc, Annecy-le-Vieux, France\\
$^{6}$ High Energy Physics Division, Argonne National Laboratory, Argonne IL, United States of America\\
$^{7}$ Department of Physics, University of Arizona, Tucson AZ, United States of America\\
$^{8}$ Department of Physics, The University of Texas at Arlington, Arlington TX, United States of America\\
$^{9}$ Physics Department, National and Kapodistrian University of Athens, Athens, Greece\\
$^{10}$ Physics Department, National Technical University of Athens, Zografou, Greece\\
$^{11}$ Department of Physics, The University of Texas at Austin, Austin TX, United States of America\\
$^{12}$ Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{13}$ Institut de F{\'\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Barcelona, Spain\\
$^{14}$ Institute of Physics, University of Belgrade, Belgrade, Serbia\\
$^{15}$ Department for Physics and Technology, University of Bergen, Bergen, Norway\\
$^{16}$ Physics Division, Lawrence Berkeley National Laboratory and University of California, Berkeley CA, United States of America\\
$^{17}$ Department of Physics, Humboldt University, Berlin, Germany\\
$^{18}$ Albert Einstein Center for Fundamental Physics and Laboratory for High Energy Physics, University of Bern, Bern, Switzerland\\
$^{19}$ School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{20}$ $^{(a)}$ Department of Physics, Bogazici University, Istanbul; $^{(b)}$ Department of Physics Engineering, Gaziantep University, Gaziantep; $^{(d)}$ Istanbul Bilgi University, Faculty of Engineering and Natural Sciences, Istanbul,Turkey; $^{(e)}$ Bahcesehir University, Faculty of Engineering and Natural Sciences, Istanbul, Turkey, Turkey\\
$^{21}$ Centro de Investigaciones, Universidad Antonio Narino, Bogota, Colombia\\
$^{22}$ $^{(a)}$ INFN Sezione di Bologna; $^{(b)}$ Dipartimento di Fisica e Astronomia, Universit{\`a} di Bologna, Bologna, Italy\\
$^{23}$ Physikalisches Institut, University of Bonn, Bonn, Germany\\
$^{24}$ Department of Physics, Boston University, Boston MA, United States of America\\
$^{25}$ Department of Physics, Brandeis University, Waltham MA, United States of America\\
$^{26}$ $^{(a)}$ Universidade Federal do Rio De Janeiro COPPE/EE/IF, Rio de Janeiro; $^{(b)}$ Electrical Circuits Department, Federal University of Juiz de Fora (UFJF), Juiz de Fora; $^{(c)}$ Federal University of Sao Joao del Rei (UFSJ), Sao Joao del Rei; $^{(d)}$ Instituto de Fisica, Universidade de Sao Paulo, Sao Paulo, Brazil\\
$^{27}$ Physics Department, Brookhaven National Laboratory, Upton NY, United States of America\\
$^{28}$ $^{(a)}$ Transilvania University of Brasov, Brasov, Romania; $^{(b)}$ Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest; $^{(c)}$ National Institute for Research and Development of Isotopic and Molecular Technologies, Physics Department, Cluj Napoca; $^{(d)}$ University Politehnica Bucharest, Bucharest; $^{(e)}$ West University in Timisoara, Timisoara, Romania\\
$^{29}$ Departamento de F{\'\i}sica, Universidad de Buenos Aires, Buenos Aires, Argentina\\
$^{30}$ Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{31}$ Department of Physics, Carleton University, Ottawa ON, Canada\\
$^{32}$ CERN, Geneva, Switzerland\\
$^{33}$ Enrico Fermi Institute, University of Chicago, Chicago IL, United States of America\\
$^{34}$ $^{(a)}$ Departamento de F{\'\i}sica, Pontificia Universidad Cat{\'o}lica de Chile, Santiago; $^{(b)}$ Departamento de F{\'\i}sica, Universidad T{\'e}cnica Federico Santa Mar{\'\i}a, Valpara{\'\i}so, Chile\\
$^{35}$ $^{(a)}$ Institute of High Energy Physics, Chinese Academy of Sciences, Beijing; $^{(b)}$ Department of Physics, Nanjing University, Jiangsu; $^{(c)}$ Physics Department, Tsinghua University, Beijing 100084, China\\
$^{36}$ $^{(a)}$ Department of Modern Physics, University of Science and Technology of China, Anhui; $^{(b)}$ School of Physics, Shandong University, Shandong; $^{(c)}$ Department of Physics and Astronomy, Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology (SKLPPC), Shanghai Jiao Tong University, Shanghai;, China\\
$^{37}$ Laboratoire de Physique Corpusculaire, Universit{\'e} Clermont Auvergne, Universit{\'e} Blaise Pascal, CNRS/IN2P3, Clermont-Ferrand, France\\
$^{38}$ Nevis Laboratory, Columbia University, Irvington NY, United States of America\\
$^{39}$ Niels Bohr Institute, University of Copenhagen, Kobenhavn, Denmark\\
$^{40}$ $^{(a)}$ INFN Gruppo Collegato di Cosenza, Laboratori Nazionali di Frascati; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} della Calabria, Rende, Italy\\
$^{41}$ $^{(a)}$ AGH University of Science and Technology, Faculty of Physics and Applied Computer Science, Krakow; $^{(b)}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Krakow, Poland\\
$^{42}$ Institute of Nuclear Physics Polish Academy of Sciences, Krakow, Poland\\
$^{43}$ Physics Department, Southern Methodist University, Dallas TX, United States of America\\
$^{44}$ Physics Department, University of Texas at Dallas, Richardson TX, United States of America\\
$^{45}$ DESY, Hamburg and Zeuthen, Germany\\
$^{46}$ Lehrstuhl f{\"u}r Experimentelle Physik IV, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{47}$ Institut f{\"u}r Kern-{~}und Teilchenphysik, Technische Universit{\"a}t Dresden, Dresden, Germany\\
$^{48}$ Department of Physics, Duke University, Durham NC, United States of America\\
$^{49}$ SUPA - School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{50}$ INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{51}$ Fakult{\"a}t f{\"u}r Mathematik und Physik, Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany\\
$^{52}$ Departement  de Physique Nucleaire et Corpusculaire, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{53}$ $^{(a)}$ INFN Sezione di Genova; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Genova, Genova, Italy\\
$^{54}$ $^{(a)}$ E. Andronikashvili Institute of Physics, Iv. Javakhishvili Tbilisi State University, Tbilisi; $^{(b)}$ High Energy Physics Institute, Tbilisi State University, Tbilisi, Georgia\\
$^{55}$ II Physikalisches Institut, Justus-Liebig-Universit{\"a}t Giessen, Giessen, Germany\\
$^{56}$ SUPA - School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{57}$ II Physikalisches Institut, Georg-August-Universit{\"a}t, G{\"o}ttingen, Germany\\
$^{58}$ Laboratoire de Physique Subatomique et de Cosmologie, Universit{\'e} Grenoble-Alpes, CNRS/IN2P3, Grenoble, France\\
$^{59}$ Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge MA, United States of America\\
$^{60}$ $^{(a)}$ Kirchhoff-Institut f{\"u}r Physik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(b)}$ Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(c)}$ ZITI Institut f{\"u}r technische Informatik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Mannheim, Germany\\
$^{61}$ Faculty of Applied Information Science, Hiroshima Institute of Technology, Hiroshima, Japan\\
$^{62}$ $^{(a)}$ Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong; $^{(b)}$ Department of Physics, The University of Hong Kong, Hong Kong; $^{(c)}$ Department of Physics and Institute for Advanced Study, The Hong Kong University of Science and Technology, Clear Water Bay, Kowloon, Hong Kong, China\\
$^{63}$ Department of Physics, National Tsing Hua University, Taiwan, Taiwan\\
$^{64}$ Department of Physics, Indiana University, Bloomington IN, United States of America\\
$^{65}$ Institut f{\"u}r Astro-{~}und Teilchenphysik, Leopold-Franzens-Universit{\"a}t, Innsbruck, Austria\\
$^{66}$ University of Iowa, Iowa City IA, United States of America\\
$^{67}$ Department of Physics and Astronomy, Iowa State University, Ames IA, United States of America\\
$^{68}$ Joint Institute for Nuclear Research, JINR Dubna, Dubna, Russia\\
$^{69}$ KEK, High Energy Accelerator Research Organization, Tsukuba, Japan\\
$^{70}$ Graduate School of Science, Kobe University, Kobe, Japan\\
$^{71}$ Faculty of Science, Kyoto University, Kyoto, Japan\\
$^{72}$ Kyoto University of Education, Kyoto, Japan\\
$^{73}$ Department of Physics, Kyushu University, Fukuoka, Japan\\
$^{74}$ Instituto de F{\'\i}sica La Plata, Universidad Nacional de La Plata and CONICET, La Plata, Argentina\\
$^{75}$ Physics Department, Lancaster University, Lancaster, United Kingdom\\
$^{76}$ $^{(a)}$ INFN Sezione di Lecce; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} del Salento, Lecce, Italy\\
$^{77}$ Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{78}$ Department of Experimental Particle Physics, Jo{\v{z}}ef Stefan Institute and Department of Physics, University of Ljubljana, Ljubljana, Slovenia\\
$^{79}$ School of Physics and Astronomy, Queen Mary University of London, London, United Kingdom\\
$^{80}$ Department of Physics, Royal Holloway University of London, Surrey, United Kingdom\\
$^{81}$ Department of Physics and Astronomy, University College London, London, United Kingdom\\
$^{82}$ Louisiana Tech University, Ruston LA, United States of America\\
$^{83}$ Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies, UPMC and Universit{\'e} Paris-Diderot and CNRS/IN2P3, Paris, France\\
$^{84}$ Fysiska institutionen, Lunds universitet, Lund, Sweden\\
$^{85}$ Departamento de Fisica Teorica C-15, Universidad Autonoma de Madrid, Madrid, Spain\\
$^{86}$ Institut f{\"u}r Physik, Universit{\"a}t Mainz, Mainz, Germany\\
$^{87}$ School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{88}$ CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{89}$ Department of Physics, University of Massachusetts, Amherst MA, United States of America\\
$^{90}$ Department of Physics, McGill University, Montreal QC, Canada\\
$^{91}$ School of Physics, University of Melbourne, Victoria, Australia\\
$^{92}$ Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{93}$ Department of Physics and Astronomy, Michigan State University, East Lansing MI, United States of America\\
$^{94}$ $^{(a)}$ INFN Sezione di Milano; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Milano, Milano, Italy\\
$^{95}$ B.I. Stepanov Institute of Physics, National Academy of Sciences of Belarus, Minsk, Republic of Belarus\\
$^{96}$ Research Institute for Nuclear Problems of Byelorussian State University, Minsk, Republic of Belarus\\
$^{97}$ Group of Particle Physics, University of Montreal, Montreal QC, Canada\\
$^{98}$ P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow, Russia\\
$^{99}$ Institute for Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$^{100}$ National Research Nuclear University MEPhI, Moscow, Russia\\
$^{101}$ D.V. Skobeltsyn Institute of Nuclear Physics, M.V. Lomonosov Moscow State University, Moscow, Russia\\
$^{102}$ Fakult{\"a}t f{\"u}r Physik, Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen, M{\"u}nchen, Germany\\
$^{103}$ Max-Planck-Institut f{\"u}r Physik (Werner-Heisenberg-Institut), M{\"u}nchen, Germany\\
$^{104}$ Nagasaki Institute of Applied Science, Nagasaki, Japan\\
$^{105}$ Graduate School of Science and Kobayashi-Maskawa Institute, Nagoya University, Nagoya, Japan\\
$^{106}$ $^{(a)}$ INFN Sezione di Napoli; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Napoli, Napoli, Italy\\
$^{107}$ Department of Physics and Astronomy, University of New Mexico, Albuquerque NM, United States of America\\
$^{108}$ Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen, Netherlands\\
$^{109}$ Nikhef National Institute for Subatomic Physics and University of Amsterdam, Amsterdam, Netherlands\\
$^{110}$ Department of Physics, Northern Illinois University, DeKalb IL, United States of America\\
$^{111}$ Budker Institute of Nuclear Physics, SB RAS, Novosibirsk, Russia\\
$^{112}$ Department of Physics, New York University, New York NY, United States of America\\
$^{113}$ Ohio State University, Columbus OH, United States of America\\
$^{114}$ Faculty of Science, Okayama University, Okayama, Japan\\
$^{115}$ Homer L. Dodge Department of Physics and Astronomy, University of Oklahoma, Norman OK, United States of America\\
$^{116}$ Department of Physics, Oklahoma State University, Stillwater OK, United States of America\\
$^{117}$ Palack{\'y} University, RCPTM, Olomouc, Czech Republic\\
$^{118}$ Center for High Energy Physics, University of Oregon, Eugene OR, United States of America\\
$^{119}$ LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Orsay, France\\
$^{120}$ Graduate School of Science, Osaka University, Osaka, Japan\\
$^{121}$ Department of Physics, University of Oslo, Oslo, Norway\\
$^{122}$ Department of Physics, Oxford University, Oxford, United Kingdom\\
$^{123}$ $^{(a)}$ INFN Sezione di Pavia; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Pavia, Pavia, Italy\\
$^{124}$ Department of Physics, University of Pennsylvania, Philadelphia PA, United States of America\\
$^{125}$ National Research Centre "Kurchatov Institute" B.P.Konstantinov Petersburg Nuclear Physics Institute, St. Petersburg, Russia\\
$^{126}$ $^{(a)}$ INFN Sezione di Pisa; $^{(b)}$ Dipartimento di Fisica E. Fermi, Universit{\`a} di Pisa, Pisa, Italy\\
$^{127}$ Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh PA, United States of America\\
$^{128}$ $^{(a)}$ Laborat{\'o}rio de Instrumenta{\c{c}}{\~a}o e F{\'\i}sica Experimental de Part{\'\i}culas - LIP, Lisboa; $^{(b)}$ Faculdade de Ci{\^e}ncias, Universidade de Lisboa, Lisboa; $^{(c)}$ Department of Physics, University of Coimbra, Coimbra; $^{(d)}$ Centro de F{\'\i}sica Nuclear da Universidade de Lisboa, Lisboa; $^{(e)}$ Departamento de Fisica, Universidade do Minho, Braga; $^{(f)}$ Departamento de Fisica Teorica y del Cosmos and CAFPE, Universidad de Granada, Granada (Spain); $^{(g)}$ Dep Fisica and CEFITEC of Faculdade de Ciencias e Tecnologia, Universidade Nova de Lisboa, Caparica, Portugal\\
$^{129}$ Institute of Physics, Academy of Sciences of the Czech Republic, Praha, Czech Republic\\
$^{130}$ Czech Technical University in Prague, Praha, Czech Republic\\
$^{131}$ Charles University, Faculty of Mathematics and Physics, Prague, Czech Republic\\
$^{132}$ State Research Center Institute for High Energy Physics (Protvino), NRC KI, Russia\\
$^{133}$ Particle Physics Department, Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{134}$ $^{(a)}$ INFN Sezione di Roma; $^{(b)}$ Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, Roma, Italy\\
$^{135}$ $^{(a)}$ INFN Sezione di Roma Tor Vergata; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{136}$ $^{(a)}$ INFN Sezione di Roma Tre; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} Roma Tre, Roma, Italy\\
$^{137}$ $^{(a)}$ Facult{\'e} des Sciences Ain Chock, R{\'e}seau Universitaire de Physique des Hautes Energies - Universit{\'e} Hassan II, Casablanca; $^{(b)}$ Centre National de l'Energie des Sciences Techniques Nucleaires, Rabat; $^{(c)}$ Facult{\'e} des Sciences Semlalia, Universit{\'e} Cadi Ayyad, LPHEA-Marrakech; $^{(d)}$ Facult{\'e} des Sciences, Universit{\'e} Mohamed Premier and LPTPM, Oujda; $^{(e)}$ Facult{\'e} des sciences, Universit{\'e} Mohammed V, Rabat, Morocco\\
$^{138}$ DSM/IRFU (Institut de Recherches sur les Lois Fondamentales de l'Univers), CEA Saclay (Commissariat {\`a} l'Energie Atomique et aux Energies Alternatives), Gif-sur-Yvette, France\\
$^{139}$ Santa Cruz Institute for Particle Physics, University of California Santa Cruz, Santa Cruz CA, United States of America\\
$^{140}$ Department of Physics, University of Washington, Seattle WA, United States of America\\
$^{141}$ Department of Physics and Astronomy, University of Sheffield, Sheffield, United Kingdom\\
$^{142}$ Department of Physics, Shinshu University, Nagano, Japan\\
$^{143}$ Fachbereich Physik, Universit{\"a}t Siegen, Siegen, Germany\\
$^{144}$ Department of Physics, Simon Fraser University, Burnaby BC, Canada\\
$^{145}$ SLAC National Accelerator Laboratory, Stanford CA, United States of America\\
$^{146}$ $^{(a)}$ Faculty of Mathematics, Physics {\&} Informatics, Comenius University, Bratislava; $^{(b)}$ Department of Subnuclear Physics, Institute of Experimental Physics of the Slovak Academy of Sciences, Kosice, Slovak Republic\\
$^{147}$ $^{(a)}$ Department of Physics, University of Cape Town, Cape Town; $^{(b)}$ Department of Physics, University of Johannesburg, Johannesburg; $^{(c)}$ School of Physics, University of the Witwatersrand, Johannesburg, South Africa\\
$^{148}$ $^{(a)}$ Department of Physics, Stockholm University; $^{(b)}$ The Oskar Klein Centre, Stockholm, Sweden\\
$^{149}$ Physics Department, Royal Institute of Technology, Stockholm, Sweden\\
$^{150}$ Departments of Physics {\&} Astronomy and Chemistry, Stony Brook University, Stony Brook NY, United States of America\\
$^{151}$ Department of Physics and Astronomy, University of Sussex, Brighton, United Kingdom\\
$^{152}$ School of Physics, University of Sydney, Sydney, Australia\\
$^{153}$ Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{154}$ Department of Physics, Technion: Israel Institute of Technology, Haifa, Israel\\
$^{155}$ Raymond and Beverly Sackler School of Physics and Astronomy, Tel Aviv University, Tel Aviv, Israel\\
$^{156}$ Department of Physics, Aristotle University of Thessaloniki, Thessaloniki, Greece\\
$^{157}$ International Center for Elementary Particle Physics and Department of Physics, The University of Tokyo, Tokyo, Japan\\
$^{158}$ Graduate School of Science and Technology, Tokyo Metropolitan University, Tokyo, Japan\\
$^{159}$ Department of Physics, Tokyo Institute of Technology, Tokyo, Japan\\
$^{160}$ Tomsk State University, Tomsk, Russia, Russia\\
$^{161}$ Department of Physics, University of Toronto, Toronto ON, Canada\\
$^{162}$ $^{(a)}$ INFN-TIFPA; $^{(b)}$ University of Trento, Trento, Italy, Italy\\
$^{163}$ $^{(a)}$ TRIUMF, Vancouver BC; $^{(b)}$ Department of Physics and Astronomy, York University, Toronto ON, Canada\\
$^{164}$ Faculty of Pure and Applied Sciences, and Center for Integrated Research in Fundamental Science and Engineering, University of Tsukuba, Tsukuba, Japan\\
$^{165}$ Department of Physics and Astronomy, Tufts University, Medford MA, United States of America\\
$^{166}$ Department of Physics and Astronomy, University of California Irvine, Irvine CA, United States of America\\
$^{167}$ $^{(a)}$ INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine; $^{(b)}$ ICTP, Trieste; $^{(c)}$ Dipartimento di Chimica, Fisica e Ambiente, Universit{\`a} di Udine, Udine, Italy\\
$^{168}$ Department of Physics and Astronomy, University of Uppsala, Uppsala, Sweden\\
$^{169}$ Department of Physics, University of Illinois, Urbana IL, United States of America\\
$^{170}$ Instituto de Fisica Corpuscular (IFIC) and Departamento de Fisica Atomica, Molecular y Nuclear and Departamento de Ingenier{\'\i}a Electr{\'o}nica and Instituto de Microelectr{\'o}nica de Barcelona (IMB-CNM), University of Valencia and CSIC, Valencia, Spain\\
$^{171}$ Department of Physics, University of British Columbia, Vancouver BC, Canada\\
$^{172}$ Department of Physics and Astronomy, University of Victoria, Victoria BC, Canada\\
$^{173}$ Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{174}$ Waseda University, Tokyo, Japan\\
$^{175}$ Department of Particle Physics, The Weizmann Institute of Science, Rehovot, Israel\\
$^{176}$ Department of Physics, University of Wisconsin, Madison WI, United States of America\\
$^{177}$ Fakult{\"a}t f{\"u}r Physik und Astronomie, Julius-Maximilians-Universit{\"a}t, W{\"u}rzburg, Germany\\
$^{178}$ Fakult{\"a}t f{\"u}r Mathematik und Naturwissenschaften, Fachgruppe Physik, Bergische Universit{\"a}t Wuppertal, Wuppertal, Germany\\
$^{179}$ Department of Physics, Yale University, New Haven CT, United States of America\\
$^{180}$ Yerevan Physics Institute, Yerevan, Armenia\\
$^{181}$ Centre de Calcul de l'Institut National de Physique Nucl{\'e}aire et de Physique des Particules (IN2P3), Villeurbanne, France\\
$^{a}$ Also at Department of Physics, King's College London, London, United Kingdom\\
$^{b}$ Also at Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{c}$ Also at Novosibirsk State University, Novosibirsk, Russia\\
$^{d}$ Also at TRIUMF, Vancouver BC, Canada\\
$^{e}$ Also at Department of Physics {\&} Astronomy, University of Louisville, Louisville, KY, United States of America\\
$^{f}$ Also at Physics Department, An-Najah National University, Nablus, Palestine\\
$^{g}$ Also at Department of Physics, California State University, Fresno CA, United States of America\\
$^{h}$ Also at Department of Physics, University of Fribourg, Fribourg, Switzerland\\
$^{i}$ Also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain\\
$^{j}$ Also at Departamento de Fisica e Astronomia, Faculdade de Ciencias, Universidade do Porto, Portugal\\
$^{k}$ Also at Tomsk State University, Tomsk, Russia, Russia\\
$^{l}$ Also at The Collaborative Innovation Center of Quantum Matter (CICQM), Beijing, China\\
$^{m}$ Also at Universita di Napoli Parthenope, Napoli, Italy\\
$^{n}$ Also at Institute of Particle Physics (IPP), Canada\\
$^{o}$ Also at Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest, Romania\\
$^{p}$ Also at Department of Physics, St. Petersburg State Polytechnical University, St. Petersburg, Russia\\
$^{q}$ Also at Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{r}$ Also at Centre for High Performance Computing, CSIR Campus, Rosebank, Cape Town, South Africa\\
$^{s}$ Also at Louisiana Tech University, Ruston LA, United States of America\\
$^{t}$ Also at Institucio Catalana de Recerca i Estudis Avancats, ICREA, Barcelona, Spain\\
$^{u}$ Also at Graduate School of Science, Osaka University, Osaka, Japan\\
$^{v}$ Also at Fakult{\"a}t f{\"u}r Mathematik und Physik, Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany\\
$^{w}$ Also at Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen, Netherlands\\
$^{x}$ Also at Department of Physics, The University of Texas at Austin, Austin TX, United States of America\\
$^{y}$ Also at Institute of Theoretical Physics, Ilia State University, Tbilisi, Georgia\\
$^{z}$ Also at CERN, Geneva, Switzerland\\
$^{aa}$ Also at Georgian Technical University (GTU),Tbilisi, Georgia\\
$^{ab}$ Also at Ochadai Academic Production, Ochanomizu University, Tokyo, Japan\\
$^{ac}$ Also at Manhattan College, New York NY, United States of America\\
$^{ad}$ Also at Academia Sinica Grid Computing, Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{ae}$ Also at School of Physics, Shandong University, Shandong, China\\
$^{af}$ Also at Departamento de Fisica Teorica y del Cosmos and CAFPE, Universidad de Granada, Granada (Spain), Portugal\\
$^{ag}$ Also at Department of Physics, California State University, Sacramento CA, United States of America\\
$^{ah}$ Also at Moscow Institute of Physics and Technology State University, Dolgoprudny, Russia\\
$^{ai}$ Also at Departement  de Physique Nucleaire et Corpusculaire, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{aj}$ Also at International School for Advanced Studies (SISSA), Trieste, Italy\\
$^{ak}$ Also at Department of Physics and Astronomy, University of South Carolina, Columbia SC, United States of America\\
$^{al}$ Also at Institut de F{\'\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Barcelona, Spain\\
$^{am}$ Also at School of Physics, Sun Yat-sen University, Guangzhou, China\\
$^{an}$ Also at Institute for Nuclear Research and Nuclear Energy (INRNE) of the Bulgarian Academy of Sciences, Sofia, Bulgaria\\
$^{ao}$ Also at Faculty of Physics, M.V.Lomonosov Moscow State University, Moscow, Russia\\
$^{ap}$ Also at Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{aq}$ Also at National Research Nuclear University MEPhI, Moscow, Russia\\
$^{ar}$ Also at Department of Physics, Stanford University, Stanford CA, United States of America\\
$^{as}$ Also at Institute for Particle and Nuclear Physics, Wigner Research Centre for Physics, Budapest, Hungary\\
$^{at}$ Also at Giresun University, Faculty of Engineering, Turkey\\
$^{au}$ Also at CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{av}$ Also at University of Malaya, Department of Physics, Kuala Lumpur, Malaysia\\
$^{aw}$ Also at LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Orsay, France\\
$^{*}$ Deceased
\end{flushleft}

%\end{document}
% Created with xml2latex.py

